A learning scheme by sparse grids and Picard approximations for semilinear parabolic PDEs

Relying on the classical connection between Backward Stochastic Differential Equations (BSDEs) and non-linear parabolic partial differential equations (PDEs), we propose a new probabilistic learning scheme for solving high-dimensional semi-linear parabolic PDEs. This scheme is inspired by the approach coming from machine learning and developed using deep neural networks in Han and al. [32]. Our algorithm is based on a Picard iteration scheme in which a sequence of linear-quadratic optimisation problem is solved by means of stochastic gradient descent (SGD) algorithm. In the framework of a linear specification of the approximation space, we manage to prove a convergence result for our scheme, under some smallness condition. In practice, in order to be able to treat high-dimensional examples, we employ sparse grid approximation spaces. In the case of periodic coefficients and using pre-wavelet basis functions, we obtain an upper bound on the global complexity of our method. It shows in particular that the curse of dimensionality is tamed in the sense that in order to achieve a root mean squared error of order ${\epsilon}$, for a prescribed precision ${\epsilon}$, the complexity of the Picard algorithm grows polynomially in ${\epsilon}^{-1}$ up to some logarithmic factor $ |log({\epsilon})| $ which grows linearly with respect to the PDE dimension. Various numerical results are presented to validate the performance of our method and to compare them with some recent machine learning schemes proposed in Han and al. [20] and Hur\'e and al. [37].

==> v4.33 - arXiv submission/appbis.tex <==
%!TEX root = main.tex
\section{Appendix}

%\subsection{Auxiliary results}


 

%\subsection{Algorithms parameters}
\label{se algo param}

We gather below all the  parameters values used in the various algorithms, examples and basis functions settings.
In particular, we recall that the domain specification is given in \eqref{eq de BM domain} and \eqref{eq de GBM domain} The learning rates are given by \eqref{eq de learning rate}.
Denoting
\[ \Gamma(\lambda) := ( \alpha(\lambda ), \beta_1(\lambda), \beta_0(\lambda), m_0(\lambda)) \in \mathbb{R}^4,  \]
we set the  parameters in all the approximating space  $\mathscr{V}^z_n , 1\le n\le N-1$ to be the same: namely $\Gamma(\mathfrak{z}^{n, \cdot}) = \Gamma(\mathfrak{z}^{1, \cdot })$ for all $n\ge 2$. Thus, in the table below, the parameters of the learning rates are simply denoted by: 
\[ \Gamma := \{ \Gamma(\mathfrak{y}), \Gamma(\mathfrak{z}^{0, \cdot} ), \Gamma(\mathfrak{z}^{1, \cdot }) \} \in \mathbb{R}^{3\times 4}.  \]


\begin{table}[H]
	\centering
	\resizebox{\textwidth}{30mm}{
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c| } 
		\hline
		Algorithms & Basis functions &  dim & N & M & T &  Initial $\mathfrak{z}^{n, k}$ & p & $\Gamma$ & $\cE_{\mathrm{MSE}} $ \\
%		\hline
%		\multirow{2.5}*{\tabincell{c}{\emph{Direct Algorithm} }} & \multirow{2.5}*{Pre-wavelets} & 1 & 10  & 30000   & 0.3  & 0 &   \diagbox{}{} &  \tabincell{c}{ (0.6, 0, 2, 4000),  \\ (0.6, 0, 300, 4000) } & 0.0025  \\
%		\cline{3 - 10}
%		  & &  3 & 10  & 100000   &   0.3  &  0 &   \diagbox{}{}  &  \tabincell{c}{ (0.6, 0, 3, 8000),  \\ (0.6, 0, 20, 8000) } & 0.0273 \\
		\hline
		\multirow{8}*{\tabincell{c}{ \emph{Picard Algorithm} }} & \multirow{8}*{Pre-wavelets} & \multirow{8}*{3} & \multirow{8}*{10}  & \multirow{8}*{100000}   &  \multirow{8}*{0.3}  &  \multirow{8}*{0} &  1 &  \tabincell{c}{ (0.6, 0, 3, 15000),  \\ (0.6, 0, 20, 10000) }  & 0.0286 \\
		\cline{8 - 10}
		&  &  &   &   &    &   &  2 &  \tabincell{c}{ (0.6, 0, 2, 8000),  \\ (0.6, 0, 10, 8000 } & 0.0247  \\
		\cline{8 - 10}
		&  &  &   &   &    &   &  3 &  \tabincell{c}{ (0.6, 0, 1, 8000),  \\ (0.6, 0, 5, 8000 } & 0.0219 \\
		\cline{8 - 10}
		&  &  &   &   &    &   &  4 &  \tabincell{c}{ (0.6, 0, 0.5, 8000),  \\ (0.6, 0, 3, 8000) } & 0.0207 \\
		\cline{8 - 10}
		&  &  &   &   &    &   &  5 &  \tabincell{c}{ (0.6, 0, 0.5, 8000),  \\ (0.6, 0, 3, 8000) } & 0.0201 \\
		\hline
	\end{tabular}
	} 
	\caption{Parameters for the periodic example} \label{Parameters periodic}
\end{table}


\begin{table}[H]
	\centering
	\resizebox{\textwidth}{32mm}{
	\begin{tabular}{|c|c|c|c|c|c|c|c| } 
		\hline
		\multicolumn{1}{|c|}{\multirow{1}*{Examples}}&  a & dim & M &  N &   Initial $y_0$  & \multirow{1}*{ Learning rate } \\
		\hline
		\multirow{1}*{\tabincell{c}{Quadratic}} & 1  & 5  & 2000 &  10   &  0.5 & 0.01    \\
		\hline
		\multirow{1}*{\tabincell{c}{Limits to \\ Picard algorithm}} & -0.4  & 2 & 5000 & 20   &  0.3 &  0.002   \\
		\cline{2 - 7}
%		  & -0.8 & 2  &    &  0.1  &    \\
%		\cline{2 - 6}
		 & -1.5 & 2  & 5000 &  20  &  0  &  0.001  \\
		\hline
		\multirow{7}*{\tabincell{c}{Financial \\ example}} & \multirow{7}*{N.A.}  & 2  &6000 &  20  &  2  &  0.005    \\
		\cline{3 - 7}
		& & 4  & 6000&  20  & 5   &   0.005  \\
		\cline{3 - 7}
		 &   & 5  &  5000&   20  & 5   &   0.005      \\
		\cline{3 - 7}
		& & 10  & 5000  & 20  & 8   &   0.005     \\
		\cline{3 - 7}
		&  & 15  &5000 &  20  & 8   &   0.005     \\
		\cline{3 - 7}
		&  & 20  &5000 &   20  & 8   &   0.005    \\
		\cline{3 - 7}
		&  & 25  & 5000 &  20  & 8   &   0.005   \\
		\hline
	\end{tabular}
	} 
	\caption{Parameters by model for the \emph{deep learning method} with $ layers = 4, batchsize = 64$}
	 \label{Parameters deep learning}
\end{table}




\begin{table}[htp]
	\centering
	\resizebox{\textwidth}{110mm}{
	\begin{tabular}{|c|c|c|c|c|c|c|c|c| } 
		\hline
		\multicolumn{1}{|c|}{\multirow{2}*{Examples}}& \multicolumn{1}{c|}{\multirow{2}*{Basis functions}}&  \multirow{2}*{ dim }& \multirow{2}*{ N }& \multirow{2}*{r} & \multicolumn{3}{c|}{ \multirow{1}*{Initial value}}  & \multirow{2}*{ $\Gamma$ } \\
		 \cline{6-8}
		& &   & & & $\mathfrak{y} $ & $ \mathfrak{z}^{0, \cdot} $ &  $\mathfrak{z}^{n, k}$ & \\
		\hline
		\multirow{4}*{\tabincell{c}{Quadratic \\ model}} & Pre-wavelets & 5 & 10  & 2   & 0.5  &  -0.2 & 0 &  \tabincell{c}{ (1, 0, 1, 100), \\ (0.8, 0, 1, 100),  \\ (0.86, 0.02, 0.05, 100) }  \\
		\cline{2 - 9}
		  & \multirow{1}*{Hat} & 
%		  25 & 10  & 2.8   &   4 &  0 &0  &  \tabincell{c}{ (0.9, 0, 0.7, 100), \\ (0.7, 0, 1, 100),  \\ (1, 0.08, 0.15, 1000) }  \\
%		  \cline{3 - 9}
%		  &  & 
		  100 & 10  & 3.2   &   5.5  &  0 & 0  &  \tabincell{c}{ (0.9, 0, 1, 100), \\ (0.7, 0, 1, 100),  \\ (1, 0.003, 0.01, 1000) }  \\
		\hline
		\multirow{20}*{\tabincell{c}{Financial \\ example}} & \multirow{3}*{Pre-wavelets} & 2 & 10  & 2   &  2  &  0 &  0&  \tabincell{c}{ (1, 0, 1.5, 1000), \\(1, 0, 20, 1000),     \\ (1, 0.003, 0.01, 1000)}  \\
		\cline{3 - 9}
		& & 4& 10  & 2   &  5  &  0 &  0&  \tabincell{c}{(1, 0, 1, 1000), \\(1, 0, 20, 1000),     \\ (1, 0.001, 0.01, 1000) }  \\
		\cline{2 - 9}
		 & \multirow{13}*{Hat}  & 5 & 10 & 2   &  5  & 0  & 0 &  \tabincell{c}{ (0.95, 0, 0.3, 100), \\ (1, 0, 5, 100), \\ (1, 0.001, 0.01, 100) }  \\
		\cline{3 - 9}
		& & 10 & 10 & 2.5   &   8 &  0 & 0 &  \tabincell{c}{ (0.9, 0, 0.35, 300), \\ (1, 0, 5, 300), \\ (1, 0.001, 0.01, 300) }  \\
		\cline{3 - 9}
		&  & 15& 10  & 2.5   &  8  & 0  & 0 &  \tabincell{c}{ (0.85, 0, 0.3, 500), \\ (1, 0, 5, 500), \\ (1, 0.001, 0.01, 500) }  \\
		\cline{3 - 9}
		&  & 20 & 10 & 2.5   &  8  & 0  & 0 &  \tabincell{c}{(0.8, 0, 0.2, 1000), \\ (1, 0, 5, 1000), \\ (1, 0.001, 0.01, 1000) }  \\
		\cline{3 - 9}
		&  & 25 & 10 & 2.8   &  8  &  0 & 0 &  \tabincell{c}{ (0.7, 0, 0.2, 1500), \\ (1, 0, 5, 1500), \\ (1, 0.001, 0.01, 1500) }  \\
		\hline
		\multirow{13}*{\tabincell{c}{The \\challenging\\ example}} & \multirow{13}*{Hat}  & 1 & 10 & 2   &  0.5  &  0  &  0 &  \tabincell{c}{ (1, 0, 0.5, 100), \\ (1, 0, 3, 100),  \\ (1, 0.1, 0.1, 100) }  \\
		\cline{3 - 9}
		&   & 2  & 20 & 2   &  0.1  & 0  &  0&  \tabincell{c}{ (1, 0, 0.5, 100), \\ (1, 0, 5, 100),  \\ (1, 0.2, 0.5, 100) }  \\
		\cline{3 - 9}
		&  & 5 & 40 & 2   &   0.4 &-1   & 0 &  \tabincell{c}{ (1, 0, 0.5, 300), \\ (0.95, 0, 5, 500),  \\ (1, 0.2, 0.1, 500) }  \\
		\cline{3 - 9}
		&  & 8  & 60& 2.2  &   0.6 & 1  & 0.08 &  \tabincell{c}{ (1, 0, 0.35, 500), \\ (1, 0, 5, 500),  \\ (1, 0.2, 1, 500) }  \\
		\cline{3 - 9}
		& & 10 & 100 & 2.5  &  0.1  & -1  & -0.1 &  \tabincell{c}{  (1, 0, 0.35, 500), \\ (0.95, 0, 5, 500),  \\ (1, 0.2, 1, 500) }  \\
		\hline
	\end{tabular}
	} 
	\caption{Parameters by model for the \emph{direct algorithm}}
	 \label{Parameters direct}
\end{table}


\begin{table}[htp]
	\centering
	\resizebox{\textwidth}{110mm}{
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c| } 
		\hline
		\multicolumn{1}{|c|}{\multirow{2}*{Examples}}& \multicolumn{1}{c|}{\multirow{2}*{Basis functions}}&  \multirow{2}*{ dim }& \multirow{2}*{ r }&  \multicolumn{3}{c|}{ \multirow{1}*{Initial value}}  & \multirow{2}*{ a } & \multirow{2}*{ p } & \multirow{2}*{ $\Gamma$ } \\
		 \cline{5-7}
		& &   & & $\mathfrak{y} $ & $ \mathfrak{z}^{0, \cdot} $ &  $\mathfrak{z}^{n, k}$  & & & \\
		\hline
		\multirow{10}*{\tabincell{c}{Quadratic \\ model}} & \multirow{8}*{Pre-wavelets} &  \multirow{8}*{5}  &  \multirow{8}*{2}   &  \multirow{8}*{0.5}  &  \multirow{8}*{-0.2} & \multirow{8}*{0} &  \multirow{8}*{1} &  1 & \tabincell{c}{ (1, 0, 0.8, 100), \\ (0.9, 0, 1, 100),  \\ (0.84, 0.02, 0.05, 100) }  \\
		\cline{ 9 -10}
		&  & &&&& & &2 &   \tabincell{c}{ (1, 0, 0.3, 100), \\ (0.9, 0, 0.4, 100),  \\ (0.84, 0.01, 0.02, 100) }  \\
		\cline{9 - 10}
		&  & &&&& &  & $ p \ge 3 $& \tabincell{c}{ (1, 0, 0.2, 100), \\ (0.9, 0, 0.2, 100),  \\ (0.84, 0.005, 0.01, 100) }  \\
		\cline{2 - 10}
		  & \multirow{1}*{Hat} & \multirow{1}*{25}  & \multirow{1}*{2.8 }  & \multirow{1}*{ 2}   & \multirow{1}*{0.1}  & \multirow{1}*{0} &\multirow{1}*{1} &$1\le p\le 3$ & \tabincell{c}{ (0.9, 0, 0.5, 100), \\ (0.8, 0, 0.8, 100),  \\ (1, 0.003, 0.01, 1000) }  \\
%		  \cline{9 - 10}
%		  &&&   &    &   &  & & 2& \tabincell{c}{ (0.9, 0, 0.45, 100), \\ (0.7, 0, 0.6, 100),  \\ (0.8, 0.03, 0.06, 100) }  \\
%		  \cline{9 - 10}
%		  &&&   &    &   &  & & 3& \tabincell{c}{ (0.9, 0, 0.4, 100), \\ (0.7, 0, 0.5, 100),  \\ (0.8, 0.02, 0.04, 100) }  \\
%		  \cline{9 - 10}
%		  &&&   &    &   &  & & 4& \tabincell{c}{ (0.9, 0, 0.2, 100), \\ (0.7, 0, 0.3, 100),  \\ (0.8, 0.01, 0.03, 100) }  \\
%		   \cline{9 - 10}
%		  &&&   &    &   &  & & $p\ge 5$ & \tabincell{c}{ (0.9, 0, 0.1, 100), \\ (0.7, 0, 0.2, 100),  \\ (0.8, 0.01, 0.02, 100) }  \\
		\hline
		\multirow{25}*{\tabincell{c}{Financial \\ example}} & \multirow{12}*{Pre-wavelets} & \multirow{12}*{4}  & \multirow{12}*{2}   & \multirow{12}*{5}   & \multirow{12}*{0.1}  & \multirow{12}*{-0.01} & \multirow{12}*{N.A.} & 1&  \tabincell{c}{ (1, 0, 1, 1000), \\ (1, 0, 20, 1000),  \\ (1, 0.001, 0.01, 1000) }  \\
		\cline{9- 10}
		& &   &    &    &   &  & &2&  \tabincell{c}{(1, 0, 0.3, 1000), \\ (1, 0, 5, 1000),  \\ (1, 0.0005, 0.005, 1000)  }  \\
		\cline{9- 10}
		& &   &    &    &   &  & &3&  \tabincell{c}{ (1, 0, 0.2, 1000), \\ (1, 0, 5, 1000),  \\ (1, 0.0003, 0.003, 1000) }  \\
		\cline{9- 10}
		& &   &    &    &   &  & &4, 5&  \tabincell{c}{ (1, 0, 0.15, 1000), \\ (1, 0, 3, 1000),  \\ (1, 0.0002, 0.002, 1000) }  \\
		\cline{9- 10}
		& &   &    &    &   &  & & $p\ge 6$ &  \tabincell{c}{ (1, 0, 0.1, 1000), \\ (1, 0, 2, 1000),  \\ (1, 0.0001, 0.001, 1000)  }  \\
		\cline{2- 10}
		 & \multirow{10}*{Hat}  &\multirow{10}*{ 20}  & \multirow{10}*{2.5}   &   \multirow{10}*{8} & \multirow{10}*{0} & \multirow{10}*{0} & \multirow{10}*{N.A.} & 1& \tabincell{c}{ (0.9, 0, 0.6, 1000), \\ (1, 0, 5, 1000),  \\ (1, 0.001, 0.01, 1000) }  \\
		 \cline{9 - 10}
		 &&&  &    &  & &  &2 & \tabincell{c}{ (0.9, 0, 0.2, 1000), \\ (1, 0, 4, 1000),  \\ (1, 0.001, 0.01, 1000) }  \\
		 \cline{9 - 10}
		 & &&  &    &  & &  & 3& \tabincell{c}{ (0.9, 0, 0.15, 1000), \\ (1, 0, 3, 1000),  \\ (1, 0.0005, 0.005, 1000) }  \\
		 \cline{9 - 10}
		 &&&   &    &  & &  &  $p\ge 4$& \tabincell{c}{ (0.9, 0, 0.1, 1000), \\ (1, 0, 2, 1000),  \\ (1, 0.0005, 0.005, 1000) }  \\
		\hline
		\multirow{4}*{\tabincell{c}{Limits to \\ Picard \\ algorithm}} & \multirow{4}*{Pre-wavelets}  &  \multirow{4}*{2}  &  \multirow{4}*{2}   & 0.3   & 0 & 0   & -0.4&  $1\le p \le 9$  &   \tabincell{c}{ (1, 0, 1, 300), \\ (1, 0, 1, 300),  \\ (1, 0.6, 0.1, 300) }  \\
		\cline{5 - 10}
		&   & &   &  0  &  0 & 0&  -1.5 & $1\le p \le 9$ &  \tabincell{c}{ (1, 0, 2, 300), \\ (1, 0, 1, 300),  \\ (1, 0.6, 0.1, 300)  }  \\
		\hline
%
%		\multirow{5}*{\tabincell{c}{The \\challenging \\ example}} & \multirow{5}*{Hat}  & 1  & 2   &  0.5  & 0& 0   & N.A. &&  \tabincell{c}{ }  \\
%		\cline{3 - 10}
%		&   & 2  & 2   &  0.1 & 0 & 0  & N.A. & &  \tabincell{c}{  }  \\
%		\cline{3 - 10}
%		&  & 5  & 2   &0.4 &  -2 & 0 & N.A.  &  &  \tabincell{c}{ }  \\
%		\cline{3 - 10}
%		&  & 8  & 2    &0.6 & 1  &  0.08 &  N.A.& &  \tabincell{c}{  }  \\
%		\cline{3 - 10}
%		& & 10  & 2.5    & 0.1&  -1 &  -0.1&  N.A. &  & \tabincell{c}{ }  \\
%		\hline
	\end{tabular}
	} 
	\caption{Parameters by model for the \emph{Picard algorithm}}
	 \label{Parameters picard 1}
\end{table}


\begin{table}[htp]
	\centering
	\resizebox{\textwidth}{80mm}{
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c| c| } 
		\hline
		\multicolumn{1}{|c|}{\multirow{2}*{Examples}}& \multicolumn{1}{c|}{\multirow{2}*{Basis functions}}&  \multirow{2}*{ dim }& \multirow{2}*{ r }&  \multicolumn{3}{c|}{ \multirow{1}*{Initial value}}  & \multirow{2}*{ N } & \multirow{2}*{ p } & \multirow{2}*{ $\Gamma$ } \\
		 \cline{5-7}
		& &   & & $\mathfrak{y} $ & $ \mathfrak{z}^{0, \cdot} $ &  $\mathfrak{z}^{n, k}$  & & & \\
%		\hline
%		\multirow{4}*{\tabincell{c}{Limits to \\ Picard \\ algorithm}} & \multirow{4}*{Pre-wavelets}  &  \multirow{4}*{2}  &  \multirow{4}*{2}   & 0.3   & 0 & 0   & -0.4&  $1\le p \le 9$  &   \tabincell{c}{ (1, 0, 1, 300), \\ (1, 0, 1, 300),  \\ (1, 0.6, 0.1, 300) }  \\
%		\cline{5 - 10}
%		&   & &   &  0  &  0 & 0&  -1.5 & $1\le p \le 9$ &  \tabincell{c}{ (1, 0, 2, 300), \\ (1, 0, 1, 300),  \\ (1, 0.6, 0.1, 300)  }  \\
		\hline
		\multirow{25}*{\tabincell{c}{The \\challenging \\ example}} & \multirow{25}*{Hat}  & 1  & 2   &  0.5  & 0& 0   & 10 & $1\le p\le 5$ &  \tabincell{c}{(1, 0, $0.5*(0.8)^{p-1}$, 100), \\ (1, 0, 3$*(0.8)^{p-1}$, 100),  \\ (1, 0.1$*(0.8)^{p-1}$, 0.1$*(0.8)^{p-1}$, 100)  }  \\
		\cline{3 - 10}
		&   & 2  & 2   &  0.1 & 0 & 0  & 20 & $1\le p\le 5$ &  \tabincell{c}{  (1, 0, 0.5$*(0.8)^{p-1}$, 100), \\ (1, 0, 5$*(0.8)^{p-1}$, 100),  \\ (1, 0.2$*(0.8)^{p-1}$, 0.5$*(0.8)^{p-1}$, 100)  }  \\
		\cline{3 - 10}
		&  & 5  & 2   &0.4 &  -2 & 0 & 40  & $1\le p\le 5$ &  \tabincell{c}{ (1, 0, 0.5$*(0.8)^{p-1}$, 300), \\ (0.95, 0, 5$*(0.8)^{p-1}$, 500),  \\ (1, 0.2$*(0.8)^{p-1}$, 0.1$*(0.8)^{p-1}$, 500)}  \\
		\cline{3 - 10}
		&  & 8  & 2.2    &0.6 & 1  &  0.08 &  60 & $1\le p\le 5$&  \tabincell{c}{ (1, 0, 0.35$*(0.8)^{p-1}$, 500), \\ (1, 0, 5$*(0.8)^{p-1}$, 500),  \\ (1, 0.2$*(0.8)^{p-1}$, $(0.8)^{p-1}$, 500) }  \\
		\cline{3 - 10}
		& & \multirow{13}*{10}  & \multirow{13}*{2.5}    & \multirow{13}*{0.1} &  \multirow{13}*{-1} &  \multirow{13}*{-0.1} &  \multirow{13}*{100} & 1 & \tabincell{c}{(1, 0, 0.25, 500),     \\ (0.95, 0, 4, 500),     \\ (1, 0.15, 0.5, 500) }  \\
		\cline{9 - 10}
		& & &&&&&   &2  & \tabincell{c}{ (1, 0, 0.2, 500),    \\ (0.95, 0, 3, 500),     \\ (1, 0.12, 0.4, 500) }  \\
		\cline{9 - 10}
		& & &&&&&  &3  & \tabincell{c}{ (1, 0, 0.15, 500),    \\ (0.95, 0, 2, 500),     \\ (1, 0.1, 0.3, 500)  }  \\
		\cline{9 - 10}
		& & &&&&&   &  $p\ge 4$ & \tabincell{c}{  (1, 0, 0.1, 500),     \\ (0.95, 0, 1, 500),    \\  (1, 0.08, 0.25, 500)}  \\
		\cline{9 - 10}
		& & &&&&&  & $p\ge 6$  & \tabincell{c}{ (1, 0, 0.05, 500),    \\ (0.95, 0, 0.5, 500),   \\ (1, 0.05, 0.2, 500)}  \\
		\hline
	\end{tabular}
	} 
	\caption{Parameters by model for the \emph{Picard algorithm}}
	 \label{Parameters picard 2}
\end{table}
















==> v4.33 - arXiv submission/basecom.tex <==
%env


\newenvironment{bluetext}{\color{blue}}{\ignorespacesafterend}

%letters



%calligraphic
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

%mathbb
\newcommand{\E}{\mathbb{E}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\G}{\mathbb{G}}
\renewcommand{\P}{\mathbb{P}}
\renewcommand{\H}{\mathbb{H}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\renewcommand{\S}{\mathbb{S}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\Z}{\mathbb{Z}}
%?? shortcuts

\newcommand{\wh}[1]{\ensuremath{ \widehat{#1} }}

%deltas
\newcommand{\dZ}
    {\ensuremath{\delta Z }}
    
\newcommand{\dY}
    {\ensuremath{\delta Y }}

    
\newcommand{\dX}
    {\ensuremath{\delta X}}

%%%%%
%MATH
%%%%%%

%symbols

\def \proof{{\noindent \bf Proof. }}
\def \eproof{\hbox{ }\hfill$\Box$}

\newcommand{\ud}{\, \mathrm{d}}

\newcommand{\HYP}[1]
    {\ensuremath{({H#1} ) }}

\newcommand{\1}{{\bf 1}}
    
%spaces and norms

\newcommand{\set}[1]
    {\ensuremath{\{ #1 \}}}
    
\newcommand{\HP}[1] %L2DPDT sur 0,T
    {\ensuremath{\mathscr{H}^{#1}}}    

\newcommand{\NH}[2] 
    { \ensuremath{ \|#2\|_{\mathscr{H}^{#1}} } }

\newcommand{\SP}[1]{\ensuremath{\mathscr{S}^{#1}}}

\newcommand{\NS}[2]
    {\ensuremath{\|#2\|_{ \mathscr{S}^{#1} }}}
%proba

\newcommand{\esp}[1]{\ensuremath{\mathbb{E} \! \left[#1\right] }}
\newcommand{\espQ}[1]{\ensuremath{\mathbb{E}^\mathbb{Q} \left[#1\right] }}
\newcommand{\EFp}[2]
    {\ensuremath{% raccourci esperance conditionnelle discretisation
     \mathbb{E}_{#1}\!\!\left[#2\right] }}
     
%numerical analysis
\newcommand{\ti}[1]{t_{i #1}}
\newcommand{\tk}[1]{t_{k #1}}
\newcommand{\tj}[1]{t_{j #1}}

%\newcommand{\oldXi}{\Xi}
%\renewcommand{\Xi}[1]{X_{i #1}}
\newcommand{\Yi}[1]{Y_{i #1}}
\newcommand{\Zi}[1]{Z_{i #1}}

\newcommand{\yi}[1]{y_{i #1}}
\newcommand{\zi}[1]{z_{i #1}}
\newcommand{\whyi}[1]{\widehat{y}_{i #1}}
\newcommand{\whzi}[1]{\widehat{z}_{i #1}}

\newcommand{\tYi}[1]{\tilde{Y}_{i #1}}
\newcommand{\tZi}[1]{\tilde{Z}_{i #1}}
\newcommand{\wtYi}[1]{\widetilde{Y}_{i #1}}
\newcommand{\wtZi}[1]{\widetilde{Z}_{i #1}}
\newcommand{\whYi}[1]{\widehat{Y}_{i #1}}
\newcommand{\whZi}[1]{\widehat{Z}_{i #1}}
\newcommand{\whXi}[1]{\widehat{X}_{i #1}}
\newcommand{\whHi}[1]{\widehat{H}_{i#1}}


\newcommand{\whEFp}[2]
    {\ensuremath{%
     \widehat{\mathbb{E}}_{#1}\!\left[#2\right] }}
\newcommand{\whesp}[1]
    {\ensuremath{%
     \widehat{\mathbb{E}}\!\left[#1\right] }}

\newcommand{\dYi}[1]{\delta Y_{i #1}}
\newcommand{\dZi}[1]{\delta Z_{i #1}}
\newcommand{\dYj}[1]{\delta Y_{j #1}}
\newcommand{\dZj}[1]{\delta Z_{j #1}}
\newcommand{\dYk}[1]{\delta Y_{k #1}}
\newcommand{\dZk}[1]{\delta Z_{k #1}}


\newcommand{\Ui}[1]{U_{i #1}}
\newcommand{\ui}[1]{u_{i #1}}
\newcommand{\dUi}[1]{\delta U_{i #1}}
\newcommand{\dui}[1]{\delta u_{i #1}}
\newcommand{\dfi}[1]{\delta f_{i #1}}
\newcommand{\dfj}[1]{\delta f_{j #1}}
\newcommand{\Uj}[1]{U_{j #1}}
\newcommand{\uj}[1]{u_{j #1}}
\newcommand{\dUj}[1]{\delta U_{j #1}}
\newcommand{\dUk}[1]{\delta U_{k #1}}

\newcommand{\errYi}[1]{\zeta^{Y}_{i #1}}
\newcommand{\errZi}[1]{\zeta^{Z}_{i #1}}
\newcommand{\errYj}[1]{\zeta^{Y}_{j #1}}
\newcommand{\errZj}[1]{\zeta^{Z}_{j #1}}
\newcommand{\errYk}[1]{\zeta^{Y}_{k #1}}
\newcommand{\errZk}[1]{\zeta^{Z}_{k #1}}

\newcommand{\Hy}{\ensuremath{{}^Y \!\! H}}
\newcommand{\Hf}{\ensuremath{{}^f \! H}}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\essinf}{essinf}
\DeclareMathOperator{\Tr}{Tr}
\newcommand{\probcond}[2]{\P\left[#1 | #2\right]}

==> v4.33 - arXiv submission/convergence.tex <==
%!TEX root = main.tex



\subsection{Convergence  and complexity analysis for sparse grid approximations}
\label{se con and com analysis}

%
%\subsubsection{Sparse multilinear interpolation}
%
%\paragraph{Energy-based space grid approximation}\label{subsubsection 1.1.1}
%\textcolor{red}{some notations will have to change below...}
%
%Here, we work on sparse grids and approach the solution of (\ref{eq pde})  by hat functions if it is vanish on the boundary of compact set $ [0, 1]^d \in \mathbb{R}^d $, see the review paper by H.-J. Bungartz and M. Griebel \cite{bungartz2004sparse}, and the references therein. Namely, 
%\begin{align}\label{eq pres spgd first}
%\varphi(x) = \sum_{\textbf{l}} \sum_{\textbf{j} \in \textbf{I}_{\textbf{l}} } \theta^{\textbf{l,j}} \phi^{\textbf{l,j}}(x),  \quad x \in [0, 1]^d,
%\end{align}
%where $\textbf{l} =(l_1, l_2, \cdots, l_d) \in \mathbb{R}^d$ is the level of sparse grids for all the directions, and $\textbf{I}_{\textbf{l}} := \{ \textbf{j} \in \mathbb{N}^d: \textbf{1}\leq \textbf{j} \leq 2^{\textbf{l}} - \textbf{1}, \; j_k \; \text{odd  for} \; \forall 1\leq s \leq d \}$,  
%\begin{equation}\label{eq 0.6}
%	 \phi^{\textbf{l,j}}(x) = \prod\limits_{s=1}^{d}  \phi^{l_s,j_s}(x_s) = \prod\limits_{s=1}^{d}  \phi \left( \dfrac{x_s  - j_s  \cdot  h_{l_s}}{h_{l_s} } \right),
%\end{equation}
%\begin{equation} \label{eq 0.7}
%	 \phi(x)   =\left\{
%\begin{array}{rcl}
%1- |x|     &      & {if \; -1<x<1}\\
%0       &      & {otherwise\,,}
%\end{array} \right.
%\end{equation}
%\begin{equation}\label{eq 0.8}
%	h_{l_s} = \dfrac{1}{2^{l_s}}\,.
%\end{equation}
%However,  usually the solution of PDE (\ref{eq pde}) is not vanish on  $ \partial ( [0, 1]^d ) $. We just need modify the hat functions (\ref{eq 0.7}) close to the boundary by the following method(similar to the equation (2.16) of \cite{frommert2010efficient}),
%\begin{equation} \label{eq 1.7}
%	 \phi^{l_s,j_s}(x_s) :=\left\{
%\begin{array}{ll}
% 1 
%% - \phi(  \dfrac{x_s - j_s  \cdot  h_{l_s}}{h_{l_s} } ) \times  \epsilon   
%     & {if\; l_s=1\wedge j_s =1}\\
%\left\{
%\begin{array}{ll} 
% 1 - 2^{l_s -1} \cdot x  & \qquad\quad {if\; x\in [0 , 2h_{l_s } ] }\\
% 0 & \qquad\quad {otherwise}
%\end{array} \right\}
%        & {if \; l_s>1\wedge j_s =1}\\
%\left\{
%\begin{array}{ll} 
%  2^{l_s-1} \cdot x  + (1-j_s)/2 &  {if\; x\in [1 - 2 h_{l_s}, 1] }\\
% 0 &  {otherwise}
%\end{array} \right\}
%          &  {if\; l_s>1\wedge j_s = 2^{l_s} - 1}\\
%\phi(  \dfrac{x_s - j_s  \cdot  h_{l_s}}{h_{l_s} } )         & {otherwise\,,}
%\end{array} \right.
%\end{equation}
%%where $\epsilon$ is a small positive real number. 
%Now, we want to extend the definition of the solution  to all $\R^d$ but keeping the compact supports $ \Omega_n = [a^n, b^n]\in \mathbb{R}^d $ for all $n\le N-1$. We can use the affine functions to extend the equation (\ref{eq 1.7}) to $\Omega_i$ and some smooth functions to connect the boundary to 0 in some small intervals $ [a^n -\epsilon_0, a^n]  $ and $ [b^n, b^n+\epsilon_0] $. We define the new scale 
%\begin{equation}
%	h_{l_s, n} = \dfrac{b_s^n -a_s^n}{2^{l_s}}, \quad n\le N-1,
%\end{equation}
%and for $n\le N-1$,
%\begin{align}\label{eq de fonction}
%\varphi_n(x) = \sum_{\textbf{l}} \sum_{\textbf{j} \in \textbf{I}_{\textbf{l}} } \theta_n^{\textbf{l,j}} \phi_n^{\textbf{l,j}}(x) = \sum_{\textbf{l}} \sum_{\textbf{j} \in \textbf{I}_{\textbf{l}} } \theta_n^{\textbf{l,j}} \prod\limits_{s=1}^{d}  \phi_n^{l_s,j_s}(x_s) ,  \quad x \in  \mathbb{R}^d ,
%\end{align}
%where 
%\begin{equation}\label{eq de basic functions}
%	\phi^{l_s,j_s}_n(x_s) :=\left\{
%\begin{array}{ll}
%	\phi^{l_s,j_s}\left( \dfrac{ x_s -  \textcolor{red}{+?}a_s^n}{ b_s^n - a_s^n}  \right)    & {if\; x_s \in [a_s^n, b_s^n]} \\
%	 p^{l_s,j_s}_n(x_s) & {if\; x_s \in  [a_s^n -\epsilon_0, a_s^n] }\\
%	 q^{l_s,j_s}_n(x_s) & {if \; x_s \in [b_s^n, b_s^n + \epsilon_0]} \\
%	 0 & {otherwise\,,}
%\end{array} \right.
%\end{equation}
%the functions $  p^{l_s,j_s}_n(x_s),  q^{l_s,j_s}_n(x_s) $ are continuous and $ p^{l_s,j_s}_n(a_s^n - \epsilon_0 ) = q^{l_s,j_s}_n(b_s^n + \epsilon_0 ) = 0,  p^{l_s,j_s}_n(a_s^n) =  q^{l_s,j_s}_n(b_s^n)=1 $. Therefore, the space $\mathscr{E}_n $ can be built as
%\begin{equation}
%	\mathscr{E}_n = \left\{\varphi_n \in \cW^{2,2}\;  \bigg| \;\varphi_n(x) = \sum_{\textbf{l}} \sum_{\textbf{j} \in \textbf{I}_{\textbf{l}} } \theta_n^{\textbf{l,j}} \phi_n^{\textbf{l,j}}(x), x\in \mathbb{R}^d  \right\}, \quad n\le N-1\,.
%\end{equation}
%In practice, we work on the space $\mathscr{E}_n^\ell $ and reorder these basic functions,
%\begin{equation}
%	\mathscr{E}_n^\ell = \left\{\varphi_i \in \cW^{2,2}\;  \bigg| \;\varphi_n(x) = \sum_{\textbf{l} \in  J(\mathbf{\ell_i}) } \sum_{\textbf{j} \in \textbf{I}_{\textbf{l}} } \theta_n^{\textbf{l,j}} \phi_n^{\textbf{l,j}}(x) = \sum_{k=0}^{K_n}  \theta_n^k \phi_n^k(x) ,  \;x\in \mathbb{R}^d   \right\} \subset \mathscr{E}_n,
%\end{equation}
%\textcolor{magenta}{
%where $ \mathbf{\ell_n}:=(\ell_n, \cdots, \ell_n )\in \mathbb{R}^d$ is the max level of the sparse grids that we used, $K_i$ is number of the points of the sparse grids at time $t_{n}$.  and 
%\begin{align}\label{condition to l}
%	J(\mathbf{\ell}) := \left\{
%	\begin{array}{ ll }
%		\{\textbf{l} \in \mathbb{R}^d \; | \; \textbf{l}_j \le \ell, \quad \forall 1\le j\le d \} & {\text{full grids}} \\
%		\{ \textbf{l} \in \mathbb{R}^d \;|\; | \textbf{l} |_1 \le \ell +d -1 \} & {\text{sparse grids}} \\
%		\left\{  \textbf{l} \in \mathbb{R}^d \; \bigg| \; |\textbf{l}|_1 \leq (\ell +d-1) +  \frac{1}{5} \cdot \log_2 \left(\dfrac{ \sum_{j=1}^d 4^{l_j} }{4^\ell +4d-4} \right) \right\} & {\text{energy sparse grids}} \\
%	\end{array}
%	\right.
%\end{align} 
%} 
%%\begin{bluetext}
%We have $ \partial_x \phi^1_n(x) \equiv (0, 0, \cdots, 0)  $ since $  \phi^1_n(x) =\prod_{s=1}^{d} \phi^{1,1}(x_s) \equiv 1  $ for modified hat functions. The class $\cC^\pi$ is thus parametrized by the vectors $\Theta=(\theta^k_n)_{1 \le k \le K_n, 0 \le n \le N-1} \in \R^{1+\sum_{n=1}^{N-1} K_n }$. For latter use, we set $\bar{K}:=\sum_{n=0}^{N-1}K_n $. Note that $K_0=1$, so that
%$\theta^1_0 \in \R$ simply as  at the initial condition there is no randomness.   Then, we rewrite, for $\varphi \in \cE_n$,
%$$ \partial_x\varphi_n(x) = \sum_{k=0}^{K_n} \theta^k_n \partial_x \phi^k_n(x) = \sum_{k=1}^{K_n} \theta^k_n \partial_x \phi^k_n(x) .$$
%\\



%\subsection{Error analysis}

%\subsubsection{Preliminary estimates}

For this part, we work in the setting of Section \ref{subse picard periodic}. Our goal is to prove the theoretical upper-bound on the algorithm's complexity stated in Theorem \ref{thm full complexity}. 

%\begin{bluetext}
%\noindent From the above result, 

\vspace{2mm}
\noindent We first state the following useful estimate.
\begin{Lemma}\label{le main estimate for frame}
Suppose that Assumption \ref{ass periodic} is satisfied. Let $\phi:\R^d \rightarrow \R$ be a non-negative measurable function whose support is included in $\cO$ and $\widecheck{\phi}$ be its $1$-\emph{periodisation} defined by \eqref{eq de one periodisation}. Then, it holds
\begin{align*}
\mathfrak{C}^{-1}\esp{\phi(U)} \le \esp{\widecheck{\phi}(X_{t_n})} = \esp{\phi(\widehat{X}_{t_n})} \le \mathfrak{C} \esp{\phi(U)}
\end{align*}
where $U$ has law $\cU((0,1)^d)$ and $\mathfrak{C}$ is given in Lemma \ref{Aronson:two:sided:bounds}.
\end{Lemma}


\proof
We denote by $x' \mapsto p_X(t_n, x')$ the density function of $X_{t_n}$ given by the Euler-Maruyama scheme taken at time $t_n$ and starting from $\cX_0$ with  law $\cU((0,1)^d)$ at time $0$. Note that we have
$p_X(t_n,x') = \int p^{\pi}(0, t_n, x, x') \1_{(0,1)^d}(x) \ud x $ and using
\eqref{Aronson:bounds:transition:density},
\begin{align*}
\mathfrak{C}^{-1} \int p(\mathfrak{c} t_n, x - x')\1_{(0,1)^d}(x) \ud x  \leq p_X(t_n,x') \leq \mathfrak{C} \int p(\mathfrak{c} ^{-1}t_n, x'-x) \1_{(0,1)^d}(x) \ud x \,.
\end{align*}
Then,
\begin{align*}
 \esp{\phi(\widehat{X}_{t_n})} &= \esp{\widecheck{\phi}(X_{t_n})}  \ge \mathfrak{C}^{-1} \int \widecheck{\phi}(x')\int p(\mathfrak{c}  t_n, x - x')\1_{(0,1)^d}(x)\ud x \ud x'
 \end{align*}
 so that introducing the notation $\Xi = \xi + W_{ \mathfrak{c}  t_n}$,
\begin{align}
\int \widecheck{\phi}(x')\int p(\mathfrak{c}  t_n, x - x')\1_{(0,1)^d}(x)\ud x \ud x' &= \esp{\widecheck{\phi}(\Xi)}
%\\
%&
= \esp{{\phi}(\widehat{ \Xi})}
 \end{align}
 The proof is then concluded by observing that $\cL(\widehat{\Xi}) = \cL(U)$. The proof of the upper-bound follows from similar arguments.
\eproof

%\end{bluetext}

%
%\subsubsection{Discrete time error}
%Let us first observe that the discrete time approximation error is now well understood for SDEs and BSDEs.
%We shall use the following result,  see e.g. Ma and Zhang \cite{ma2002path} and Pag\`es \cite{pages2018numerical}.
%\begin{Lemma}\label{le disc time error}
%Assume that the coefficients $f$, $g$, $b$, $\sigma$ are Lipschitz-continuous. Then, it holds
%\begin{align*}
%\cE_{\pi} :=  \esp{ \sum_{n=0}^{N-1}  \int_{t_{n}}^{t_{n+1}}\left( |\cY_s-\cY_{t_{n}}|^2 + |\cZ_s-\cZ_{t_{n}}|^2 + |\cX^{x_0}_{t_{n+1}} - X^{x_0}_{t_{n+1}}|^2 \right)ds } 
%\le C |\pi|\,,
%\end{align*}
%where $\pi$ is a time grid of the interval $[0,T]$, with $|\pi| = h$.
%	\end{Lemma}


%\subsubsection{space}

\subsubsection{Sparse grid approximation error}

\noindent We now provide some upper-bound estimates for the sparse grid approximation error.

% For later use, we introduce a so-called \emph{reference solution} $(\bar{y},\bar{\Theta})$ 
%Then, we set $\bar{\cZ} := Z^{\bar{\Theta}}$, recall \eqref{eq de Z Psi}. The goal of this section is to understand the following error
%\begin{align}\label{de SG error}
%\cE_{\mathrm{SG}} := \sum_{n=0}^{N-1}h\esp{|\bar{\cZ}_{t_n}-\cZ_{t_n}|^2} = \sum_{n=1}^{N-1}h\esp{|\bar{\cZ}_{t_n}-\cZ_{t_n}|^2}
%\end{align}
%recalling the definition of $\cZ_0$.

\begin{Theorem} \label{th main sg error}
Under Assumption \ref{ass periodic}, there exists a positive constant $C:=C(T, b, \sigma, d, \lambda_0)$ such that %\textcolor{red}{$c:=c(b, \sigma, d, \lambda_0) \in (0,1]$} such that
\begin{align}
\cE_{\psi} \le C 2^{-4\ell} \ell^{d-1}.
\end{align}
%\noindent where we introduced the notation $\mathrm{A}(a) := \exp(-a^2/2)/a$. Moreover, if one sets 
%\begin{align*}
%$
%\textcolor{red}{a = \sqrt{\mathfrak{c} \ell }  \text{ with } \mathfrak{c} = 8\log(2)/c}
%$
%%\end{align*}
%then it holds
%\begin{align*}
%\cE_{\psi} \le C  2^{-4\ell}\ell^{\frac{7d-2}{2}}.% \text{ with } q_d = \frac92d - 2\;.
%\end{align*}
\textcolor{black}{
To obtain an error of order $\varepsilon^2$ for the quantity $\cE_{\psi}$ one may thus set $\ell_\varepsilon = \log_2(\varepsilon^{-\frac12}|\log_2(\varepsilon)|^{\frac{d-1}{ 4 }})$ so that, for each $n=1, \cdots, N-1$, the number of basis functions required satisfies
\begin{align*}
%\textcolor{red}{???
K_\varepsilon = \varepsilon^{-\frac12}|\log_2(\varepsilon)|^{  \frac{5(d-1)}4 }.
%}
\end{align*}
}
\end{Theorem}
%\begin{Remark}
%If $\mathfrak{c}\ell < 1$ above then we have the better bound $\cE_{\psi} \le C 2^{-4\ell} \ell^{d-1} $.
%\end{Remark}
\proof %\textcolor{red}{sketch of proof: missing approx at time 0 of y! and the question of $z$ as well}
%Using \eqref{eq error approx space}, we have that
%\begin{align*}
%\cE_{\psi} 
%%&= \inf_{\theta \in (\R^d)^{\bar{K}}}\sum_{n=0}^{N-1} h\esp{|\cZ_{t_n}-Z^\theta_{t_n}|^2}
%%\\
%&\leq h \sum_{n=1}^{N-1} \inf_{\theta_n \in \R^{d K}}\esp{|(\sigma^\top\nabla_x u)(t_n,X^{x_0}_{t_n})-Z^\upsilon_{t_n}|^2}
%\\
%&\quad\quad\quad+ h \sum_{n=1}^{N-1}\esp{|(\sigma^\top\nabla_x u)(t_n,X^{x_0}_{t_n})|^2\1_{\set{X^{x_0}_{t_n } \notin \cO_n }}} \\
%& =: A_1 + A_2.
%\end{align*}
%We treat the two terms separately.\\
%\noindent \emph{Step 1: Upper-bound for $A_1$.}
%\begin{bluetext}
 For $1 \le i \le d$, $n=0, \cdots, N-1$, setting $v_i(t_n, x) = (\sigma^{\top}\nabla_x u)_i(t_n, x)\1_{\set{x \in \cO}}$, $x \in \mathbb{R}^d$, from \eqref{bound:multi:indices:derivatives:pde:solution} we have
 \begin{align}\label{eq bound hmix}
 \|u\|_{H^{k}_{mix}(\mathcal{O})} + \max_{1 \le i \le d}\|v_i\|_{H^{k}_{mix}(\mathcal{O})} \le C.
 \end{align}
 Moreover, from \eqref{identity:periodic:function:euler:scheme}, we obtain
 \begin{align*}
 (\sigma^\top\nabla_x u)_i(t_n,X_{t_n}) = v_i(t_n, \widehat{X}_{t_n})\,,
 \end{align*}
 thus
\begin{align*}
\esp{|(\sigma^\top\nabla_x u)(t_n,X_{t_n})-Z^{\mathfrak{u}}_{t_n}|^2} & =  \sum_{i=1}^d  \esp{\Big|v_i(t_n, \widehat{X}_{t_n}) - \sum_{k=1}^{K}\mathfrak{z}^{n, k}_i \psi^{k}_{n}(\widehat{X}_{t_n})\Big|^2} 
\\
&\le \mathfrak{C} \sum_{i=1}^d  \esp{\Big|v_i(t_n, U) - \sum_{k=1}^{K}\mathfrak{z}^{n, k}_i \psi^{k}_{n}(U)\Big|^2} 
\end{align*}
\noindent with $U\sim \mathcal{U}((0,1)^d)$ and where we use the upper-estimate given in Lemma \ref{le main estimate for frame} to obtain the last inequality.
We also recall that
\begin{align}
\esp{|u(0,\cX_0)-Y^{\mathfrak{u}}_0|^2} = \esp{|u(0,U) - \sum_{k=1}^{K}\mathfrak{y}^k \psi^k_y(U)|^2} \,.
\end{align}

\noindent From \eqref{eq error approx space brut} and the previous estimates, we thus deduce
\begin{align}
\cE_{\psi}  &\le C\left(
\inf_{\xi \in \mathscr{V}^y} \|\xi-u(0, .)\|^2_{L^2(\cO)} 
+
 \max_{0 \le n \le N-1} 
\sum_{i=1}^d\inf_{\xi \in \mathscr{V}^z_n} \|\xi-v_{i}(t_n, .)\|^2_{L^2(\cO)} 
\right) \,,
\nonumber \\
%&\le 
%  C \max_{1 \le n \le N-1} 2^{-4\ell} \ell^{d-1}
%  \sum_{\mathbf{j}\in \mathbf{J}^\infty_{d,2}} 
%a^{2|\mathbf{j}|_1+d} \sum_{i=1}^d|D^{\mathbf{j}}v_i^n(t_n, .)|^2_\infty \nonumber \\
%&\le
%  C (1\vee a)^{5d}\max_{1 \le n \le N-1} 2^{-4\ell } \ell^{d-1}
%  \sum_{\mathbf{j}\in \mathbf{J}^\infty_{d,2}} 
% \sum_{i=1}^d|D^{\mathbf{j}}v_i^n(t_n,.)|^2_\infty \nonumber \\
 & \leq C 2^{-4\ell} \ell^{d-1}, \label{eq control A1}
\end{align}
where for the last inequality we used \eqref{eq control sparse basic} and \eqref{eq bound hmix}.
\\
Finally, setting $\ell_\varepsilon = \log_2(\varepsilon^{-\frac12}|\log_2(\varepsilon)|^{\frac{d-1}{ \textcolor{black}{4} }})$ yields $\cE_\psi = O(\varepsilon^2)$ as $\varepsilon \downarrow 0$
and from \eqref{eq dim approx space} (see also Remark \ref{re indexation}) we deduce that in this case
$K_\varepsilon = \varepsilon^{-\frac12}|\log_2(\varepsilon)|^{  \frac{5(d-1)}4 }$.
%\end{bluetext}
%
%\noindent \emph{Step 2: Upper-bound for $A_2$.} Using again the Gaussian upper-estimate \eqref{Aronson:bounds:transition:density} for the transition density of the Euler scheme
%\textcolor{magenta}{ 
%\begin{align}\label{eq 1.10}
%	\esp{\mathbbm{1}_{\left\{X^{x_0}_{t_n} \notin  \cO_n \right\}} } &= \mathbb{P}( X^{x_0}_{t_n} \notin  \cO_n  )   = 1 - \mathbb{P}( X^{x_0}_{t_n} \in  \cO_n  ) = 1 - \prod_{s=1}^d  \mathbb{P}( X^{x_0, s}_{t_n} \in  \cO_n^s  )   = 1 - (\Xi(a\sqrt{c}) )^d 
%\end{align}
%\noindent where $\Xi(x) := \displaystyle{\int_{-x}^{x} \dfrac{1}{\sqrt{2\pi} }e^{-\frac{t^2}{2} } dt }$. By Komatsu's inequality, see e.g. \cite{ito2012diffusion}, we derive
%%\[ \forall x \in \mathbb{R}^{+}, \qquad \dfrac{2}{x+\sqrt{x^2+4}} < e^{x^2/2} \int_{x}^{\infty} e^{-t^2/2}dt < \dfrac{2}{x+\sqrt{x^2+2}} \,,\]
%%In fact, the equality on the left is true for $\forall x \in \mathbb{R}$. In \cite{szarek1997confidence}, the authors sharpened the inequality on the right to become 
%%\[ \forall x>-1, \qquad e^{x^2/2} \int_{x}^{\infty} e^{-t^2/2}dt < \dfrac{4}{3x+\sqrt{x^2+8}}.  \]
%\begin{equation}\label{ineq Komatsu}
%\frac{	1 - \Xi(a\sqrt{c})}{2} = \displaystyle{\int_{a\sqrt{c}}^{\infty} \dfrac{1}{\sqrt{2\pi} }e^{-\frac{t^2}{2} } dt }  \leq \dfrac{1}{\sqrt{2\pi}}  \frac{2 \exp(-ca^2/2)}{a \sqrt{c}+\sqrt{a^2 c+2}} \leq  \dfrac{1}{\sqrt{2\pi}}  \dfrac{\exp(-ca^2/2)}{a\sqrt{c}}.
%\end{equation}
%Then
%\begin{equation}
%	(\Xi(a\sqrt{c}))^d \geq (1 - A(a\sqrt{c}))^d \geq 1 - d A(a\sqrt{c})
%\end{equation}
%\\ 
%Under Assumption \ref{assumption:coefficient}, the map $\sigma^{\top}\nabla_x u: [0,T] \times \mathbb{R}^d \longmapsto \mathbb{R} $ is bounded so that using (\ref{eq 1.10})-(\ref{ineq Komatsu}), we eventually deduce
%\begin{align}\label{eq 1.13}
%	%\begin{split}
%		A_2 \leq T \max_{1 \leq n \leq N-1} \esp{ |(\sigma^{\top}\nabla_x u)(t_n,X^{x_0}_{t_n}) |^2 \mathbbm{1}_{\left\{X^{x_0}_{t_n} \notin  \cO_n \right\} } } 	& \le C \mathbb{P}( X^{x_0}_{t_n} \notin  \cO_n  ) 
%		%  \esp{\mathbbm{1}_{W^x_{t_n} \notin  \Omega_n }}^\frac{1}{2}\\
%	 \leq  C \mathrm{A}(a\sqrt{c} ).
%	%\esp{1+|W^x_{t_n}|^{4\beta }}^\frac{1}{2} \\
%	%&:= c_2   (2\Phi^C(a) )^\frac{d}{2}  \lambda(x, t_n) \,,
%	%\end{split}
%\end{align}
%}
%
%\noindent \emph{Step 3: Conclusion.} The other statements follow from standard computations recalling \eqref{eq dim approx space}.
%
\eproof
%\left(\sum_{\mathbf{j}\in \mathbf{J}^\infty_d} 
%(a\sqrt{t_n})^{2|\mathbf{j}|_1+d} |D^{\mathbf{j}}v|_\infty
%+
%\sum_{\mathbf{j}\in \mathbf{J}^2_d} 
%(a\sqrt{t_n})^{2|\mathbf{j}|_1} |D^{\mathbf{j}}v|_2
%\right)
%\end{bluetext}

%
%
%\textcolor{red}{things have to change below...\\}
%%\noindent Assume $(\bar{y}_0, \bar{\cZ})$ is the theoretical discrete approximation of $(\cY_0, \cZ)$ built via the energy sparse grid approximation of $u$. 
%Denote$\bar{Y}_t^{\bar{y}_0, \bar{\cZ}} = \hat{u}(t, W_t^x) $ and $\bar{\cZ}_t = \partial_x \hat{u}(t,W^x_{t}) $, then
%\begin{align} \label{eq space error}
%\max_{n> 0} \esp{\|\cZ_{t_{n}} - \bar{\cZ}_{t_{n}} \|^2}^\frac12  \le C_0 \max_{n> 0}  \| \bar{u}(t_{n}, W^x_{t_{n}} ) - u(t_{n},  W^x_{t_{n}}  ) \|_{E, \mathbb{R}^d}  \;,
%\end{align}
%%This last term is related to the quality of approximation on the basis $(\phi^k)$. This can be optimised and the error that appears naturally is linked to an energy norm.\\
%%\\
%%A first "basic" approach would be to use sparse grid build to optimise error in terms of the energy norm, see \cite{bungartz2004sparse}.\\
%%\\
%where the constant $C_0 = \max\limits_{n>0} \dfrac{1}{ \sqrt{(2\pi)^d | \Sigma |} } $, $\Sigma$ is the covariance matrix of $W_{t_{n}}^x$, and $ \| u \|_{E, \Omega}  $ is the energy-based semi-norm on space $ \Omega $, it  is defined by
%\begin{align*}
%\| u \|_{E, \Omega} := \left(\int_\Omega \sum_{j=1}^d |\partial_{x_j} u|^2 \ud x \right)^\frac12.\;
%\end{align*}
%%which is very close to the quantities appearing in \eqref{eq space error}.
%%The Lebesgue measure being replaced by the gaussian one.
%%\\
%%To control this term, we can truncate the path of BM or maybe even build better approx using the energy norm with gaussian weight and the sparse grid paradigm...\\
%
%On the $d$-dimensional space $\mathbb{R}^d$, we consider multivariate functions $u, u(\textbf{x}) \in \mathbb{R}, \textbf{x} :=(x_1, \cdots, x_d) \in  \Omega \subseteq \mathbb{R}^d$,  with bounded weak mixed derivatives
% \begin{align*}
%	D^{\boldsymbol{\alpha} }u := 	\dfrac{\partial^{|\boldsymbol{\alpha}|_1} u}{\partial x_1^{\alpha_1}\cdots \partial x_d^{\alpha_d}}
%\end{align*}
%for $ |\boldsymbol{\alpha}|_\infty \le r \in \mathbb{N} $, where $ \boldsymbol{\alpha} \in \mathbb{N}^d$ denotes a $d$-dimensional multi-index with two norms 
%\[ |\boldsymbol{\alpha}|_1 := \sum_{j=1}^d \alpha_j \quad and \quad |\alpha|_\infty := \max_{1\leq j \leq d} \alpha_j  \]
%\\
%
%We study the spaces 
%\begin{align*}
%	X^{2, r}(\Omega) := \{u: [0, T] \times \Omega \rightarrow \mathbb{R}: D^{\boldsymbol{\alpha}}u \in L_2(\Omega), |\alpha|_\infty \leq r \},
%\end{align*}
%and
%\begin{align*}
%	X_0^{2, r}(\Omega) := \{u\in X^{2, r}(\Omega) : u(t, x) = 0 \; \text{for} \; \forall (t, x) \in [0, T] \times \partial\Omega  \}.
%\end{align*}
%
%
%Finally, we introduce the semi-norm
%\begin{align*}
%	|u|_{\boldsymbol{\alpha}, \infty}^{\Omega}:= ||D^{\boldsymbol{\alpha}} u ||_{\infty, \Omega} = \max_{\Omega} |D^{\boldsymbol{\alpha}} u|\,.
%\end{align*}
%
%\begin{Theorem} \label{thm 1}
%	For $\forall u(t, x) \in X_0^{2, 2}(\Omega_t )$, suppose that $\Omega_t = [ - a \sqrt{t}, a \sqrt{t} ]^d + x, a\in \mathbb{R}^+, d\in \mathbb{N}^+, x\in \mathbb{R}^d $ ,  then
%	\begin{equation}
%		|| \bar{u}(t, \cdot) - u(t, \cdot)||_{E, \Omega_t} \leq   (2a\sqrt{t})^\frac{5d}{2}  C_1(d) |u|_{\textbf{2},\infty}^{\Omega_t} \cdot 2^{-\ell}, \quad \forall t \in [0, T],
%	\end{equation}
%	where $C_1(d) = \dfrac{d}{3^{(d-1)/2} 4^{d-1}} \cdot \left(\frac{1}{2} + \left(\frac{5}{2}\right)^{d-1}\right)$,  $\ell$ is the max level of the energy-based  sparse grids, $\bar{u}(t, \cdot) = \sum\limits_{\textbf{l} \in J(\ell) }\sum\limits_{j\in \textbf{I}_{\textbf{l}}} \theta_n^{\textbf{l,j}} \phi_n^{\textbf{l,j}}(\cdot), \; \forall t\in [t_n, t_{n+1} ), 0\leq n\leq N-1$, $J(\ell)$ is the set defined for energy-based sparse grids in (\ref{condition to l}),   $\phi_n^{\textbf{l,j}}(\cdot) $ are hat functions on the space $\Omega_{t_n} $ defined by (\ref{eq 0.6}), (\ref{eq 0.7}) and (\ref{eq 0.8}).
%\end{Theorem}
%\proof
%From the theorem 3.10 of \cite{bungartz2004sparse}, the energy norm of the interpolation error of $u(t, \cdot) \in  X_0^{2, 2}([0, 1]^d )$ in the energy-based sparse grid space is bound by 
%\begin{equation}
%	||\bar{u}(t, \cdot) - u(t, \cdot)||_{E, [0,1]^d} \le \dfrac{d\cdot |u|_{\textbf{2}, \infty}^{[0,1]^d}}{3^{(d-1)/2} 4^{d-1}} \cdot \left(\frac{1}{2} + \left(\frac{5}{2}\right)^{d-1}\right) \cdot 2^{-\ell} =C_1(d)  |u|_{\textbf{2}, \infty}^{[0,1]^d} 2^{-\ell} = O(2^{-\ell})\,,
%\end{equation}
%%where $\textbf{l}$ s.t. $|\textbf{l}|_1 - \frac{1}{5} \cdot \log_2 (\sum_{j=1}^d 4^{l_j} ) \leq (n+d-1) - \frac{1}{5} \cdot \log_2 (4^n +4d-4)$. \\
%And by the lemma 3.9 of \cite{bungartz2004sparse}, the sparse grid space $V_\ell^{(E)}$ is a subspace of $V_\ell^{(1)}$, its dimension fulfils 
%\[ |V_\ell^{(E)}| \leq 2^\ell \cdot \dfrac{d}{2} \cdot e^d = \cO(2^\ell)\,. \]
%So the $\epsilon-complexity$ $\ell(\epsilon) = O(\epsilon^{-1})$.  Thus, for a fixed number of $N$ of grid points, the following accuracy can be obtained: $\epsilon(\ell) = \cO(\ell^{-1})$.\\
%
%
%Let $g(y) = \partial_y(\bar{u} - u )(t, y)$ and $ y = a\sqrt{t}(2z-1)+x,\; z\in [0,1] $, then
%\begin{equation}
%	\begin{split}
%		 &\quad || \bar{u}(t, y) - u(t, y)||_{E, \Omega_t} \\
%		&= \left(\int_{\Omega_t} ||\partial_y(\bar{u} - u )(t, y)||_2^2 dy\right)^\frac{1}{2} \\
%		& =  \left(\int_{\Omega_t} ||g(y)||_2^2 dy\right)^\frac{1}{2} \\
%		& = \left(\int_{[0,1]^d}  ||g(a\sqrt{t}(2z-1)+x)||_2^2 (2a\sqrt{t})^d dz \right)^\frac{1}{2} \\
%		&=  (2a\sqrt{t})^\frac{d}{2} ||\bar{u}(t, a\sqrt{t}(2z-1)+x) - u(t, a\sqrt{t}(2z-1)+x)||_{E, [0,1]^d} \\
%		& = (2a\sqrt{t})^\frac{d}{2} ||\bar{v}(t, z) - v(t, z)||_{E, [0,1]^d} \\
%		&\le (2a\sqrt{t})^\frac{d}{2}  C_1(d) |v|_{\textbf{2},\infty}^{[0,1]^d} \cdot 2^{-n} \\
%		&  = (2a\sqrt{t})^\frac{5d}{2}  C_1(d) |u|_{\textbf{2},\infty}^{\Omega} \cdot 2^{-n}\,,
%	\end{split}
%\end{equation}
%since
%\begin{equation}
%\begin{split}
%		|v(t, z)|_{\textbf{2},\infty}^{[0,1]^d}  &= |u(t, a\sqrt{t}(2z-1)+x)|_{\textbf{2},\infty}^{[0,1]^d} \\
%		& = \max_{z \in [0, 1]^d} \dfrac{\partial^{2d} u(t, a\sqrt{t}(2z-1)+x) }{\partial z_1^2 \cdots \partial z_d^2 }\\
%		& = \max_{y\in \Omega_t} \; \dfrac{\partial^{2d} u(t, y) }{\partial y_1^2 \cdots y_d^2 } \cdot \left(\dfrac{\partial^2 y_1}{\partial z_1^2} \cdots   \dfrac{\partial^2 y_d}{\partial z_d^2} \right) \\
%		& = (2a\sqrt{t})^{2d} |u|_{\textbf{2},\infty}^{\Omega_t}\,,
%\end{split}
%\end{equation}
%where $v(t, z) = u(t, a\sqrt{t}(2z-1)+x) \in X_0^{2, 2}([0, 1]^d ) $ and $\bar{v}(t, z) =  \bar{u}(t, a\sqrt{t}(2z-1)+x) $.\\
%\eproof
%\\
%
%\begin{Theorem}\label{thm 1.3}
%	The energy norm of the interpolation error of some $u \in X^{2, 2}([0,1]^d)$ in the energy-based sparse grid space $ V_\ell^{(E)} $ is bounded by 
%	\begin{equation}
%		|| u - u_\ell^{(E)}||_{E, [0,1]^d} \le C_2(d)  \max_{\boldsymbol{0}\le \boldsymbol{\alpha} \le \boldsymbol{2} } |u|_{\boldsymbol{\alpha} , \infty}^{[0,1]^d}\cdot  2^{-\ell} = \cO(2^{-\ell})
%	\end{equation}
%	where $C_2(d) = 40d \cdot \left( \frac{100}{3}\right)^{(d-1)/2}  \cdot \left(\frac{1}{2} + \left(\frac{5}{2}\right)^{d-1} \right) $,  $\ell$ is the max level of the sparse grids, $ u_\ell^{(E)} = \sum\limits_{\textbf{l}\in J(\ell)}\sum\limits_{j\in \textbf{I}_{\textbf{l}}} \theta^{\textbf{l,j}} \phi^{\textbf{l,j}}(\cdot), $$J(\ell)$ is the set defined for energy-based sparse grids in (\ref{condition to l}),  $ \phi^{\textbf{l,j}}(\cdot) $ are the modified hat functions on the space $ [0, 1]^d $ defined by (\ref{eq 1.7}) and (\ref{eq 0.6}).
%\end{Theorem}
%\proof
%Please find the proof in the appendix.\\
%\eproof
%\\
%\begin{Theorem} \label{thm 1.2}
%	For $\forall u(t, x) \in X^{2, 2}(\Omega_t )$, suppose that $\Omega_t = [ - a \sqrt{t}, a \sqrt{t} ]^d + x, a\in \mathbb{R}^+, d\in \mathbb{N}^+, x\in \mathbb{R}^d $ ,  then
%	\begin{equation}
%		|| \bar{u}(t, \cdot) - u(t, \cdot)||_{E, \Omega_t} \leq    (2a\sqrt{t})^{\frac{d}{2}+ |\overline{\boldsymbol{\alpha} }|_1 }  C_2(d) |u|_{\overline{\boldsymbol{\alpha}} ,\infty}^{\Omega_t} \cdot 2^{-\ell }, \quad \forall t \in [0, T],
%	\end{equation}
%	where $C_2(d) = 40d \cdot \left( \frac{100}{3}\right)^{(d-1)/2}  \cdot \left(\frac{1}{2} + \left(\frac{5}{2}\right)^{d-1} \right) $, $ \overline{\boldsymbol{\alpha} } = \arg \max\limits_{\boldsymbol{0}\le \boldsymbol{\alpha} \le \boldsymbol{2} } |u|_{\boldsymbol{\alpha} ,\infty}^{\Omega_t}   $,  $\ell$ is the max level of the sparse grids, $\bar{u}(t, \cdot) = \sum\limits_{\textbf{l}\in J(\ell)}\sum\limits_{j\in \textbf{I}_{\textbf{l}}} \theta_n^{\textbf{l,j}} \phi_n^{\textbf{l,j}}(\cdot), \; \forall t\in [t_n, t_{n+1} ), 0\leq n\leq N-1,  $$J(\ell)$ is the set defined for energy-based sparse grids in (\ref{condition to l}), $\phi_n^{\textbf{l,j}}(\cdot) $ are modified hat functions on the space $\Omega_{t_n} $ defined by (\ref{eq 0.6}) and (\ref{eq de basic functions}).
%\end{Theorem}
%\proof
%It is easy to proof \Cref{thm 1.2} by \Cref{thm 1.3} with the same method of proving the \Cref{thm 1}.\\
%\eproof
%\\
%
%\begin{Theorem}\label{th main control error sparse grid}
%Assume $\partial_x u: [0,T] \times \mathbb{R}^d \longmapsto \mathbb{R} $ is an at most polynomially growing continuous function, 
%\begin{equation}\label{eq 1.12}
%	\partial_x  u(t_n,W^x_{t_n})  \le c_1 (1+ |W^x_{t_n}|^{\beta} ), \qquad \beta \in \mathbb{N}\,.
%\end{equation}
%And assume $ W^x_{t_n}  \sim \mathcal{N}(x, t_n I_d), \ell_n = \ell, \forall 1\le n\le N-1 $, let $\Omega_n = [ - a \sqrt{t_n}, a \sqrt{t_n} ]^d + x,  1\leq n \leq N-1 $, $ (\overline{\boldsymbol{\alpha} }, \bar{n}) = \arg \max\limits_{\boldsymbol{0}\le \boldsymbol{\alpha} \le \boldsymbol{2} \atop 1\le n \le N-1 }  |u|_{\boldsymbol{\alpha} ,\infty}^{\Omega_n}   $, then 
%\begin{equation}
%	\begin{split}
%		& \quad  \max_{n>0}  \esp{\| \cZ_{t_n} - \bar{\cZ}_{t_n} \|^2} =  \max_{n>0}  \esp{\|\partial_x \bar{u}(t_n,W^x_{t_n}) -\partial_x u(t_n,W^x_{t_n})\|^2}  \\
%		& \le C(\overline{ \boldsymbol{\alpha} }, \beta, d, T, x)  \left( (a)^{d+2|\overline{ \boldsymbol{\alpha} }|_1} ( |u|_{\overline{\boldsymbol{\alpha} } ,\infty}^{\Omega_{\bar{n}}})^2 \cdot 2^{-2\ell } + \Gamma(a, d) \right),  
%	\end{split}
%\end{equation}
%where $ \Gamma(a, d) :=  \left(e^{-\frac{a^2}{2}} \dfrac{1}{a} \right)^\frac{d}{2}   $, $ C(\overline{ \boldsymbol{\alpha} }, \beta, d, T, x) $ is a constant depend on the five fixed parameters. Then
%\begin{equation}
%	\begin{split}
%		&\quad h\sum_{n=1}^{N-1}\esp{\| \cZ_{t_n} - \bar{\cZ}_{t_n} \|^2}    =h \sum_{n=1}^{N-1} \mathbb{E}[ |\partial_x\bar{u}(t_n, W_{t_n}^x) - \partial_x u(t_n, W_{t_n}^x) |^2  ] \\
%%		& \le h |\partial_x\bar{u}(0,  x) - \partial_x u(0, x) |^2 + 
%		& \le  \dfrac{N-1}{N} \max_{1 \le n\le N-1} \mathbb{E}[ |\partial_x\bar{u}(t_n, W_{t_n}^x) - \partial_x u(t_n, W_{t_n}^x) |^2  ] \\
%%		&<  h |\partial_x \bar{u}(0,  x) - \partial_x u(0, x) |^2 +
%& \le   C(\overline{ \boldsymbol{\alpha} }, \beta, d, T, x)  \left( (a)^{d+2|\overline{ \boldsymbol{\alpha} }|_1} ( |u|_{\overline{\boldsymbol{\alpha} } ,\infty}^{\Omega_{\bar{n} }})^2 \cdot 2^{-2\ell } + \Gamma(a, d) \right).
%	\end{split}
%\end{equation}
%\end{Theorem}
%\proof
% For any $n\le N-1$, we have \\
%\begin{equation}\label{eq 1.8}
%	\begin{split}
%		& \quad  \esp{|\partial_x \bar{u}(t_n,W^x_{t_n}) -\partial_x u(t_n,W^x_{t_n})|^2} \\
%		& = \esp{|\partial_x \bar{u}(t_n,W^x_{t_n}) -\partial_x u(t_n,W^x_{t_n})|^2 \mathbbm{1}_{W^x_{t_n} \in \Omega_n } }  +  \esp{|\partial_x \bar{u}(t_n,W^x_{t_n}) -\partial_x u(t_n,W^x_{t_n})|^2 \mathbbm{1}_{W^x_{t_n} \notin  \Omega_n } } \\
%		& \le \dfrac{1}{\sqrt{(2\pi t_n)^d}} || \bar{u}(t_n, \cdot) - u(t_n, \cdot)||_{E, \Omega_n}^2 + \esp{ | \partial_x u(t_n,W^x_{t_n}) |^2 \mathbbm{1}_{W^x_{t_n} \notin  \Omega_n } }\,.
%	\end{split}
%\end{equation}
%For the first part, by the \Cref{thm 1.2}, we have 
%\begin{align}\label{eq 1.9}
%	\dfrac{1}{\sqrt{(2\pi t_n)^d}} || \bar{u}(t_n, \cdot) - u(t_n, \cdot)||_{E, \Omega_n}^2 \leq \dfrac{1}{\sqrt{(2\pi t_n)^d}}   (2a\sqrt{t_n})^{d + 2| \overline{\boldsymbol{\alpha} } |_1 }  C_2(d)^2 (|u|_{\overline{\boldsymbol{\alpha}} ,\infty}^{\Omega_n} )^2 \cdot 2^{-2\ell}
%\end{align}
%\\
%For the second part, since  $ W^x_{t_n}  \sim \mathcal{N}(x, t_n I_d) $,
%\begin{align}\label{eq 1.10}
%	\esp{\mathbbm{1}_{W^x_{t_n} \notin  \Omega_n } } &= \mathbb{P}( W^x_{t_n} \notin  \Omega_n  ) 
%%	& = (\mathbb{P}( X \notin [-a, a] ) )^d, \qquad X \sim \mathcal{N}(0,1) \\
%	= (2\Phi^C(a) )^d\,,
%\end{align}
%where $\Phi^C(x) := \displaystyle{\int_{x}^{\infty} \dfrac{1}{\sqrt{2\pi} }e^{-\dfrac{t^2}{2} } dt }$.\\
%By the Komatsu's inequality\cite{ito2012diffusion} , we have 
%\[ \forall x \in \mathbb{R}^{+}, \qquad \dfrac{2}{x+\sqrt{x^2+4}} < e^{x^2/2} \int_{x}^{\infty} e^{-t^2/2}dt < \dfrac{2}{x+\sqrt{x^2+2}} \,.\]
%In fact, the equality on the left is true for $\forall x \in \mathbb{R}$. In \cite{szarek1997confidence}, the authors sharpened the inequality on the right to become 
%\[ \forall x>-1, \qquad e^{x^2/2} \int_{x}^{\infty} e^{-t^2/2}dt < \dfrac{4}{3x+\sqrt{x^2+8}}.  \]
%So that,
%\begin{equation}
%	\Phi^C(a) < \dfrac{1}{\sqrt{2\pi}} e^{-\dfrac{a^2}{2}} \dfrac{4}{3a+\sqrt{a^2+8}}<  \dfrac{1}{\sqrt{2\pi}} e^{-\dfrac{a^2}{2}} \dfrac{1}{a}.
%\end{equation}
%\\ 
%Since $\partial_x u: [0,T] \times \mathbb{R}^d \longmapsto \mathbb{R} $ is an at most polynomially growing continuous function, 
%by the inequalities (\ref{eq 1.10}) and (\ref{eq 1.12}), the second part has a upper bound below
%\begin{equation}\label{eq 1.13}
%	\begin{split}
%		\esp{ | \partial_x u(t_n,W^x_{t_n}) |^2 \mathbbm{1}_{W^x_{t_n} \notin  \Omega_n } } 	& \le \esp{  | \partial_x u(t_n,W^x_{t_n}) |^4}^\frac{1}{2} \esp{\mathbbm{1}_{W^x_{t_n} \notin  \Omega_n }}^\frac{1}{2}\\
%	& \le c_2 (2\Phi^C(a) )^\frac{d}{2} \esp{1+|W^x_{t_n}|^{4\beta }}^\frac{1}{2} \\
%	&:= c_2   (2\Phi^C(a) )^\frac{d}{2}  \lambda(x, t_n) \,,
%	\end{split}
%\end{equation}
%where
% \begin{equation}
% 	\begin{split}
% 		\lambda(x, t_n) &=  \esp{1+|x + W_{t_n}|^{4\beta }}^\frac{1}{2} \\
% 		&= \esp{1+ 2^{4\beta -1} (x^{4\beta } + | W_{t_n}|^{4\beta}) }^\frac{1}{2} \\
% 		&= (1+2^{4\beta - 1} (x^{4\beta } + t_n^{4\beta } (4\beta -1)!! ))^\frac{1}{2} \\
% 		& < (1+2^{4\beta - 1} (x^{4\beta } + T^{4\beta } (4\beta -1)!! ))^\frac{1}{2}, \qquad \forall n<N\,,
% 	\end{split}
% \end{equation}
% here, if $\beta = 0$, we define $ (-1)!!  := 1 $.\\
% 
%So that, from the inequalities  (\ref{eq 1.8}), (\ref{eq 1.9}) and (\ref{eq 1.13}) we have
%\begin{equation}
%\begin{split}
%	& \quad  \max_{1\le n\le N-1} \esp{|\partial_x \bar{u}(t_n,W^x_{t_n}) -\partial_x u(t_n,W^x_{t_n})|^2} \\
%		& \le   \max_{1\le n\le N-1} \left\{ \dfrac{1}{\sqrt{(2\pi t_n)^d}}  (2a\sqrt{t_n})^{d+2|\overline{ \boldsymbol{\alpha} }|_1}  C_2(d)^2( |u|_{\overline{\boldsymbol{\alpha}} ,\infty}^{\Omega_n})^2 \cdot 2^{-2\ell} + c_2  (2\Phi^C(a) )^\frac{d}{2}  \lambda(x, t_n) \right\} \\
%		& <     C(d) \left( (a)^{d + 2|\overline{ \boldsymbol{\alpha} }|_1} T^{2|\overline{ \boldsymbol{\alpha} }|_1}  \cdot 2^{-2\ell}  \max_{1\le n\le N-1} \left\{ ( |u|_{\overline{\boldsymbol{\alpha}} ,\infty}^{\Omega_n})^2 \right\} + (1+2^{4\beta - 1} (x^{4\beta } + T^{4\beta } (4\beta -1)!! ))^\frac{1}{2} \Gamma(a, d) \right)\\
%		& < C(\overline{ \boldsymbol{\alpha} }, \beta, d, T, x)  \left( (a)^{d+2|\overline{ \boldsymbol{\alpha} }|_1}  \cdot 2^{-2\ell } ( |u|_{\overline{\boldsymbol{\alpha}} ,\infty}^{\Omega_{\bar{n}}})^2  + \Gamma(a, d) \right).
%\end{split}
%\end{equation}
%%And when $n = 0 $,\\
%%\begin{align}
%%	h\; \esp{|\partial_x \bar{u}(t_n,W^x_{t_n}) -\partial_x u(t_n,W^x_{t_n})|^2} = \dfrac{1}{N} |\partial_x \hat{u}(0, x) -\partial_x u(0,x)|^2 \,.
%%\end{align}
%\eproof 
%\\
%\noindent
%\begin{Remark}\label{remark 2.1}
%If we want
%\begin{equation*}
%	\begin{split}
%		&\max_{1\le n \le N-1}  \esp{|\partial_x \bar{u}(t_n,W^x_{t_n}) -\partial_x u(t_n,W^x_{t_n})|^2} \le  C(\overline{ \boldsymbol{\alpha} }, \beta, d, T, x)  \left( (a)^{d+2|\overline{ \boldsymbol{\alpha} }|_1} ( |u|_{\overline{\boldsymbol{\alpha} } ,\infty}^{\Omega_{\bar{n}}})^2 \cdot 2^{-2\ell } + \Gamma(a, d) \right) \le \epsilon,  \\
%%		& h\; \esp{|\partial_x \bar{u}(t_0,W^x_{t_0}) -\partial_x u(t_0,W^x_{t_0})|^2}= \dfrac{1}{N} |\partial_x \bar{u}(0, x) -\partial_x u(0,x)|^2   \le \epsilon ,
%	\end{split}
%\end{equation*}
%we should have 
%%\begin{equation}
%%	N \ge \dfrac{|\partial_x \bar{u}(0, x) -\partial_x u(0,x)|^2}{\epsilon},
%%\end{equation}
%\begin{equation}
%	(a)^{d+2|\overline{ \boldsymbol{\alpha} }|_1} ( |u|_{\overline{\boldsymbol{\alpha} } ,\infty}^{\Omega_{\bar{n}}})^2 \cdot 2^{-2\ell } + \Gamma(a, d)  \le \dfrac{\epsilon}{C(\overline{\boldsymbol{\alpha}},\beta , d, T, x) } := C(\overline{\boldsymbol{\alpha}},\beta , d, T, x, \epsilon),
%\end{equation}
%\\
%First,
%% take
%%\begin{equation}
%%	N = \lceil\dfrac{|\partial_x \bar{u}(0, x) -\partial_x u(0,x)|^2}{\epsilon}\rceil = O(\epsilon^{-1} ),
%%\end{equation}
%%Second,
% take $a\in \mathbb{R}^+$ such that 
%\begin{equation}
%	a = \arg\min_{C(\alpha, \beta, d, T, x, \epsilon) >  \Gamma(a, d) }\left\{ \frac{a^{d + |\overline{\boldsymbol{\alpha}}|_1}}{ C(\overline{\boldsymbol{\alpha}},\beta , d, T, x,  \epsilon) - \Gamma(a, d) }  \right\}\,.
%\end{equation}
%%Third, 
%Then,
%let
%\begin{equation}
%\begin{split}
%	\ell  &= \min  \left\{k \in \mathbb{N}^* \;| \; (a)^{d+2|\overline{ \boldsymbol{\alpha} }|_1} ( |u|_{\overline{\boldsymbol{\alpha} } ,\infty}^{\Omega_{\bar{n}}})^2 \cdot 2^{-2k} \le C(\overline{\boldsymbol{\alpha}}, \beta,  d, T, x, \epsilon) - \Gamma(a, d)   \right\}\\
%	&= \left\lceil  \dfrac12 \log_2 \left( \dfrac{(a)^{d+2|\overline{ \boldsymbol{\alpha} }|_1} ( |u|_{\overline{\boldsymbol{\alpha} } ,\infty}^{\Omega_{\bar{n}}})^2 }{C(\overline{\boldsymbol{\alpha}}, \beta, d, T, x,  \epsilon) - \Gamma(a, d) }   \right)  \right\rceil\\
%	&= O( \log_2 (\epsilon^{-1/2} ) ).
%\end{split}
%\end{equation}
%In conclusion, we have 
%%\[ N = \cO(\epsilon^{-1} ) \,,\]
%\[ \ell  =\cO(\log_2 (\epsilon^{-1/2} ) ) \,, \]
%that is independent of the dimension $d$.
%\end{Remark}

\subsubsection{Norm equivalence constants}

We now provide some estimates for the value of $\alpha_{K}$ and $\kappa_{K}$ appearing in Assumption \ref{as psi function}.
\begin{Proposition} \label{pr minimal bound alpha} Suppose that Assumption \ref{ass periodic} holds. 
%Consider the basis functions $(\psi_{n}^{k})_{1 \leq n \leq N-1, 1\leq k \leq K}$ of the approximation spaces $\mathscr{V}_{n}$, $1 \le n \le N-1$, defined in Subsection \ref{subse approx space}. Then, there exists a constant $C \geq 1$ such that it holds
In the setting of Section \ref{subse picard periodic}, there exists a constant $\mathfrak{k} \leq 1$ such that
\begin{align*}
\mathfrak{k} =  \alpha_{K} = \frac1{\kappa_{K}} \;.% \le \bar{C}
\end{align*}
%\textcolor{red}{dependence in the constant}
%\noindent where the map $a \mapsto \mathrm{A}(a)$ is defined in Theorem \ref{th main sg error}. In particular, Assumption \ref{as psi function} is satisfied.
\end{Proposition}
%\begin{bluetext}
\proof 
For any $\mathfrak{u} = (\mathfrak{y}, \mathfrak{z}) \in \R^{K^y} \times \R^{d \bar{K}^z}$, any $0 \le n \le N-1$ and any $l \in \left\{1, \cdots, d\right\}$, from \eqref{eq de Z} we have
%$(Z^{\upsilon}_{t_n})_l := \sum_{k = 1}^{K} \theta^{n, k}_l  \psi_{n}^{k}(\widehat{X}_{t_n})$, one has
\begin{align*}
\esp{|(Z^{\mathfrak{u}}_{t_n})^l|^2}
= \esp{\Big| \sum_{k = 1}^{K} \mathfrak{z}^{n, k}_l  \psi^{k}_n(\widehat{X}_{t_n})\Big|^2}\,,
\end{align*}
Using Lemma \ref{le main estimate for frame}, we obtain
\begin{align}\label{eq encadrement 1}
 \mathfrak{C}^{-1}\esp{\Big| \sum_{k = 1}^{K} \mathfrak{z}^{n, k}_l  \psi^{k}_n(U)\Big|^2}
 \le
 \esp{|(Z^{\mathfrak{u}}_{t_n})^l |^2}
 \le
  \mathfrak{C}\esp{\Big| \sum_{k = 1}^{K} \mathfrak{z}^{n, k}_l  \psi^{k}_n(U)\Big|^2}\;.
\end{align}
%where we use Lemma \ref{le main estimate for frame} to get the last inequality.
%Recall that $\psi_{n}^{k}$ have support included in $\cO_n$   given by \eqref{definition:domain:On} so that the above equality reads
%\begin{align}
%\esp{|(Z_{t_n})_l|^2}
%=\int_{\cO_n }\Big| \textcolor{red}{ \sigma^{\top}(z) }  \sum_{k = 1}^{K} \theta^{n,k}_l  \psi_{n}^{k}(z)\Big|^2
%p^{\pi}(0, t_n, x_0, z) \ud z\;.
%\end{align}
%%where $\Xi_n$ is the density of $\cL(W_{t_n})$. \\
%From the Gaussian lower-estimate \eqref{Aronson:bounds:transition:density} for the transition density of the Euler scheme, and the diffusion coefficients are bounded, we obtain
%%\begin{align}
%%\forall z \in \cA_n,\frac{1}{(2\pi t_n)^{\frac{d}2}}\exp(-\frac{da^2}{2}) \le \Xi_n(z) \le \frac{1}{(2\pi t_n)^{\frac{d}2}}
%%\end{align}
%%leading to
%
%\begin{align}\label{eq min z 1}
%\esp{|(Z^{\upsilon}_{t_n})_l|^2}
%\ge C^{-1} \left(\frac{c^{-1}}{2\pi t_n}\right)^{\frac{d}2}\exp\left(-c^{-1}\frac{da^2}{2}\right)\int_{\cO_n^l}\Big|\sum_{k = 1}^{K} \theta^{n,k}_l \psi_{n}^{k}(z)\Big|^2
% \ud z\;, 
%\end{align}
%
%\noindent while using the Gaussian upper-estimate \eqref{Aronson:bounds:transition:density} yields
%\begin{align}\label{eq max z 1}
%\esp{|(Z^{\upsilon}_{t_n})_l|^2}
%\le  C \left(\frac{c}{2\pi t_n}\right)^{\frac{d}{2}} \int_{\cO_n }\Big|\sum_{k = 1}^{K} \theta^{n, k}_l \psi_{n}^{k}(z)\Big|^2
% \ud z\;. 
%\end{align}
Note that in our setting, $\psi_{n}^{k} = \chi^k$, so it holds
%From the definition of $\psi_{n}^{k}$, recall \eqref{defintion:space:basis:function:translated}, we get
\begin{align}
\int_{\cO}\Big|\sum_{k = 1}^{K} \mathfrak{z}^{n, k}_l  \psi_{n}^{k}(z)\Big|^2
 \ud z &= \int_{\cO}\Big|\sum_{k = 1}^{K} \mathfrak{z}^{n, k}_l  \chi^{k}(x)\Big|^2
\ud x\;. \label{eq min z 2}
\end{align}
Since the basis functions $(\chi^k)_{1 \le k \le K}$ forms a Riesz basis \cite{griebel1995tensor}, there exists a constant $\underline{c}\geq 1$ such that it holds
\begin{align}
\underline{c}^{-1} \sum_{k = 1}^{K} |\mathfrak{z}^{n, k}_l |^2  \le 
\int_{[0, 1]^d}\Big|\sum_{k = 1}^{K} \mathfrak{z}^{n, k}_l  \chi^{k}(x)\Big|^2 \ud x
\le \underline{c}
\sum_{k = 1}^{K} |\mathfrak{z}^{n, k}_l |^2 
\label{eq min z 3}
\end{align}
Combining \eqref{eq encadrement 1}-\eqref{eq min z 2}-\eqref{eq min z 3} and taking into account all the component of $Z^{\mathfrak{u}}_{t_n}$, we compute
\begin{align}\label{eq conclusion for z}
\underline{c}^{-1} \mathfrak{C}^{-1} d \sum_{k=1}^{K}  |\mathfrak{z}^{n, k}_l |^2  \le 
\esp{|(Z^{\mathfrak{u}}_{t_n}) |^2}
\le \underline{c}  \mathfrak{C} d \sum_{k=1}^{K} |\mathfrak{z}^{n, k}_l |^2 \;.
\end{align}
We also observe that
\begin{align}
\esp{|Y^{\mathfrak{u}}_0|^2}
= \esp{\Big| \sum_{k = 1}^{K} \mathfrak{y}^{k}  \chi^{k}(\cX_0)\Big|^2}\,.
\end{align}
Since $\cX_0 \sim \cU((0,1)^d)$, we similarly deduce that
\begin{align}
\underline{c}^{-1} \sum_{k = 1}^{K} |\mathfrak{y}^{n, k}_l |^2  \le 
\esp{|Y^{\mathfrak{u}}_0|^2}
\le \underline{c}
\sum_{k = 1}^{K} |\mathfrak{y}^{n, k}_l |^2. 
\label{eq conclusion y}
\end{align}
The proof is concluded by combining \eqref{eq conclusion for z} and \eqref{eq conclusion y} with \eqref{eq rewritte norms} and setting $\mathfrak{k} = \underline{c}^{-1} \mathfrak{C}^{-1}d^{-1}$.
\eproof
%\end{bluetext}
%\\
%
%\textcolor{magenta}{
%another bound:\\
%For any fixed point $X$ in the sparse grids, a pre-wavelet function is non-zero value in at most three hierarchical subspaces for a given level, so there are at most $3\ell$ basis functions of $K$ basis functions to approach are not zeros at point $X$. 
%\begin{align}
%	||\theta ||_{\pi, \psi}^2 &= h \sum_{n=1}^{N-1} \esp{|Z_{t_n}^{\upsilon}|^2} = h \sum_{n=1}^{N-1}\sum_{l=1}^d  \esp{|(Z_{t_n}^{\upsilon})_l|^2} \\
%	& =  h \sum_{n=1}^{N-1}\sum_{l=1}^d  \esp{| \sum_{k=1}^K \theta_{l}^{n,k} \psi_n^k(X_{t_n})   |^2} \\
%	& \le   h \sum_{n=1}^{N-1}\sum_{l=1}^d \esp{ O_d( \# \cL_\ell ) \sum_{k=1}^K |\theta_{l}^{n,k} \psi_n^k(X_{t_n})   |^2} \\
%	& \le h 3^dO_d( \# \cL_\ell ) \sup_{1\le l\le d, 1\le n\le N-1, 1\le k\le K, X_{t_n} \in \mathcal{O}_n } \psi_n^k(X_{t_n})   \sum_{n=1}^{N-1}\sum_{l=1}^d \sum_{k=1}^K |\theta_{l}^{n,k}|^2 \\
%	& \le Ch 3^dO_d( \# \cL_\ell ) \sup_{ l \in \mathcal{L}_{\ell} }  2^{ |\mathbf{l}|_1 } |\theta |^2 \le Ch 3^dO_d( \# \cL_\ell ) 2^{\frac{\ell + d -1}{2}} |\theta |^2
%\end{align}
%For the (energy) sparse grids with hat functions, we will have 
%\begin{equation}
%	||\theta ||_{\pi, \psi}^2 \le Ch  2^{ \ell } O_d( \# \cL_\ell ) \ell^{ - \frac12} |\theta |^2
%\end{equation}
%}
%

%\subsubsection{RM}

\subsubsection{Complexity analysis}\label{subse Com analysis}

%\textcolor{yellow}{
%\begin{Lemma}\label{le bound beta OLD}
%Under $\HYP{imp}$,
%\begin{align}
%\beta_{\pi,\psi} \le C_d  a^d 4^\ell \ell^{2d - 2}\,.
%\end{align}
%Note that $a$ has to be determined optimally in term of $\ell$ the "maximum level" of the space approximation. In this case $a = O_d(\ell^{\frac12})$, which leads to
%\begin{align}
%\beta_{\pi,\psi} \le C_d  4^\ell \ell^{\frac52d - 2}\,.
%\end{align}
%\end{Lemma}
%\proof
%1. We have
%\begin{align}
%\esp{||\Omega||^4}  &= \esp{( 1+\sum_{n=0}^{N-1}\sum_{k=1}^{K_n} ||\omega_n^k||^2 )^2} 
%\\
%&\le 2\left(1 + \esp{(\sum_{n=0}^{N-1}\sum_{k=1}^{K_n} ||\omega_n^k||^2 )^2 }\right)
%\end{align}
%Using Cauchy-Schwarz inequality, we compute
%\begin{align}
%	\esp{||\Omega||^4}& \le 2 (1+\bar{K} \sum_{n=0}^{N-1}\sum_{k=1}^{K_n} \esp{||\omega_n^k||^4} ) \\
%	&\le   C_d(1+h \bar{K} \sum_{k=1}^{K_n}  \esp{||\psi_n^k(W_{t_n})||^4} )\;. \label{eq first majo}
%\end{align}
%Recall Remark \ref{re indexation}, we now use the indexation related to the sparse grid description, to write
%\begin{align}\label{eq start majo}
%\sum_{k=1}^{K_n}  \esp{|\psi_n^k(W_{t_n})|^4} &= \sum_{(\mathbf{l},\mathbf{i}) \in \cC_n}\esp{|\psi_{n,(\mathbf{l},\mathbf{i})}(W_{t_n})|^4 }
%%\\
%%&\le C_d \sum_{(\mathbf{l},\mathbf{i}) \in \cC_n} 2^{2|\mathbf{l}|_1}
%\end{align}
%2. We study $\esp{|\psi_{n,(\mathbf{l},\mathbf{i})}(W_{t_n})|^4 }$ and remark that
%\begin{align}\label{eq dim d}
%\esp{|\psi_{n,(\mathbf{l},\mathbf{i})}(W_{t_n})|^4}  &= \esp{|\gamma_{(\mathbf{l},\mathbf{i})}(\tau_n(W_{t_n}))|^4 }
%\\
%&= \Pi_{j=1}^d \esp{|\gamma_{({l}_j,{i}_j)}(\tau^j_n(W_{t_n}))|^4 }
%\end{align}
%We now work component by  component. First, since
% $\tau^j_n(W_{t_n}) \sim \cN(\frac12 ,\frac1{4a^2})$ we get
% \begin{align}\label{eq one dim}
%\esp{|\gamma_{({l}_j,{i}_j)}(\tau^j_n(W_{t_n}))|^4 } 
%\le \sqrt{\frac2{\pi}}a\int |\gamma_{({l}_j,{i}_j)}(x)|^4 \ud x
% \end{align}
% Secondly, we compute,
% \begin{align}
% \int |\phi_{(l,i)}(x)|^4 \ud x = \int |\phi(2^l x - i)|^4 \ud x \le C 2^{-l}
% \end{align}
% and from the definition of $\gamma_{(l_j,i_j)}$, we deduce
% \begin{align}
% \int |\gamma_{({l}_j,{i}_j)}(x)|^4 \ud x \le C 2^{l} \;.
% \end{align}
% This leads , combining the previous inequality with \eqref{eq one dim} and \eqref{eq dim d}, to
% \begin{align}
% \esp{|\psi_{n,(\mathbf{l},\mathbf{i})}(W_{t_n})|^4}  = O_d(a^d2^{|\mathbf{l}|_1})\;.
% \end{align}
% 3. Combining the previous result with \eqref{eq start majo}, we obtain
% \begin{align} \label{eq first step 3}
% \sum_{k=1}^{K_n}  \esp{|\psi_n^k(W_{t_n})|^4} &\le C_d a^d \sum_{(\mathbf{l},\mathbf{i}) \in \cC_n} 2^{|\mathbf{l}|_1}
% \end{align}
% Here, we assume that  \HYP{imp} holds: all the $\cC_n$ are build with level $\ell$. We thus have
% \begin{align}
%Q :=  \sum_{(\mathbf{l},\mathbf{i}) \in \cC_n} 2^{|\mathbf{l}|_1}
% = 1 + \sum_{k=1}^\ell \sum_{\mathbf{l} \in \mathbb{N}^d} 2^{|\mathbf{l}|_1}\1_{\set{\zeta_d(\mathbf{l})=k}}\;.
% \end{align}
% We denote by $\| \mathbf{l} \|_0 = |\set{j|l_j = 0}|$. For $\mathbf{l} \neq \mathbf{0}$,
% recall that $\zeta_d(\mathbf{l}) = |\mathbf{l}|_1 + \|\mathbf{l}\|_0 -(d-1)$ (from the definition of $\zeta_d$). Thus, 
% \begin{align}
% Q &= 1 + \sum_{k=1}^\ell 
% \sum_{q=0}^{d-1}
% \sum_{\mathbf{l} \in (\mathbb{N}_{>0})^{d-q}} 
% 2^{|\mathbf{l}|_1}\1_{\set{|\mathbf{l}|_1=k+(d-1)-q  \text{ and } \|\mathbf{l}\|_0 = q } }
% \\
% &= 1 + \sum_{k=1}^\ell \sum_{q=0}^{d-1} 2^{k+(d-1)-q} \mathrm{C}_{k + d-q-2}^{d-q-1}
% \mathrm{C}_d^q
% \end{align}
% recall that $|\set{ \mathbf{l} \in (\mathbb{N}_{>0})^{d-q} \,| \,|\mathbf{l}|_1=k+(d-1)-q}| =\mathrm{C}_{k + d-q-2}^{d-q-1} $.
% Introducing $\theta = d-1-q$, we get
% \begin{align}
% Q = 1 + \sum_{k=1}^\ell d2^k + \sum_{\theta = 1}^{d-1} 2^{1+\theta} \mathrm{C}^{d-1 - \theta}_{d} \sum_{k=1}^\ell 2^{k-1} \mathrm{C}_{k-1+\theta}^{\theta}
% \end{align}
% From Lemma 3.6 in \cite{bungartz2004sparse}, we know that $\sum_{k=1}^\ell 2^{k-1} \mathrm{C}_{k-1+\theta}^{\theta} = 2^\ell(\frac{\ell^\theta}{\theta!} + O_d(\ell^{\theta-1}))$. Thus, we compute
% \begin{align}
% Q = 2^\ell\left(\frac{2^d}{(d-1)!}\ell^{d-1} + O_d(\ell^{d-2})\right)
%\end{align}
%Combining the previous equality with \eqref{eq first step 3}, we obtain
%\begin{align} \label{eq last step 3}
% \sum_{k=1}^{K_n}  \esp{|\psi_n^k(W_{t_n})|^4} \le C_d a^d2^\ell \ell^{d-1}
% \end{align}
% which combined with \eqref{eq first majo} concludes the proof.
%\eproof
%}

%\begin{bluetext}

%\subsubsection{Preparatory results}
\begin{Lemma}\label{le bound beta}
Under Assumption \ref{ass periodic}, one can set
\begin{align}
%\bcancel{
\beta_{K} = C_d(1+  2^\ell \ell^{d - 1})
\end{align}
\noindent for some positive constant $C_d$ which depends on the PDE dimension $d$.
\end{Lemma}
\proof


\noindent \emph{Step 1: } For any $n \in \set{0,\dots,N-1}$, any $\ell \in \set{1,\dots,d}$, one has
\begin{align}
\esp{|\tilde{\omega}^{n,\cdot}_\ell |^4}  &= \esp{\left(\sum_{k=1}^{K} |\tilde{\omega}^{n,k}_\ell|^2\right)^2} \,.
%\\
%&\le 2\left(1 + \esp{(\sum_{n=0}^{N-1}\sum_{k=1}^{K_n} ||\omega_n^k||^2 )^2 }\right)
\end{align}
Using Jensen's inequality, we obtain
\begin{align}
\esp{|\tilde{\omega}^{n,\cdot}_\ell |^4}  &\le K \esp{\sum_{k=1}^{K} |\tilde{\omega}^{n,k}_\ell|^4}  \le 3 {d^2}K  \sum_{k=1}^{K} \esp{|\psi_{n}^{k}(\widehat{X}_{t_n})|^4} \;. \label{eq first majo}
\end{align}
From now on, we use the indexation related to the sparse grid description introduced in Remark \ref{re indexation}, namely, we write
\begin{align}\label{eq start majo}
\sum_{k=1}^{K}  \esp{|\psi_{n}^{k}(\widehat{X}_{t_n})|^4} &= \sum_{(\mathbf{l},\mathbf{i}) \in \cC}\esp{|\psi_{n}^{(\mathbf{l},\mathbf{i})}(\widehat{X}_{t_n})|^4 }
%\\
%&\le C_d \sum_{(\mathbf{l},\mathbf{i}) \in \cC_n} 2^{2|\mathbf{l}|_1}
\\
&= \sum_{(\mathbf{l},\mathbf{i}) \in \cC}\esp{|\chi^{(\mathbf{l},\mathbf{i})}(\widehat{X}_{t_n})|^4 }
\end{align}
in our setting.

\noindent \emph{Step 2: }
%\begin{bluetext}
%We now study $\esp{|\psi_{n}^{(\mathbf{l},\mathbf{i})}(\widehat{X}_{t_n})|^4 }$.
 Using Lemma \ref{le main estimate for frame}, we observe
\begin{align}\label{eq control beta interm 1}
\esp{|\chi^{(\mathbf{l},\mathbf{i})}(\widehat{X}_{t_n})|^4 }  &\le \mathfrak{C} 
\esp{|\chi^{(\mathbf{l},\mathbf{i})}(U)|^4}\;.
%\\
%\esp{|\chi^{(\mathbf{l},\mathbf{i})}(\tau_n(U)|^4 }
%\nonumber \\
%&=  \esp{\prod_{j=1}^d |\chi^{({l}_j,{i}_j)}(\tau^j_n(X^{x_0}_{t_n}))|^4 } \nonumber \\
%& = \int_{\mathbb{R}^d} \prod_{j=1}^d  |\chi^{({l}_j,{i}_j)}(\tau^j_n(x))|^4 \, p^{\pi}(0, t_n, x_0, x) \, dx \label{eq dim d}
\end{align}
%\textcolor{red}{assuming $\psi = \chi$}
%\noindent where $\tau^{j}_n(x) = (x_j -  \mathfrak{a}^n_j)/(2 a\sqrt{t_n})$ stands for the $j$-th coordinate of $\tau_n(x)$. Using the Gaussian upper-estimate \eqref{Aronson:bounds:transition:density} for the transition density of the Euler-Maruyama scheme and then the change of variable $x_j=(x_0)_j -a \sqrt{t_n}+ y_j 2a\sqrt{t_n}$, $j=1, \cdots, d$, we obtain
% \begin{align}\label{eq one dim}
%\int_{\mathbb{R}^d} \prod_{j=1}^d  |\chi^{({l}_j,{i}_j)}(\tau^j_n(x))|^4 \, p^{\pi}(0, t_n, x_0, x) \, dx 
%\le C \left(\frac{2 c a^2}{\pi}\right)^{\frac{d}{2}}\prod_{j=1}^d \int |\chi^{({l}_j,{i}_j)}(y_j)|^4 \ud y_j.
% \end{align}

%\begin{align}\label{eq dim d}
%\esp{|\psi_{n}^{(\mathbf{l},\mathbf{i})}(\widehat{X}_{t_n})|^4}  &\le \mathfrak{C} 
%\esp{|\chi^{(\mathbf{l},\mathbf{i})}(U)|^4}
%\end{align}

\noindent Moreover, we compute
 \begin{align*}
 \int |\phi^{(l,i)}(x)|^4 \ud x = \int |\phi(2^l x - i)|^4 \ud x \le C 2^{-l}
 \end{align*}
 
 \noindent and from the definition of $\chi^{(l_j,i_j)}$, we deduce
 \begin{align*}
 \int |\chi^{({l}_j,{i}_j)}(x)|^4 \ud x \le C 2^{l} \;.
 \end{align*}

\noindent Combining the previous inequality with  \eqref{eq control beta interm 1} leads to
 \begin{align*}
\esp{|\chi^{(\mathbf{l},\mathbf{i})}(\widehat{X}_{t_n})|^4 }  \leq {C} 2^{|\mathbf{l}|_1}\;
 \end{align*}
 
 \noindent and inserting the previous estimate in \eqref{eq start majo} yields
 \begin{align} \label{eq first step 3}
 \sum_{k=1}^{K}  \esp{|\psi_{n}^{k}(\widehat{X}_{t_n})|^4} &\le {C} \sum_{(\mathbf{l},\mathbf{i}) \in \cC} 2^{|\mathbf{l}|_1}.
 \end{align}
 %\end{bluetext}
\noindent \emph{Step 3: } We now quantify the term appearing in the right-hand side of \eqref{eq first step 3}, namely
 \begin{align}
Q :=  \sum_{(\mathbf{l},\mathbf{i}) \in \cC} 2^{|\mathbf{l}|_1}
 = 1 + \sum_{k=1}^\ell \sum_{\mathbf{l} \in \mathbb{N}^d} 2^{|\mathbf{l}|_1}\1_{\set{\zeta_d(\mathbf{l})=k}}\;.
 \end{align}
 We denote by $\| \mathbf{l} \|_0 = |\set{j|l_j = 0}|$. For $\mathbf{l} \neq \mathbf{0}$,
 recall that $\zeta_d(\mathbf{l}) = |\mathbf{l}|_1 + \|\mathbf{l}\|_0 -(d-1)$ (from the definition of $\zeta_d$). Thus, 
 \begin{align*}
 Q &= 1 + \sum_{k=1}^\ell 
 \sum_{q=0}^{d-1}
 \sum_{\mathbf{l} \in (\mathbb{N}_{>0})^{d-q}} 
 2^{|\mathbf{l}|_1}\1_{\set{|\mathbf{l}|_1=k+ d-1 -q  \text{ and } \|\mathbf{l}\|_0 = q } }
 \\
 &= 1 + \sum_{k=1}^\ell \sum_{q=0}^{d-1} 2^{k+ d-1-q} \mathrm{C}_{k + d-q-2}^{d-q-1}
 \mathrm{C}_d^q
 \end{align*}
 recall that $|\set{ \mathbf{l} \in (\mathbb{N}_{>0})^{d-q} \,| \,|\mathbf{l}|_1=k+ d-1 -q}| =\mathrm{C}_{k + d-q-2}^{d-q-1} $.
 Introducing $\theta = d-1-q$, we get
 \begin{align}
 Q = 1 + \sum_{k=1}^\ell d2^k + \sum_{\theta = 1}^{d-1} 2^{1+\theta} \mathrm{C}^{d-1 - \theta}_{d} \sum_{k=1}^\ell 2^{k-1} \mathrm{C}_{k-1+\theta}^{\theta}
 \end{align}
 From Lemma 3.6 in \cite{bungartz2004sparse}, we know that $\sum_{k=1}^\ell 2^{k-1} \mathrm{C}_{k-1+\theta}^{\theta} = 2^\ell(\frac{\ell^\theta}{\theta!} + O_d(\ell^{\theta-1}))$. We thus obtain
 \begin{align*}
 Q = 2^\ell\left(\frac{2^d}{(d-1)!}\ell^{d-1} + O_d(\ell^{d-2})\right)
\end{align*}
\noindent which combined with \eqref{eq first step 3} yields
\begin{align} \label{eq last step 3}
 \sum_{k=1}^{K}  \esp{|\psi_{n}^{k}(\widehat{X}_{t_n})|^4} \le C_d 2^\ell \ell^{d-1}.
 \end{align}
Combining the previous inequality with \eqref{eq first majo}, we obtain
\begin{align}
\esp{|\tilde{\omega}^{n,\cdot}_\ell|^4} \le C_d 2^{2\ell} \ell^{2d-2}\;.
\end{align}
Using similar arguments, as the basis function are chosen to be the same in our setting, we also have
\begin{align*}
\esp{|\theta|^4} \le C_d 2^{2\ell} \ell^{2d-2}\;.
\end{align*}
The proof is then concluded recalling the definition of $\beta_{K}$ in \eqref{eq de beta psi}.
\eproof

%\begin{Remark}\label{remark:value:beta:parameter:h:l}
%Note that the value of the parameter $a$ has to be determined optimally in term of $\ell$ the level of the sparse grid approximation space. According to Theorem \ref{th main sg error}, one has $a = O_d(\ell^{\frac12})$, which leads to
%\begin{align*}
%\beta_{\pi,\psi} = C ( 1 + h 2^\ell \ell^{\frac54d - 1})\,.
%\end{align*}
%\end{Remark}


\vspace{2mm}
\noindent We now turn to the analysis of the convergence and complexity of the full Picard algorithm. The following corollary is a preparatory result and expresses the main convergence results in terms of the parameters $P$, $M$, $\ell$ and $h$.

\begin{Corollary} \label{co conv results new}
Suppose that Assumption \ref{ass periodic} as well as \eqref{eq constraint alpha-beta-M 1} and \eqref{eq ass cs control global}  hold. Set $\gamma_m = \gamma/ m^{\rho}$, for some $\rho \in (1/2, 1)$ and $\gamma > 0$. If $T(1+ 2L^2(1+ h)) < 1$ and $\delta_{h,\eta}=\frac{16L^2 T (1+2\eta)}{1-T(1+ 2L^2(1+ h))} < 1$, then, with the notations of Proposition \ref{error of Picard}, for any $\varepsilon>0$ such that $\delta_{h, \varepsilon}:= \delta_{h, \eta } (1+\varepsilon)<1$ there exist constants $C_\varepsilon:=C(\varepsilon, T, b, \sigma, d, \gamma,\rho)\geq1$, $c := c(T, b, \sigma, d, \gamma) > 0$ such that it holds
\begin{align} \label{global:mean:squared:error:before:complexity}
\cE_P \le \delta_{h, \varepsilon}^P \cE_0 + C_{\varepsilon} 
\left(
Ne^{- c \frac{M^{1-\rho}}{1 + 2^\ell\ell^{d-1}}} 
+  \frac{ 1 + 2^\ell\ell^{d-1}}{h M^\rho } + 2^{-4\ell}\ell^{d-1} + h
\right) \;.
\end{align}

%\begin{align}
%\cE_P \le \delta_{h, \varepsilon}^P \cE_0 &+ C_{\varepsilon} \left(\frac{1}{M} + h +  2^{-4\ell} \ell^{\frac{7d-2}{2}} + (2^{\textcolor{red}{\frac{4\ell d}{c^2}}}+\textcolor{red}{\ell^{\frac{d}{2}}}) \left( e^{-\textcolor{red}{2 \ln(2)}\gamma\mathfrak{d}_{h,\ell}M^{1-\rho}  } +  \frac{ 1}{\mathfrak{d}_{h,\ell}M^\rho} \right)
% \right)
%\end{align}
%with
%\begin{align*}
% C^{-1} \frac{h 2^{-\textcolor{red}{\frac{4\ell d}{c^2}}} \ell^{\frac{d}{2}}}{1+h2^{\ell} \ell^{\frac{5}{4}d-1}}  \leq  \mathfrak{d}_{h,\ell}  := \frac{\alpha_{\pi, \psi}}{\beta_{\pi,\psi}}. 
% %\leq C \frac{h 2^{-4\ell} \ell^{\frac{d}{2}}}{1+h2^{\ell} \ell^{\frac{5}{4}d-1}} \;.
%\end{align*}
\end{Corollary}
\proof Combining Proposition \ref{pr main abstract error} with Theorem \ref{th main sg error} and \eqref{eq control disc error}, we obtain
\begin{align}%\label{global:control:error}
\cE_P \le \delta_{h, \varepsilon}^P \cE_0 + C_\varepsilon \left(
\frac{\kappa_{K}}{h \wedge \alpha_{K} } L_{K,M}  + 2^{-4\ell}\ell^{d-1} + h \right).
\end{align}
From Proposition \ref{pr minimal bound alpha}, we have that $\frac{\kappa_{K}}{h \wedge \alpha_{K} } \le \frac{C}{h}$, which combined with Lemma \ref{le gamma spec LpipsiM} gives
\begin{align}
\frac{\kappa_{K}}{h \wedge \alpha_{K} } L_{K,M} &\le \frac{ C_{\rho,\gamma} }{h} \left(e^{- \gamma 2 \sqrt{2} \ln(2)\frac{\mathfrak{k} }{\beta_{K}}M^{1-\rho}} 
+  \frac{ \beta_{K}}{\mathfrak{k} M^\rho }
\right)
\\
&\le \frac{ C_{\rho,\gamma} }{h} \left(e^{- c \frac{M^{1-\rho}}{1 + 2^\ell\ell^{d-1}}} 
+  \frac{ 1 + 2^\ell\ell^{d-1}}{M^\rho }
\right)
\end{align}
for some positive constant $c$, where we used Lemma \ref{le bound beta} for the last inequality.
\eproof
%\begin{align}
%\cE_P \le \delta_{h, \varepsilon}^P \cE_0 &+ C_{\varepsilon} \Big(\frac{1}{M} + h +   2^{-4\ell}\ell^{\frac{7d-2}{2}} + L_{\pi,\psi,M}\kappa_{\pi,\psi}N  + L_{\pi, \psi, M} \frac{\kappa_{\pi, \psi}}{\alpha_{\pi,\psi}} 
% \Big).
%\end{align}
%Using Theorem \ref{th main sg error} and Proposition \ref{pr minimal bound alpha}, there exists some constant $C:=C(T, b, \sigma, d)\geq1$ such that
%\begin{align}\label{upper:bound:ratio:constant:parameters}
%&\frac{\kappa_{\pi,\psi}}{\alpha_{\pi,\psi}} \leq C e^{\frac{d a^2}{2c}}
% \leq C 2^{\textcolor{red}{\frac{4 \ell d}{c^2}}} \text{ and }
%\kappa_{\pi, \psi} N  \leq C (\sqrt{c} a)^d\leq C \ell^{\frac{d}{2}} \\
%\end{align}
%and from Lemma \ref{le bound beta} it holds
%\begin{align}
%C^{-1} \frac{h 2^{- \textcolor{red}{\frac{4\ell d}{c^2}}} \ell^{\frac{d}{2}}}{1+h2^{\ell} \ell^{\frac{5}{4}d-1}} \leq \mathfrak{d}_{h,\ell} := \frac{\alpha_{\pi, \psi}}{\beta_{\pi,\psi}}.
%% \leq C \frac{h 2^{-4\ell} \ell^{\frac{d}{2}}}{1+h2^{\ell} \ell^{\frac{5}{4}d-1}} . %= 
%%\textcolor{red}{c_d  2^{-5\ell} \ell^{-\frac34 d+1}}
%\end{align}
%We eventually conclude by combining the above upper-bounds with Lemma \ref{le gamma spec LpipsiM}.

%\end{bluetext}

%\begin{yellowtext}
%\begin{Corollary} \label{co conv results}
%Let \HYP{r}, \HYP{L}-\HYP{b} and \HYP{imp} hold. Set $\gamma_m = \gamma_1/ m^{\rho}$, for some $\rho \in (1/2, 1)$.
%Assume \eqref{eq ass cs control global} hold. If $T(1+ 2L^2(1+ h)) < 1$ and
%$\delta:=\frac{8L^2 T (1+2C)}{1-T(1+ 2L^2(1+ h))} < 1$, then for any $\varepsilon>0$ such that $\delta_\varepsilon := \delta (1+\varepsilon)<1$, for some positive constant $C_\varepsilon$ one has
%%\begin{align}\label{eq conv results}
%%\cE_P &\le C_{\delta} \Big( \delta^P \cE_0+  2^{-4\ell}\ell^{3d-1} +  h 
%%+ \frac{2^{7\ell}\ell^{2d-2}}{{M^{2\eta-1}}} + 2^{4\ell} \exp\left(-4\gamma h 2^{-4 \ell} \ell^{\frac{d}2}(M^{1-\eta}-1)\right)\Big)\;,
%%\end{align}
%\begin{align}
%\label{ineq:conv:results}
%\cE_P \le \delta_\varepsilon^P \cE_0 + C_\varepsilon  \sum_{p=1}^{P}\delta_{\varepsilon}^{P-p} [\frac{1}{M_p} + L_{\pi,\psi,M_p} [h \ell^{\frac{d}{2}} +  2^{4\ell}] + h +  2^{-4\ell}\ell^{3d-1}] 
%\end{align}
%\noindent with
%\begin{align}
%L_{\pi, \psi, M_p} & \leq \frac{1}{M^{\rho}_p}+ e^{-2 \gamma_1\tilde{\alpha}_{\pi,\psi} \frac{2^{1-\rho}-1}{2^{1-\rho}(1-\rho)} M_p^{1-\rho}} +  e^{-2\gamma_1\frac{\tilde{\alpha}_{\pi, \psi}}{1-\rho} M^{1-\rho}_p} \nonumber\\
%& \leq \frac{1}{M^{\rho}_p}+2 e^{-2 \gamma_1\tilde{\alpha}_{\pi,\psi} \frac{2^{1-\rho}-1}{2^{1-\rho}(1-\rho)} M_p^{1-\rho}} \label{bound:L2:error:sg:algorithm}
%%L^2_{\psi, \pi, M_p} & \leq \sum_{\ell=1}^{M_p} e^{-2 \tilde{\alpha}_{\pi, \psi}(\Gamma_{M_p}-\Gamma_\ell)} \gamma^2_\ell +  K e^{-2 \tilde{\alpha}_{\pi, \psi}\Gamma_{M_p}}
%\end{align}
%\noindent and where $\tilde{\alpha}_{\pi, \psi}$ satisfies
%$$
%\tilde{\alpha}_{\pi, \psi} \geq h 2^{-7\ell} \ell^{-\frac32 d + 2}.
%$$
%\end{Corollary}
%\proof
%The inequality \eqref{ineq:conv:results} follows directly from Proposition \ref{pr error of Picard sharper}, Theorem \ref{th main sg error} and Lemma \ref{le disc time error}. 
%From Lemma \ref{le bound beta} and Proposition \ref{pr minimal bound alpha}, it holds
%$$
%\tilde{\alpha}_{\pi, \psi} = \frac{\alpha_{\pi, \psi}}{(1+ \mathbb{E}[\|\Omega\|^4])^{\frac12}} \geq c_d \frac{h 2^{-4\ell} \ell^{\frac{d}{2}}}{2^{\ell} \ell^{\frac{5}{4}d-1}} = c_d h 2^{-5\ell} \ell^{-\frac34 d+1}
%$$
%%\begin{align}\label{eq express L}
%%L_{\pi,\psi,M} = O_d \left( 8^{\ell}\ell^{2d-2} M^{1-2\eta} + \exp\left(-4\gamma h 2^{-4 \ell} \ell^{\frac{d}2}(M^{1-\eta}-1)\right) \right)
%%\end{align}
%Using Theorem \ref{th main sg error} and Proposition \ref{pr minimal bound alpha}, we compute that
%\begin{align}
%\frac{\kappa_{\pi,\psi}}{\alpha_{\pi,\psi}} &= O( e^{\frac{da^2}2})
%=O(2^{4 \ell}), \\
%\kappa_{\pi, \psi} & = c_d h \ell^{\frac{d}{2}}
%\end{align}
%since $a=\sqrt{\mathfrak{c}\ell}$, with $\mathfrak{c}=\frac{8}d \log(2)$ is introduced in Theorem \ref{th main sg error}. The previous estimate combined with \eqref{ineq:conv:results} concludes the proof.
%\eproof
%
%\begin{Theorem} \label{thm full complexity}
%Let \HYP{r}, \HYP{L}-\HYP{b} and \HYP{imp} hold.
%%\textcolor{red}{
%For the approximation space and basis functions defined in Subsection \ref{subse approx space},
%% under the setting of Theorem \ref{th main sg error} and the estimate value of $\alpha$ and $\kappa$ in %Proposition \ref{pr minimal bound alpha},} 
%the complexity $\cC_\epsilon $of the full \emph{Picard algorithm} to obtain $\cE_P = O_d(\epsilon^2)$ is, for all $\iota > 0$,
%$$
%\cC_\epsilon = O_d(\epsilon^{-\frac{23}{2}-\mu}\log(\epsilon^{-1})^{q_{d, \mu}})
%$$
%\noindent with $q_{d, \mu} = \frac{7}{4}d+\frac{d}{1-\frac{\mu}{9+\mu}}-\frac{1}{4} \rightarrow \frac{11}{4}d-\frac{1}{4}$ as $\mu \downarrow 0$.\\
%\end{Theorem}
%\end{yellowtext}

%\begin{bluetext}

We are now ready to establish the complexity of the full Picard algorithm.
%based on the sparse grid approximation space defined in Subsection \ref{subse approx space}.  
%\begin{Theorem} \label{thm full complexity}
%Suppose that Assumption \ref{assumption:coefficient} is in force. For a prescribed $\varepsilon>0$, the complexity $\cC_\varepsilon $ of the full \emph{Picard algorithm} in order to achieve a global error $\cE_P$ of order $\varepsilon^2$ satisfies
%$$
%\cC_\varepsilon = O_d(\varepsilon^{-12\mu-\frac52}|\log_{2}(\varepsilon)|^{\frac{15+78\mu}{8}d - 3 \mu +\frac34})\;
%$$
%\noindent for any $1<\mu <\frac34$.
%%\noindent with $q_{d, \mu} = \frac{7}{4}d+\frac{d}{1-\frac{\mu}{9+\mu}}-\frac{1}{4} \rightarrow \frac{11}{4}d-\frac{1}{4}$ as $\mu \downarrow 0$.\\
%\end{Theorem}

\paragraph{Proof of Theorem \ref{thm full complexity}}
\emph{Step 1: Setting the parameters $P$, $N$, $M$, $\ell$ and $\rho$.}\\ We will chose the parameters $P$, $N$, $M$, $\ell$ and $\rho$ in order to achieve a global error $\cE_P$ of order $\varepsilon^2$, as this error controls $\cE_{\mathrm{MSE}}$. We first set $P = 2 |\log_\delta(\varepsilon)|$ and \textcolor{black}{$N_\varepsilon= \ceil*{T\varepsilon^{-2}} $ so that $h_\varepsilon=T/N_\varepsilon\leq \varepsilon^2$}. From Theorem \ref{th main sg error}, we also know that setting $\ell_\varepsilon = \log_2(\varepsilon^{-\frac12}|\log_2(\varepsilon)|^{\frac{d-1}{4 } })$, we obtain $\cE_\psi= O_d(\varepsilon^2)$ and $K_\varepsilon = O_d(\varepsilon^{-\frac12}|\log_2(\varepsilon)|^{\textcolor{black}{\frac{5(d-1)}4 }})$.

We now set $M$ such that the term $\frac{K_\varepsilon}{M^\rho h_\varepsilon}$ is of order $\varepsilon^2$, which leads to
\begin{align*}
M_\varepsilon = O_d(\varepsilon^{-\frac9{2 \rho}}|\log_2(\varepsilon)|^{ \textcolor{black}{ \frac{5(d-1)}{4\rho }} })\,.
\end{align*}
For $\iota > 1$, we set $\bar{\rho} = \frac9{10 \iota}$ with the constraint $\bar{\rho} > \frac12$ and we verify that
\begin{align*}
\frac{M_\epsilon^{1-\bar{\rho}}}{K_\varepsilon} \ge c \varepsilon^{5(1-\iota)}|\log_2(\varepsilon)|^{\textcolor{black}{\frac54}(d-1)(\frac1{\bar{\rho}} - 2)}
\end{align*}
for some constant $c>0$. This leads to
\begin{align*}
e^{- c \frac{M_\varepsilon^{1-\bar{\rho}}}{1 + 2^{\ell_\varepsilon} \ell_\varepsilon^{d-1}}}  = o(\varepsilon^4) 
\end{align*}
%\textcolor{red}{ here we should request $ o(\varepsilon^4)  $,\\  }
and we also have that \eqref{eq constraint alpha-beta-M 1} is satisfied.\\
\emph{Step 2: Computing the complexity $\cC_\varepsilon$.} Recalling Remark \ref{re num complexity direct algo}, we see that the overall complexity $\cC_\varepsilon$ to reach the prescribed approximation accuracy $\varepsilon^2$ satisfies 
\begin{align*}
\cC_\varepsilon &= P_\varepsilon N_\varepsilon K_\varepsilon M_\varepsilon
\\
&= O_d \left(
|\log_{2}(\varepsilon)| \varepsilon^{-2} \varepsilon^{-\frac12}|\log_2(\varepsilon)|^{\textcolor{black}{\frac{5(d-1)}4}}
\varepsilon^{-5\iota }|\log_2(\varepsilon)|^{ \frac{25(d-1)\iota}{18}}
\right)
\\
&=O_d(\varepsilon^{-\frac52(1+2\iota )}|\log_{2}(\varepsilon)|^{1+ \frac{45+50\iota}{36}(d - 1)} )\;,
\end{align*}
which concludes the proof.


%\emph{Step 1: Setting the parameters $P$, $N$, $M$, $\ell$ and $\rho$.}\\ In order to achieve a global error $\cE_P$ of order $\varepsilon^2$, we first set $P = 2 |\log_\delta(\varepsilon)|$ and \textcolor{red}{$N= \ceil*{T\varepsilon^{-2}} $ so that $h=T/N\leq \varepsilon^2$}. From Theorem \ref{th main sg error}, we also know that setting $\ell_\varepsilon =  \log_2(\varepsilon^{-\frac12}|\log_2(\varepsilon)|^{\frac{7d-2}8})$, we obtain $2^{-4\ell_\varepsilon}\ell_\varepsilon^{\frac{7d-2}{2}} = O_d(\varepsilon^2)$. With this choice of parameter, we also observe that
%\begin{align}
%\label{first:lower:bound:complexity:proof}
%\mathfrak{d}_{h, \ell_\varepsilon} \ge C^{-1} h2^{-\textcolor{red}{\frac{4\ell_\varepsilon}{c^2}}} \ell_\varepsilon^{\frac{d}{2}} \ge C^{-1} \varepsilon^4|\log_2(\varepsilon)|^{1-3d} =: \mathfrak{d}_\varepsilon\,.
%\end{align}.
%
%We now need to set $M$ optimally such that
%\begin{align}\label{optimality:condition:number:steps:SG}
%\exp\left( -\textcolor{red}{2\ln(2)}\gamma\mathfrak{d}_{\varepsilon}M^{1-\rho}  \right)
%+
%\frac{ 1}{\mathfrak{d}_{\varepsilon}M^\rho}
% =O( \varepsilon^{4}|\log_2(\varepsilon)|^{\frac{2-7d}{2}})
%\end{align}
%and the constraints \eqref{eq constraint alpha-beta-M 1} and \eqref{eq ass cs control global} are satisfied. It is sufficient to have, for some $c>0$,
%\begin{align*}
%\mathfrak{d}_{\varepsilon}M^{1-\rho}  \textcolor{red}{>\frac{2}{\gamma}} |\log_2(\varepsilon)| \quad \text{ and } \quad \frac{ 1}{\mathfrak{d}_{\varepsilon}M^\rho}
%\le c \varepsilon^{4}|\log_2(\varepsilon)|^{\frac{2-7d}{2}}
%\end{align*}
%\noindent \textcolor{red}{as $\varepsilon \downarrow 0$.} Now, for any $1 < \mu <\frac43$, we set 
%\begin{align}
%\rho := \frac2{3 \mu}, \text{ and  } M_\varepsilon := \varepsilon^{-\frac8\rho}|\log_2(\varepsilon)|^{\frac{13d-4}{2 \rho}}  \;.
%\end{align}
%We then verify
%\begin{align*}
%\frac{ 1}{\mathfrak{d}_{\varepsilon}M_\varepsilon^\rho} = O(\varepsilon^{4}|\log_2(\varepsilon)|^{\frac{2-7d}{2}})
%\end{align*}
%and
%\begin{align*}
%\mathfrak{d}_{\varepsilon}M_\varepsilon^{1-\rho} = \varepsilon^{4-\frac{8(1-\rho)}\rho}|\log_2(\varepsilon)|^{1-3d+\frac{13d -4}{2}\frac{1-\rho}{\rho}}
%\textcolor{red}{> \frac{2}{\gamma}|\log_2(\varepsilon)|}\;
%\end{align*}
%\textcolor{red}{it seems wrong when $\rho \rightarrow 2/3$}\\
%\noindent as $\varepsilon \downarrow0$ since $\frac{1-\rho}{\rho} \in (1/2, 1)$ for any $\rho \in (1/2,2/3)$. \textcolor{red}{Finally, it is readily seen that the upper inequality of \eqref{eq constraint alpha-beta-M 1} is satisfied. Observe also that $\sqrt{2}M_\varepsilon^{\rho-1} = \sqrt{2} \varepsilon^{8 \frac{1-\rho}{\rho}} | \log_2(\varepsilon)|^{\frac{4-13d}{2}\frac{1-\rho}{\rho}} \leq \mathfrak{d}_\varepsilon \leq \mathfrak{d}_{h, \ell_\varepsilon}$ using \eqref{first:lower:bound:complexity:proof} and the fact that $\frac{1-\rho}{\rho} \in (1/2, 1)$ for any $\rho \in (1/2,2/3)$. Hence, the constraint \eqref{eq constraint alpha-beta-M 1} is satisfied. Using \eqref{upper:bound:rate:convergence:SG:algorithm}, \eqref{optimality:condition:number:steps:SG}, \eqref{upper:bound:ratio:constant:parameters} as well as the value of $\ell_\varepsilon$, we deduce that the constraint \eqref{eq ass cs control global} is also satisfied. } \\
%
%\emph{Step 2: Computing the complexity $\cC_\varepsilon$.} Recalling Remark \ref{re num complexity direct algo}, we see that the overall complexity $\cC_\varepsilon$ to reach the prescribed approximation accuracy $\varepsilon^2$ satisfies  (\textcolor{red}{$K_\varepsilon$ should be changed if we want to take into account the implementation - slightly smaller complexity. However due to the light impact (unfortunately) maybe we can just make a remark...})
%\begin{align*}
%\cC_\varepsilon &= P_\varepsilon N_\varepsilon K_\varepsilon M_\varepsilon
%\\
%&= O_d(
%|\log_{2}(\varepsilon)| \varepsilon^{-2} \varepsilon^{-\frac12}|\log_2(\varepsilon)|^{\frac{15}{8}d-\frac14}
%\varepsilon^{-12\mu}|\log_2(\varepsilon)|^{\frac{39d-12}{4}\mu}
%)
%\\
%&=O_d(\varepsilon^{-12\mu-\frac52}|\log_{2}(\varepsilon)|^{\frac{15+78\mu}{8}d - 3 \mu +\frac34})\;,
%\end{align*}
%which concludes the proof.
\eproof
%\end{bluetext}

%\textcolor{red}{
%\begin{Remark}
%	In the numerical implementation, $K_\varepsilon$ can be much smaller if the basis functions are modified hat functions and we check whether the random variable $ X_{t_n} $ is in the support of $ \{\psi_{n}^k\}_{1\le k \le K_\epsilon} $ before computing $ \{\psi_{n}^k( X_{t_n}  )\}_{1\le k \le K_\epsilon}  $, for all $0\le n \le N-1$.
%\end{Remark}
%}

%\begin{yellowtext}
%\vspace{2mm}
%\proof
%%N: I'm trying to establish the optimal complexity in view of the modifications i made to the previous estimates so we will consider two cases. The first one refers to the natural choice $M_p = M$ for all $p=1, \cdots, P$ while in the second case we will balance the number of simulations according to the Picard iterate.\\
%%\newline
%To obtain a precision $O_d(\epsilon^2)$ in the error $\cE_P$, we first have to set $P = 2 |\log_\delta(\epsilon)|$ and $N= \epsilon^{-2} =\frac1h$. From Theorem \ref{th main sg error}, we also know that setting $\ell_\epsilon= \log_2(\epsilon^{-\frac12}|\log_2(\epsilon)|^{\frac{3d-1}4})$, we obtain $2^{-4\ell_\epsilon}\ell_\epsilon^{3d-1} = O_d(\epsilon^2)$. We now need to find an optimal sequence $(M_p)_{1\leq p \leq P}$ so that
%$$
%\sum_{p=1}^{P}\delta_{\varepsilon}^{p} [\frac{1}{M_{P-p}} + L_{\pi,\psi,M_{P-p}} [h_\epsilon \ell_\epsilon^{\frac{d}{2}} +  2^{4\ell_\epsilon}]] \leq \sum_{p=1}^{P}\delta_{\varepsilon}^{p} [\frac{1}{M_{P-p}} + L_{\pi,\psi,M_{P-p}} \epsilon^{-2}|\log_2(\epsilon)|^{3d-1}] \leq  \epsilon^2.
%$$
%In view of \eqref{bound:L2:error:sg:algorithm}, it suffices to find $(M_p)_{1\leq p \leq P}$ so that
%\begin{equation}\label{constraint:optimize:M:sequence}
%\sum_{p=1}^{P}\delta_{\varepsilon}^{p} [\frac{1}{M^{\rho}_{P-p}} +e^{-2 \gamma_1\tilde{\alpha}_{\pi,\psi} \frac{2^{1-\rho}-1}{2^{1-\rho}(1-\rho)} M_{P-p}^{1-\rho}} ]\leq \epsilon^4 |\log_2(\epsilon)|^{1-3d}.
%\end{equation}
%First note that the above choices of $h_\varepsilon$ and $\ell_\varepsilon$ imply
%\begin{equation}\label{lower:bound:alpha}
%\tilde{\alpha}_{\pi, \psi} \geq c_d \epsilon^{2} \frac{2^{-4\ell_\varepsilon} \ell_\epsilon^{\frac{d}{2}}}{(4^{\ell_\epsilon} \ell_\epsilon^{2d-1})^{\frac12}} =  c_d \epsilon^{2} 2^{-5\ell_\epsilon} \ell_\epsilon^{- \frac12d +1} =  c_d \epsilon^{\frac{9}{2}} |\log_2(\epsilon)|^{-\frac{19d}{4}+\frac94}.
%\end{equation}
%\emph{First case: $M_p=M$}. We select $M_p =M$, for $p=1, \cdots, P$ with $M$ satisfying
%$$
%e^{-2 \gamma_1 \tilde{\alpha}_{\pi,\psi} \frac{2^{1-\rho}-1}{2^{1-\rho}(1-\rho)} M^{1-\rho}}  = \epsilon^4 |\log_2(\epsilon)|^{1-3d}
%$$
%\noindent that is
%$$
%M^{1-\rho} = \frac{2}{c_d\gamma_1\frac{2^{1-\rho}-1}{2^{1-\rho}(1-\rho)}} \frac{\log_2(\epsilon^{-1})}{\epsilon^{\frac{9}{2}} |\log_2(\epsilon)|^{-\frac{d}{2}+1}}= \frac{2^{2-\rho}(1-\rho)}{c_d \gamma_1 (2^{1-\rho}-1)} \epsilon^{-\frac{9}{2}} \log(\epsilon^{-1})^{\frac d2}.
%$$
%It thus suffices to set
%$$
%M = \lceil( \frac{2^{2-\rho}(1-\rho)}{c_d \gamma_1 (2^{1-\rho}-1)} \epsilon^{-\frac{9}{2}} \log(\epsilon^{-1})^{\frac d2})^{\frac{1}{1-\rho}}\rceil.
%$$
%With the above choice and using the fact that $\rho > 1/2$, we check 
%$$
%\frac{1}{M^{\rho}} \leq \epsilon^{\frac92 \frac{\rho}{1-\rho}}  \frac{1}{\log_2(\epsilon^{-1})^{\frac{d}{2} \frac{\rho}{1-\rho}}} \leq  \epsilon^4 |\log_2(\epsilon)|^{1-3d}.
%$$
%The overall complexity $\cC_\epsilon$ to  reach the precision $O_d(\epsilon^2)$ is then, recall Remark \ref{re num complexity direct algo}
%\begin{align*}
%\cC_\epsilon &= P_\epsilon N_\epsilon K_\epsilon M_\epsilon
%\\
%&= O_d(\log(\epsilon^{-1}) \epsilon^{-2} \epsilon^{-\frac12} \log(\epsilon^{-1})^{\frac74 d - \frac54} \epsilon^{-\frac92 \frac{1}{1-\rho}} \log(\epsilon^{-1})^{\frac{d}{2(1-\rho)}})\\
%& = O_d(\epsilon^{-\frac12[5+\frac{9}{1-\rho}]} \log(\epsilon^{-1})^{\frac{7}{4}d+\frac{d}{2(1-\rho)}-\frac{1}{4}})
%\end{align*}
%Under the constraint $\rho>1/2$, setting $\rho = \frac{1}{2} [1+ \frac{\mu}{9+\mu}]$, for any $\mu>0$, we thus get the optimal complexity
%$$
%\cC_\epsilon = O_d(\epsilon^{-\frac{23}{2}-\mu}\log(\epsilon^{-1})^{q_{d, \mu}})
%$$
%\noindent with $q_{d, \mu} = \frac{7}{4}d+\frac{d}{2(1-\rho)}-\frac{1}{4} \rightarrow \frac{11}{4}d-1$ as $\mu \downarrow 0$.\\
%\newline
%\emph{Second case:} We treat the sequence $M_p$, for $p=1, \cdots, P$ as real variables. We want to minimize the total complexity $\sum_{p=1}^{P} M_p$ under the constraint $\sum_{p=1}^{P} \delta^{P-p}M_p^{-\rho} = \epsilon^4 \log_2(\epsilon)^{1-3d}$.  Writing the two first order conditions for the Lagrangian, we obtain
%\begin{align*}
%M_p &= \rho^{\frac{1}{1+\rho}} [\delta^{P-p} \lambda]^{\frac{1}{1+\rho}}, \\
% \lambda & = [\epsilon^{-4}\log_2(\epsilon^{-1})^{3d-1}\rho^{-\frac{\rho}{1+\rho}} \sum_{p=1}^{P} (\delta^{\frac{1}{1+\rho}})^{P-p}]^{\frac{1+\rho}{\rho}}  
%\end{align*}
%\noindent which in turn implies
%$$
%M_p = \delta^{\frac{P-p}{1+\rho}} [\sum_{p=1}^P \delta^{\frac{P-p}{1+\rho}}]^{\frac{1}{\rho}} [\epsilon^{-4}\log_2(\epsilon^{-1})]^{\frac1\rho}.
%$$
%However, because of the second term in the sum appearing on the left hand side of \eqref{constraint:optimize:M:sequence}, the constraint \eqref{constraint:optimize:M:sequence} is not satisfied. Indeed, from \eqref{lower:bound:alpha}, we get 
%$$
%-2 \gamma_1\tilde{\alpha}_{\pi,\psi} \frac{2^{1-\rho}-1}{2^{1-\rho}(1-\rho)} M_{P-p}^{1-\rho} \leq -C(\gamma_1, \rho, d) \epsilon^{\frac{9}{2}} (\log_2(\epsilon^{-1}))^{-\frac{19d}{4}+\frac94} \epsilon^{-4\frac{1-\rho}{\rho}} \log_2(\epsilon^{-1})^{\frac{1-\rho}{\rho}}
%$$
%\noindent with $C(\gamma_1, \rho, d) = 2\gamma_1\frac{2^{1-\rho}-1}{2^{1-\rho}(1-\rho)}  c_d  \delta^{\frac{p(1-\rho)}{1+\rho}}  [\sum_{p=1}^P \delta^{\frac{P-p}{1+\rho}}]^{\frac{1-\rho}{\rho}}$. Since $\rho>1/2$, the above right-hand side goes to zero as $\epsilon \downarrow 0$ so that the constraint cannot be satisfied.\\
%\eproof
%\end{yellowtext}


==> v4.33 - arXiv submission/intro.tex <==
%!TEX root = main.tex
\section{Introduction}
%\begin{bluetext}
In the present work, we are interested in the numerical approximation in high dimension of the solution to the semilinear parabolic PDE
\begin{equation}
\label{eq pde}
\left\{
\begin{array}{ll}
\partial_t u(t, x) + \mathcal{L} u(t, x) + f(u(t,x), \sigma^{\top}(x)\nabla_x u(t, x))  =0, &   (t, x) \in [0,T) \times \mathbb{R}^d, \\
 u(T, x) = g(x), \quad x \in \mathbb{R}^d  & 
\end{array}
\right.
\end{equation}

\noindent where $f: \mathbb{R} \times \mathbb{R}^d \rightarrow \mathbb{R}$, $g: \mathbb{R}^d \rightarrow \mathbb{R}$ are measurable functions and $\mathcal{L}$ is the infinitesimal generator of the forward diffusion process with dynamics 
\begin{equation}%\label{eq de diffusion X}
\ud \cX_t  = b(\cX_t) \ud t +    \sigma(\cX_t) \ud \cW_t \, \label{eq forward sde}
\end{equation}

\noindent and defined, for a smooth function $\varphi$, by
\begin{equation}
\label{infinitesimal:operator:diffusion}
\mathcal{L} \varphi(t, x) :=  b(x)\cdot \nabla_x \varphi(t, x) +\frac12 \mathrm{Tr}[(\sigma\sigma^{\top})(x)\nabla^2_x \varphi(t, x)].
\end{equation}
\noindent Here, $\cW$ is a $d$-dimensional brownian motion defined on a complete probability space $(\mathfrak{O}, \cA,\P)$, $b : \R^d \rightarrow \R^d$ and $\sigma: \R^d \rightarrow \cM_d$ are measurable functions, $\cM_d$ being the set of $d\times d$ matrix. 
The initial condition $\cX_0$ is a square integrable random variable independent from the Brownian Motion $\cW$.
We denote by $(\mathcal{F}_{t})_{0\leq t \leq T}$ the  filtration generated by $\cW$ and $\cX_0$, augmented with $\P$ null sets. 
 
Developing efficient algorithms for the numerical approximation of high-dimensional non-linear PDEs is a challenging task that has attracted considerable attention from the research community in the last two decades.
We can quote various approaches (limiting to the "stochastic" ones) that have proven to be efficient in a high dimensional setting: branching methods, see e.g. \cite{henry-labordere2019}, machine learning methods (especially using deep neural networks), see e.g. \cite{Han8505}, and full history recursive multilevel Picard method (abbreviated MLP in the literature) see e.g. \cite{ewhutzenthaler2016multilevel}. This is a very active field of research, we refer to the recent survey papers \cite{weinan2020algorithms,beck2020overview} for more references and an overview of the numerical and theoretical results available.
We focus now more on one stream of research which uses the celebrated link between semilinear parabolic PDEs of the form \eqref{eq pde} and BSDEs. This connection, initiated in \cite{Pardoux:Peng:90}, reads as follows: denoting by $u$ a classical solution to \eqref{eq pde}, $(u(t, \cX_t), \sigma^{\top}(\cX_t) \nabla_x u(t, \cX_t))  = (\cY_t, \cZ_t)$ where the pair $(\cY, \cZ)$ is the $\mathbb{R}\times \mathbb{R}^d$-valued and $(\mathcal{F}_{t})$-adapted process solution to the BSDE with dynamics
\begin{align}
\cY_t & = g(\cX_T) + \int_t^Tf(\cY_s,\cZ_s) \ud s - \int_t^T \cZ_s \cdot \ud \cW_s\,,\;0\le t \le T\,,
\label{eq backward sde}
\end{align} 
so that, the original problem boils down to the numerical approximation of the above stochastic system. 
%{\color{blue} 
Various strategies have been used to numerically approximate the stochastic system $(\cX_t, \cY_t, \cZ_{t})_{t \in [0,T]}$. The most studied one is based on a time discretization of \eqref{eq backward sde} leading to a backward programming algorithm to approximate $(Y,Z)$, as exposed in e.g \cite{BOUCHARD2004175, zhang2004numerical} (see the references therein for early works). This involves computing a sequence of conditional expectations and various methods have been developed: Malliavin calculus based methods \cite{BOUCHARD2004175, CRISAN, hu2011}, optimal quantization methods \cite{BALLY20031,bally2003,PAGES2018847}, cubature methods \cite{crisan2012solving,crisan2014second,chassagneux2020cubature} and (linear) regression methods, see among others \cite{gobet2005regression, gobet2016approximation, gobet2016stratified}. It is acknowledged that such approaches will be feasible for problems up to dimension 10. This limitation is a manifestation of the so-called ``curse of dimensionality''. Recently, non-linear regression methods using deep neural networks were succesfuly combined with this approach and proved to be capable of tackling problems in high dimension \cite{hure2020deep}. However, other strategies have been introduced in the last five years or so to approximate \eqref{eq backward sde} trying to adopt a "forward point of view". Relying on Wiener chaos expansion and Picard iteration,  \cite{briand2014simulation, geiss2016simulation} introduced a method  that notably works in non-Markovian setting  but is still impacted by the curse of dimension. A key step forward has been realized by the so called \emph{deep BSDEs solver} introduced in \cite{Han8505}. Interpreting the resolution of a BSDEs as an optimisation problem, it relies on the expressivity of deep neural network and well established SGD algorithms to show great performance in practice. 
More precisely, in this approach, the $\cY$-process is now interpreted as a forward SDE controlled by the $\cZ$-process. Then, an Euler-Maruyama approximation scheme is derived in which the derivative of the solution $u$ appearing in the non-linear function $f$ (through the $\cZ$-process) is approximated by a multi-layer neural network. The optimal weights are then computed by minimizing the mean-squared error between the value of the approximation scheme at time $T$ and a good approximation of the target $g(\cX_T)$ using stochastic gradient descent algorithms. Again, this kind of deep learning technique seems to be very efficient to numerically approximate the solution to semi-linear parabolic PDEs in practice. However a complete theory concerning its theoretical performance is still not achieved \cite{beck2020overview}. One important observation is that, due to highly non-linear specification, the optimisation problem that has to be solved in practice, has no convexity property. The numerical procedure designed can only converge to local minima, whose properties (with respect to the approximation question) are still not completely understood. 

Inspired by this new forward approach, we introduce here an algorithm which is shown to converge to a global minimum. This, of course, comes with a price. First, we move from the deep neural networks approximation space to a more classical linear specification of the approximation space. However, due the non-linearity in the BSDE driver, the global optimisation problem to be solved is still non-convex. To circumvent this issue, we employ a \emph{Picard iteration procedure}. The overall procedure becomes then a sequence of linear-quadratic optimisation problems which are solved by a SGD algorithm. {Our first main result is a control of the global error between the \emph{implemented algorithm} and the solution to the BSDE which notably shows the convergence of the method under some smallness conditions, see Theorem \ref{th main conv result}. In particular, contrary to \cite{Han8505, han2020convergence} or \cite{hure2020deep}, our result takes into account the error induced by the SGD algorithm. In our numerical experiments, we rely on sparse grid approximation spaces which are known to be well-suited to deal with high-dimensional problems. Under the framework of periodic coefficients, we establish  as our second main result, an upper bound on the global complexity for our \emph{implemented algorithm}, see Theorem \ref{thm full complexity}. We notably prove that the curse of dimensionality is tamed in the sense that the complexity is of order $\varepsilon^{-p} |\log(\varepsilon)|^{q(d)}$, where $p$ is a constant which does not depend on the PDE dimension and $d\mapsto q(d)$ is an affine function. We also demonstrate numerically the efficiency of our methods in high dimensional setting.}      
%}





The rest of the paper is organized as follows. In \Cref{Description of the numerical methods}, we first recall the \emph{deep BSDEs solver} of \cite{Han8505} but adapted to our framework. Namely, we use  a linear specification of the approximation space together with SGD algorithms. For sake of clarity, we denote this method: the \emph{direct algorithm}. Then, we introduce our new numerical method : the \emph{Picard algorithm}. We present our main assumptions on the coefficients and state our main convergence results. In \Cref{se main sparse grids}, we use sparse grid approximation with the \emph{direct and Picard algorithms}, using two types of basis functions: pre-wavelet \cite{bohn2018convergence} and modified hat function \cite{frommert2010efficient}. We discuss their numerical performances in practice through various test examples. We also compare them with some deep learning techniques \cite{Han8505,hure2020deep}. We also state our main theoretical complexity result. \Cref{study:optimization:problem} is devoted to the theoretical analysis required to establish our main theorems: all the proofs are contained in this section. Finally, we give a complete list of the algorithm parameters that have been used to obtain the numerical results in Appendix.




\paragraph{Notation:}
Elements of $\R^q$ are seen as column vectors. For $x\in\R^q$, $x_i$ is the $i$th component and $|x|$ corresponds to its Euclidian norm, $x \cdot y$ denotes the scalar product of $x$ and $y \in \R^q$. $\cM_q$ is the set of $q \times q$ real matrices. We denote by $\mathbf{e}^\ell$ the $\ell$th vector of the standard basis of $\R^q$. The vector $(1,\dots,1)^\top$ is denoted $\mathbf{1}$, $\mathrm{I}_d$ is the $d \times d$ identity matrix. We use the bold face notations $\bold{l} \in \mathbb{N}^{d}$ for multidimensional indices $\bold{l}:=(l_1, \cdots, l_d)$ with (index) norms denoted by $|\bold{l}|_{p}:=(\sum_{i=1}^{d} l_i^{p})^{1/p}$ and $|\bold{l}|_{\infty} := \max_{1\leq i \leq d} | l_i|$. For later use, for a positive integer $k$, we introduce the set $\mathbf{J}^\infty_{d, k}$ of multidimensional indices $\bold{l} \in \mathbb{N}^{d}$ satisfying $|\bold{l}|_{\infty} \leq k$.
For a finite set $A$, we denote by $|A|$ its cardinality. 

For a function $f:\R^d \rightarrow \R$, we denote by $\partial_{x_l} f$ the partial derivative function with respect to $x_l$, $\nabla f$ denotes the gradient function of $f$, valued in $\R^d$. We also use $\nabla^2 f = (\partial^2_{x_i, x_j} f)_{1\leq i, j \leq d}$ to denote the Hessian matrix of $f$, valued in $\cM_d$. For a sufficiently smooth real-valued function $f$ defined in $\mathbb{R}^d$, we let $D^{\bold{l}} f = \partial^{l_1}_{x_1}\cdots \partial^{l_d}_{x_d} f$ denote the differentiation operator with respect to the multi-index $\bold{l} \in \mathbb{N}^d$. For a fixed positive integer $k$ and a function $f$ defined on an open domain $ \mathcal{U} \subset \mathbb{R}^d$, we define its Sobolev norm of mixed smoothness
\begin{equation}
\label{H2:Sobolev:norm:mixed:smoothness}
\|f\|_{H^{k}_{mix}(\mathcal{U})} := \Big(\sum_{\bold{l} \in \mathbf{J}^\infty_{d, k} } \|D^{\bold{l}}f\|^2_{L_2(\mathcal{U})} \Big)^{\frac12}
\end{equation}

\noindent where the derivative $D^{\bold{l}}f$ in the above formula has to be understood in the weak sense and for a map $g:\mathcal{U} \mapsto \mathbb{R}$, $\|g\|^2_{L^2(\mathcal{U})} := \int_{\mathcal{U}} |g(x)|^2 dx$. The Sobolev space of mixed smoothness $H^{k}_{mix}(\mathcal{U})$ is then defined by 
\begin{equation}\label{Sobolev:space}
H^{k}_{mix}(\mathcal{U}) := \left\{ f \in L_2(\mathcal{U}) : \|f\|_{H^{k}_{mix}(\mathcal{U})} <\infty\right\}.
\end{equation}


For a positive integer $q$, the set $\cH^2_q$  is the set of progressively measurable processes $V$ defined on the probability space $(\mathfrak{O}, \cA,\P)$ with values in $ \mathbb{R}^q$ and satisfying $\esp{ \int_0^T |V_t|^2 \ud t}<+\infty$. The set $\cS^2_q$  is the set of adapted càdlàg processes $U$ defined on the probability space $(\mathfrak{O}, \cA,\P)$ with values in $ \mathbb{R}^q$ and satisfying $\esp{\sup_{t\in[0,T]}|U_t|^2} <+\infty$. We also define $\cB^2 := \cS^2_1\times \cH^2_d$.



==> v4.33 - arXiv submission/picard.tex <==
%!TEX root = main.tex

\subsection{Study of the \emph{Picard algorithm}} 
 \label{Study of the Picard algorithm}

%We measure the efficiency of our global algorithm by upper bounding the MSE: $\esp{|y^P_M - u(0,x)|^2}$, recall Definition \ref{de picard scheme empirical}.
%\\
%\textcolor{red}{place before?}
%We shall compare the (random) output of the Picard algorithm with a reference solution $\bar{\mathfrak{u}} = (\bar{y},\bar{\mathfrak{z}})$, with $\bar{y} := u(0,x)$, $\bar{\mathfrak{z}^1_0} = \partial_{x}u(0,x)$ and the other $\bar{\mathfrak{z}}$ coefficients are given by the unique decomposition of $\partial_x u(t_n,\cdot)$ in 
%$ \bigoplus_{\mathbf{l} \in \mathbb{N}^d} \mathscr{W}_{\mathbf{l}}$ truncated to the level $\ell_n$ considered for the approximation space $\mathscr{V}_n$, $1 \le n \le N-1$. In particular, we define
%\begin{align}
%\R^d \ni x \mapsto \bar{v}_n(x) = \sum_{k = 1}^{K_n} \bar{\mathfrak{z}}^{n,k} \psi_{n,k}(x) \in \R^d\;.
%\end{align}
%\textcolor{red}{redefinir $\bar{v}$ to obtain precisely the equality with $\cE_\psi$...}
We introduce the following mean squared error:
\begin{align}\label{eq de error picard}
\cE_p := \esp{\vvvert \mathfrak{u}^p_M - \bar{\mathfrak{u}} \vvvert^2}\,, 0 \le p \le P\,,
\end{align}
where the sequence $(\mathfrak{u}^{p}_{M})_{0\leq p \leq P}$ is given by Definition \ref{de picard scheme full}, $\vvvert\cdot\vvvert$ is given by Definition \ref{de double - triple norm} and $\bar{\mathfrak{u}}$ is the reference solution introduced in \eqref{the:reference:solution}. In this subsection, our aim is to establish an upper bound for the quantity $\cE_P$ that will allow us to prove Theorem \ref{th main conv result}.
%Note  that in particular,  $\cE_P  \ge \esp{|y^P_M - u(0,x_0)|^2}$, recall \eqref{de triple norm}.
%\begin{align*}
%\vvvert (y,\mathfrak{z}) \vvvert^2 = |y|^2 + \sum_{n=0}^{N-1}h\esp{|Z^\mathfrak{z}_n|^2} \text{ with } Z^\mathfrak{z}_n = \sum_{k=1}^{K_n} \mathfrak{z}^k_n \partial_x \phi^k_n(W_{t_n})\;.
%\end{align*}


\subsubsection{Preliminary estimates}

%\textcolor{red}{comments}

\begin{Proposition} \label{error of Picard}
%\textcolor{red}{has to be improved ? see next section Prop \ref{error of Picard sharper}}
Suppose that Assumption \ref{ass X0}, Assumption \ref{assumption:coefficient} (i), (ii) and Assumption \ref{as psi function} hold. If $T(1+ 2L^2(1+ h)) < 1$ and
$\delta_h:=\frac{ 8 L^2 T}{1-T(1+ 2L^2(1+ h))} < 1$, then for any $\varepsilon>0$ such that $\delta_{h,\varepsilon}:= \delta_h (1+\varepsilon)<1$ there exists a positive constant $C_\varepsilon$ such that for any positive integer $P$
\begin{align}
\cE_P \le \delta_{h,\varepsilon}^P \cE_0 +  C_\varepsilon \big( \cE_{\mathrm{RM}}  + \cE_{\psi} +  \cE_{\pi} \big)
\end{align}
\noindent with the notation
\begin{align}
\cE_{\mathrm{RM}} := \max_{1 \le p \le P}\esp{ \vvvert \mathfrak{u}^{p}_{M} - \Phi(\mathfrak{u}^{p-1}_{M}) \vvvert^2}.
\end{align}
%\noindent where $\mathfrak{u}^{p}_{M}$ is given by Definition \ref{de picard scheme full}.
\end{Proposition}


\proof 
From the decomposition, 
\begin{align*}
\mathfrak{u}^p_{M}- \bar{\mathfrak{u}} = &\Phi_{M}(\mathfrak{u}^{p-1}_{M}) - \Phi(\mathfrak{u}^{p-1}_{M}) + \Phi(\mathfrak{u}^{p-1}_{M})  -  \bar{\mathfrak{u}} 
\end{align*}
\noindent we obtain, for any $\varepsilon > 0$,
\begin{align*}
\cE_p \le (1+ \frac1\varepsilon)\cE_{\mathrm{RM}} + (1+\varepsilon)\esp{ \vvvert \Phi(\mathfrak{u}^{p-1}_{M})  -  \bar{\mathfrak{u}}  \vvvert^2}.
\end{align*}
Then, using Lemma \ref{le control f(y,z)} below, we get
\begin{align*}
\cE_p \le \delta_{h,\varepsilon} \cE_{p-1} +  C_\varepsilon \left(  \cE_{\psi} + \cE_{\pi}  + \cE_{\mathrm{RM}}  \right)
\end{align*}
\noindent up to a modification of $\varepsilon$. By an induction argument, we  derive
\begin{align*}
\cE_P \le \delta_{h,\varepsilon}^P \cE_0 +  C_\varepsilon \big( \cE_{\mathrm{RM}} + \cE_{\psi} +  \cE_{\pi} \big)
\end{align*}
which concludes the proof.
\eproof



\begin{Lemma}  \label{le control f(y,z)}
Suppose that Assumption \ref{ass X0}, Assumption \ref{assumption:coefficient} (i), (ii) and Assumption \ref{as psi function} hold. If $T(1+ 2L^2(1+ h)) < 1$ and
$\delta_h:=\frac{ 8 L^2 T}{1-T(1+ 2L^2(1+ h))} < 1$, then, for any $\varepsilon>0$ there exists a positive constant $C_\varepsilon$ ($\varepsilon \mapsto C_\varepsilon$ being non-increasing) such that for any $\tilde{\mathfrak{u}} \in  \R^{K^y}\times \R^{d\bar{K}^z}$  it holds 
\begin{align*}
\vvvert \Phi(\tilde{\mathfrak{u}})  -  \bar{\mathfrak{u}} \vvvert^2
\le \delta_{h}(1+\varepsilon) \vvvert \tilde{\mathfrak{u}}  -  \bar{\mathfrak{u}} \vvvert^2
+  C_\varepsilon \left(  \cE_{\psi} + \cE_{\pi}  \right).
\end{align*}
%with $\delta_{h,\varepsilon} :=  \delta_h (1+\varepsilon)$, 
%  $\bar{\mathfrak{u}}$ defined by \eqref{the:reference:solution}.
\end{Lemma}


%\begin{bluetext}
\proof 

\emph{Step 1:} We  denote $\check{\mathfrak{u}} = \Phi(\tilde{\mathfrak{u}})  $ where
$\check{\mathfrak{u}} = (\check{\mathfrak{y}},\check{\mathfrak{z}})$ and $\tilde{\mathfrak{u}} = (\tilde{\mathfrak{y}},\tilde{\mathfrak{z}})$ belongs to $\mathbb{R}^{K^y} \times \mathbb{R}^{d \bar{K}^z}$. We first observe that, recalling \eqref{eq de Phi}, \eqref{eq rewritte norms} and \eqref{eq de U starting point},
\begin{align*}
\vvvert \Phi(\tilde{\mathfrak{u}})  -  \bar{\mathfrak{u}} \vvvert^2 &=
\esp{ |Y^{\bar{\mathfrak{u}}}_0-Y^{\check{\mathfrak{u}}}_0|^2 + \int_0^T |Z^{\check{\mathfrak{u}}}_{t}-Z^{\bar{\mathfrak{u}}}_{t}|^2 \ud t}
%\\
%& \le \esp{\sup_{t \in [0,T]} |U^{(\tilde{y},\tilde{\mathfrak{z}}),(\tilde{\tilde{y}},\tilde{\tilde{\mathfrak{z}}})}_t
%- U^{(\tilde{y},\tilde{\mathfrak{z}}),(\bar{y},\bar{\mathfrak{z}})}_t
%|^2 + \int_0^T |Z^{\tilde{\tilde{\mathfrak{z}}}}_{\bar{t}}-Z^{\bar{\mathfrak{z}}}_{\bar{t}}|^2 \ud t } 
\\
&=  \esp{|U^{\tilde{\mathfrak{u}}, \check{\mathfrak{u}}}_T
- U^{\tilde{\mathfrak{u}},\bar{\mathfrak{u}}}_T|^2}.
\end{align*}
%\textcolor{red}{Bckwd estimate - arbitrary time in fact doob...}
%\\
Moreover, by optimality of $\check{\mathfrak{u}}$
\begin{align*}
\esp{|U^{\tilde{\mathfrak{u}},\check{\mathfrak{u}} }_T
- U^{\tilde{\mathfrak{u}},\bar{\mathfrak{u}}}_T|^2}
&\le 
2 \left(
\esp{|U^{\tilde{\mathfrak{u}},\check{\mathfrak{u}} }_T
- g({X}_T)|^2}
+
\esp{|g({X}_T)
- U^{\tilde{\mathfrak{u}},\bar{\mathfrak{u}}}_T|^2}
\right)
\\
&\le 4 \esp{|g({X}_T)
- U^{\tilde{\mathfrak{u}},\bar{\mathfrak{u}}}_T|^2}.
\end{align*}

We now compute, for any $\varepsilon > 0$,
\begin{align*}
\esp{|g({X}_T)
- U^{\tilde{\mathfrak{u}},\bar{\mathfrak{u}}}_T|^2}
\le
(1+\frac1\varepsilon)
\esp{|g({X}_T)
- U^{\bar{\mathfrak{u}},\bar{\mathfrak{u}}}_T|^2}
+
(1+\varepsilon)\esp{|U^{\bar{\mathfrak{u}},\bar{\mathfrak{u}}}_T
- U^{\tilde{\mathfrak{u}},\bar{\mathfrak{u}}}_T|^2}\,,
\end{align*}
which, combined with the previous inequality, yields
\begin{align} \label{eq end step 1}
 \vvvert \Phi(\tilde{\mathfrak{u}})  -  \bar{\mathfrak{u}} \vvvert^2  \le 4(1+\frac1\varepsilon)
\esp{|g({X}_T)
- U^{\bar{\mathfrak{u}},\bar{\mathfrak{u}}}_T|^2}
+
4(1+\varepsilon)\esp{|U^{\bar{\mathfrak{u}},\bar{\mathfrak{u}}}_T
- U^{\tilde{\mathfrak{u}},\bar{\mathfrak{u}}}_T|^2}\,.
\end{align}
Since $U^{\bar{\mathfrak{u}},\bar{\mathfrak{u}}} = Y^{\bar{\mathfrak{u}}}$, we can give an upper bound for the first term appearing on the right-hand side of the above inequality by using \eqref{eq co bound error ref solution},
\begin{align}\label{eq bias part}
\esp{|g({X}_T)
- U^{\bar{\mathfrak{u}},\bar{\mathfrak{u}}}_T|^2} = \mathfrak{g}(\bar{\mathfrak{u}})
\le C \left(  \cE_{\psi} + \cE_{\mathrm{\pi}}  \right).
\end{align}
\emph{Step 2: } %\textcolor{red}{continous version used here} 
We now turn to the study of the second term appearing on the right hand side of \eqref{eq end step 1}.
%\begin{align*}
%U^{\tilde{\mathfrak{u}},\bar{\mathfrak{u}}}_t & = 
%\bar{y} -\int_0^t f(Y^{\tilde{\mathfrak{u}}}_{\bar{s}},Z^{\tilde{\mathfrak{u}}}_{\bar{s}}) \ud s + \int_0^t Z^{\bar{\mathfrak{u}}}_{\bar{s}} \ud W_s\;,
%%\\
%%U^{\bar{\mathfrak{u}},\bar{\mathfrak{u}}}_t & = 
%%\bar{y} -\int_0^t f(Y^{\bar{\mathfrak{u}}}_{\bar{s}},Z^{\bar{\mathfrak{z}}}_{\bar{s}}) \ud s + \int_0^t Z^{\bar{\mathfrak{z}}}_{\bar{s}} \ud W_s 
%\end{align*}
%with
%\begin{align*}
%Y^{\tilde{\mathfrak{u}}}_{t} &=
%\tilde{y} - \int_0^t f(Y^{\tilde{\mathfrak{u}}}_{\bar{s}},Z^{\tilde{\mathfrak{u}}}_{\bar{s}}) \ud s + \int_0^t Z^{\tilde{\mathfrak{u}}}_{\bar{s}} \ud W_s \;.
%%\\
%%Y^{\bar{\mathfrak{u}}}_{t} &=
%%\bar{y} - \int_0^t f(Y^{\bar{\mathfrak{u}}}_{\bar{s}},Z^{\bar{\mathfrak{z}}}_{\bar{s}}) \ud s + \int_0^t Z^{\bar{\mathfrak{z}}}_{\bar{s}} \ud W_s
%\end{align*}
Recalling the dynamics \eqref{eq scheme picard}, denoting $\delta U := U^{\tilde{\mathfrak{u}},\bar{\mathfrak{u}}} - Y^{{\bar{\mathfrak{u}}}} $, $\delta Z = Z^{\tilde{\mathfrak{u}}}-Z^{\bar{\mathfrak{u}}}$, $\delta Y  = Y^{\tilde{\mathfrak{u}}} - Y^{\bar{\mathfrak{u}}}$ and $\delta f_{t_n} = f(Y^{\tilde{\mathfrak{u}}}_{t_n}, Z^{\tilde{\mathfrak{u}}}_{t_n}) - f(Y^{\bar{\mathfrak{u}}}_{t_n}, Z^{\bar{\mathfrak{u}}}_{t_n})$, $0\leq n \leq N-1$, using the Cauchy-Schwarz inequality and the Lipschitz-regularity of the map $f$, we get
\begin{align}
\esp{|\delta U_T|^2} &\le T\int_0^T\esp{|\delta f_{\bar{s}}|^2} \ud s  \le 2L^2 T \sum_{n=0}^{N-1}h \esp{|\delta Y_{t_n}|^2 + |\delta Z_{t_n}|^2} \ud s. 
\label{eq first upper bound}
\end{align}
For all $0 \leq n \le N-1$, one has
\begin{align*}
\delta Y_{t_{n+1}}  =& \delta Y_{t_n} - h \delta f_{t_n} + \delta Z_{t_n} \Delta W_n
\end{align*}

\noindent which in turn, setting $\Delta M_n := 2(\delta Y_{t_n} - h \delta f_{t_n}) \delta Z_{t_n} \Delta W_n$, yields
\begin{align*}
|\delta Y_{t_{n+1}}|^2 = |\delta Y_{t_n}|^2 - 2 h \delta Y_{t_n} \delta f_{t_n} + h^2 |\delta f_{t_n} |^2 + | \delta Z_{t_n} \Delta W_n|^2 + \Delta M_n.
\end{align*}
Using the fact that $\mathbb{E}[\Delta M_n]=0$ and the Lipschitz regularity of the map $f$, we deduce
\begin{align*}
\esp{|\delta Y_{t_{n+1}}|^2} & \leq \esp{|\delta Y_{t_n}|^2 + h |\delta Y_{t_n}|^2 +  (h+ h^2) |\delta f_{t_n} |^2 + h | \delta Z_{t_n}|^2}\\
& \leq  \esp{|\delta Y_{t_n}|^2 + (h + 2L^2(h+ h^2) )  (|\delta Y_{t_n}|^2 + | \delta Z_{t_n}|^2)}.
\end{align*}
Summing the previous inequality, we obtain
\begin{align*}
\esp{|\delta Y_{t_{n}}|^2}  \le |\delta Y_{0}|^2 + \esp{\sum_{j=0}^{N-1}(h + 2L^2(h+ h^2) ) (|\delta Y_{t_j}|^2 + | \delta Z_{t_j}|^2)}
\end{align*}
so that, multiplying both side of the previous inequality by $h$ and summing again, we get
\begin{align*}
\sum_{n=0}^{N-1}h\esp{|\delta Y_{t_{n}}|^2} & \le T|\delta Y_{0}|^2 + T(1+ 2L^2(1+ h)) \left(\mathbb{E}\Big[\sum_{j=0}^{N-1}h |\delta Y_{t_j}|^2\Big] + \mathbb{E}\Big[\sum_{j=0}^{N-1}h | \delta Z_{t_j}|^2\Big] \right)
\\
& 
\le \frac{T}{1-T(1+ 2L^2(1+ h))} \left( |\delta Y_{0}|^2 + (1+ 2L^2(1+ h))\mathbb{E}\Big[\sum_{j=0}^{N-1}h | \delta Z_{t_j}|^2\Big] \right)
\end{align*}

\noindent where, for the last inequality, we used the fact that $T(1+ 2L^2(1+ h))<1$. Combining the previous inequality with \eqref{eq first upper bound}, we obtain
\begin{align}\label{eq end step 3}
\esp{|\delta U_T|^2}
%&\le 2L^2 T\left( \frac{T}{1-T(1+ 2L^2(1+ h))} \left( |\delta Y_{0}|^2 + (1+ 2L^2(1+ h))\esp{\sum_{j=0}^{N-1}h | \delta Z_{t_j}|^2} \right)+ \sum_{n=0}^{N-1} \esp{h|\delta Z_{t_n}|^2} \right)
%\\
&\le
  \frac{2L^2 T}{1-T(1+ 2L^2(1+ h))}  \left( T  |\delta Y_{0}|^2
+
 \sum_{n=0}^{N-1} h\esp{|\delta Z_{t_n}|^2}
\right).
\end{align}
%4. Set $\epsilon$ such that
%$$ \delta = 4(1+\epsilon)\frac{2L^2 T}{1-T(1+ 2L^2(1+ h))} < 1,$$
We finally complete the proof by combining \eqref{eq end step 1}, \eqref{eq bias part} and \eqref{eq end step 3}.
%
%\begin{align*}
%|\delta Y_t|^2  =& |\delta Y_0|^2 
%- 2 \int_0^t \delta Y_s \delta f_{\bar{s}}\ud s + \int_0^t |\delta Z_{\bar{s}}|^2 \ud s
%+2 \int_0^t \delta Y_s \delta Z_{\bar{s}}\ud W_s\;.
%\end{align*}
%Taking expectation on both sides of the previous equality and using Young's inequality, we get
%\begin{align*}
%\esp{|\delta Y_t|^2} \le |\delta Y_0|^2 + \alpha \int_0^t \esp{|\delta Y_{\bar{s}}|^2} \ud s + \frac{1}{\alpha} \int_0^t \esp{|\delta f_{\bar{s}}|^2} \ud s +  \int_0^t \esp{|\delta Z_{\bar{s}}|^2} \ud s
%\end{align*}
%leading to
%\begin{align*}
%\int_0^T\esp{|\delta Y_t|^2} \ud t \le    \frac{T}{1-\alpha T} \left( |\delta Y_0|^2   + \frac{1}{\alpha} \int_0^T \esp{|\delta f_{\bar{s}}|^2} \ud s +  \int_0^T \esp{|\delta Z_{\bar{s}}|^2} \ud s \right)
%\end{align*}
\eproof
%\end{bluetext}


%\begin{yellowtext}
%\subsubsection{Error of the Robbins-Monro Procedure}
%
%\noindent
% We now present some results related to the stochastic gradient descent algorithm stemming from the local gradient function $H(W, \tilde{\mathfrak{u}}, .) = (H_1(W, \tilde{\mathfrak{u}},.), H_2(W, \tilde{\mathfrak{u}}, .))$ given by \eqref{H1:generic:function}-\eqref{H2:generic:function}, namely
%  \begin{align}
%  y_{m+1} & = y_{m} - \gamma_{m+1} H_1(W^{(m+1)}, \tilde{\mathfrak{u}}, y_m),  \label{dynamics:sg:y} \\
%  \mathfrak{z}_{m+1} & = \mathfrak{z}_m - \gamma_{m+1} H_2(W^{(m+1)}, \tilde{v}, \mathfrak{z}_m) \label{dynamics:sg:theta}
%  \end{align}
%  \noindent where the r.v. $\mathfrak{z}_0$, $\cW = (W^{(m+1)})_{m\geq0}$ and $\tilde{\mathfrak{u}}$ are independent and $\mathfrak{z}_0 \in L^2(\mathbb{P})$.
%   We also recall that $\Omega=\Omega(W)$, $Z^{\tilde{\mathfrak{z}}} = Z^{\tilde{\mathfrak{z}}}(W) $ and  $Y^{\tilde{\mathfrak{u}}} = Y^{\tilde{\mathfrak{u}}} (W)$ are defined respectively by \eqref{eq de omega}, \eqref{eq de Z} and \eqref{eq de input picard Y}. 
%    The deterministic and positive sequence $(\gamma_m)_{m\geq1}$ also satisfies the usual assumption $\sum_{m\geq1} \gamma_m = \infty \quad \mbox{and} \quad \sum_{m\geq1} \gamma^2_m < \infty$. We here establish the a.s. convergence of the sequence $\left\{ \mathfrak{u}_{m} = (y_m, \mathfrak{z}_m), m\geq 0 \right\}$ towards the unique minimizer $\Phi(\tilde{\mathfrak{u}})=(y^{\star}(\tilde{\mathfrak{u}}), \mathfrak{z}^{*}(\tilde{\mathfrak{u}}))$ as well as an $L^{2}(\mathbb{P})$ convergence rate which is of main importance in order to study the global complexity of our algorithm.
% \begin{Lemma}\label{lem:stochastic:gradient}
%  Under assumption 1.1, \HYP{L} and \HYP{b}, the sequence $(\mathfrak{u}_{m})_{m\geq0}$ converges a.s. to  $\Phi(\tilde{\mathfrak{u}})$ as $m\uparrow \infty$. Moreover, the following $L^{2}(\mathbb{P})$ convergence rate holds: for any integer positive $m$,
%  \begin{equation}
%  \label{L2:control:ym}
%  \mathbb{E}_{\tilde{\mathfrak{u}}}[(y_m - y^{\star})^2] = \frac{\textnormal{Var}_{\tilde{\mathfrak{u}}}(g(W_T) - \sum_{n=0}^{N-1} h f(Y^{\tilde{\mathfrak{u}}}_{t_n}, Z^{\tilde{\mathfrak{u}}}_{t_n}))}{m} \leq \frac{ (|g|_\infty + T |f|_\infty)^2}{m}
%  \end{equation}
%  \noindent and
%  \begin{equation}
%  \label{L2:control:thetam}
%  \mathbb{E}_{\tilde{\mathfrak{u}}}[\| \mathfrak{z}_{m} - \mathfrak{z}^{\star}\|^2] \leq K \exp(-2 \tilde{\alpha}_{\pi, \psi} \Gamma_{m}) \esp{ \| \mathfrak{z}_{0} - \mathfrak{z}^\star\|^2 } + C_1 K  \sum_{\ell=1}^{m} \exp(-2 \tilde{\alpha}_{\pi, \psi} (\Gamma_{m}-\Gamma_{l})) \gamma^2_l
%  \end{equation}
%  \noindent where $\tilde{\alpha}_{\pi, \psi} = \alpha_{\pi, \psi} (1+\mathbb{E}[\|\bar{\Omega}\|^2])^{-\frac12}$, $\Gamma_m = \sum_{k=1}^{m} \gamma_k$, $C_0 := 8 (|g|_\infty + T |f|_\infty)^2\vee 1$, $C_1:=C_0(1+2 \|\mathfrak{z}^{\star}\|^2)$ and $K=\exp(2C_0 \sum_{l\geq1}\gamma^2_l)$.
% \end{Lemma}
% \begin{proof}
% \emph{Step 1: a.s. convergence.} First, applying the strong law of large of numbers, from the boundedness of $g$ and $f$, conditionally on $\tilde{\mathfrak{u}}$, the sequence $(y_m)_{m\geq0}$ converges $a.s.$ towards $y^{\star}(\tilde{\mathfrak{u}}) = \mathbb{E}_{\tilde{\mathfrak{u}}}[g(W_T) - \sum_{n=0}^{N-1} h f(Y^{\tilde{\mathfrak{u}}}_{t_n}, Z^{\tilde{\mathfrak{u}}}_{t_n})]$ as $m\uparrow \infty$. Then, the estimate \eqref{L2:control:ym} readily follows. In order to establish the a.s. convergence of the sequence $(\mathfrak{z}_m)_{m\geq0}$, one only has to check that the assumptions of the Robbins-Monro algorithm are satisfied. 
% Observe that the map $\mathfrak{z} \mapsto \mathfrak{H}_2(\tilde{\mathfrak{u}},\mathfrak{z}) = \mathbb{E}[ \mathrm{H}_2(W, \tilde{\mathfrak{u}}, \mathfrak{z}) ]$ satisfies the mean-reverting assumption $\langle \mathfrak{H}_2(\tilde{\mathfrak{u}},\mathfrak{z}), \mathfrak{z} - \mathfrak{z}^{\star} \rangle \geq \tilde{\alpha}_{\pi, \psi} \| \mathfrak{z} - \mathfrak{z}^{\star}\|^2$ as a direct consequence of \eqref{eq convex prop} and assumption 1.1. We now check the linear growth with respect to $\mathfrak{u}$ of the $L^{2}(\mathbb{P})$-moment of $\mathrm{H}(W, \tilde{\mathfrak{u}}, \mathfrak{u})$. From the boundedness assumption on $g$ and $f$,
% \begin{align}\label{quadratic:growth:bound:H}
%\| \mathrm{H}_2(W,\tilde{\mathfrak{u}},\mathfrak{u})\|^2
%&=
%\frac{|\Gamma^{\tilde{\mathfrak{u}}} - \bar{\Omega}\cdot \mathfrak{z}|^2 \|\bar{\Omega}\|^2}{1+\mathbb{E}[\|\bar{\Omega}\|^4]}
%\le 2\frac{(|\Gamma^{\tilde{\mathfrak{u}}}|^2 + \|\bar{\Omega}\|^2 \|\mathfrak{u}\|^2 )}{1+\mathbb{E}[\|\bar{\Omega}\|^4]} \|\bar{\Omega}\|^2 \leq C_0 \frac{(\|\bar{\Omega}\|^2 +  \|\bar{\Omega}\|^4 \|\mathfrak{u}\|^2)}{1+\mathbb{E}[\|\bar{\Omega}\|^4]}
%\end{align}
%\noindent with $C_0= 2 (|g|_\infty + T |f|_\infty)^2\vee 1 $, which in turn yields 
%\begin{equation}
%\mathbb{E}[\| H_2(W,\tilde{\mathfrak{u}},\mathfrak{u})\|^2] \leq C_1+ C_2 \|\mathfrak{u} -  \tilde{\mathfrak{u}}^{\star}\|^2 \label{second:moment:H}
%\end{equation}
%\noindent with $C_1 = C_0(1+2 \|\tilde{v}^{\star}\|^2)$, $C_2=2C_0$. The Robbins-Monro theorem thus implies the a.s. convergence of the sequence $(\mathfrak{z}_m)_{m\geq0}$ towards $\mathfrak{z}^{\star}(\tilde{\mathfrak{u}})$.\newline
%\medskip
% \emph{Step 2: $L^2(\mathbb{P})$ convergence rate.\\} In order to derive an $L^{2}(\mathbb{P})$ convergence rate for the sequence $\mathbb{E}[\|\mathfrak{u}_m- \tilde{\mathfrak{u}}^{\star}\|^2]$, $m\geq0$, we proceed as follows. We introduce the natural filtration of the algorithm namely $\cF= (\cF_m)_{0 \le m \le M}$, defined by $\cF_m = \sigma(\mathfrak{z}_0, W^{(k)}, 1 \le k \le m)$.
% From the dynamics \eqref{dynamics:sg:theta}, we directly get
% \begin{align*}
% \|   \mathfrak{z}_{m+1} - \mathfrak{z}^{\star} \|^2 & =   \|   \mathfrak{z}_{m} - \mathfrak{z}^{\star} \|^2 - 2 \gamma_{m+1} H_2(W^{(m+1)}, \tilde{v}, \mathfrak{z}_m)\cdot( \mathfrak{z}_{m} - \mathfrak{z}^{\star}) + \gamma^2_{m+1}\| H_2(W^{(m+1)},\tilde{\mathfrak{u}},\mathfrak{z}_m)\|^2 \\
% & =  \|   \mathfrak{z}_{m} - \mathfrak{z}^{\star} \|^2 - 2 \gamma_{m+1} \partial_{\mathfrak{z}}\mathfrak{H}_2(\tilde{\mathfrak{u}},\mathfrak{z}_{m})  \cdot( \mathfrak{z}_{m} - \mathfrak{z}^{\star}) + 2 \gamma_{m+1} \Delta M_{m+1}  + \gamma^2_{m+1} \| H_2(W^{(m+1)},\tilde{\mathfrak{u}},\mathfrak{z}_m)\|^2
% \end{align*}
% \noindent where we introduced the sequence of $\cF$-martingale increments 
% $$
% \Delta M_{m+1} := (\partial_\mathfrak{u} \mathfrak{H}_2(\tilde{\mathfrak{u}},\mathfrak{z}_{m}) - H_2(W^{(m+1)}, \tilde{v}, \mathfrak{z}_m)) \cdot( \mathfrak{z}_{m} - \mathfrak{z}^{\star}),\,  m\geq 0.
% $$
%  Now, from the previous equality, \eqref{eq convex prop}, \eqref{second:moment:H} and the fact that $\mathbb{E}[\Delta M_{m+1} | \cF_m] = 0$, we obtain
%\begin{align*}
% \mathbb{E}[ \|   \mathfrak{z}_{m+1} - \mathfrak{z}^{\star} \|^2] & \leq  \mathbb{E}[\|   \mathfrak{z}_{m} - \mathfrak{z}^{\star} \|^2] (1-2\tilde{\alpha}_{\pi, \psi}\gamma_{m+1}) + \gamma^2_{m+1} \mathbb{E}[ \| H_2(W^{(m+1)},\tilde{\mathfrak{u}},\mathfrak{z}_m)\|^2] \\
% & \leq  \mathbb{E}[\|   \mathfrak{z}_{m} - \mathfrak{z}^{\star} \|^2] (1-2\tilde{\alpha}_{\pi, \psi}\gamma_{m+1} + C_2 \gamma^2_{m+1})  + C_1 \gamma^2_{m+1}.
% \end{align*}
%Thus, introducing $\Pi_m = \prod_{k=1}^{m} (1-2\tilde{\alpha}_{\pi,\psi} \gamma_{k} + C_2 \gamma^2_{k})$ and $\Gamma_m = \sum_{k=1}^{m} \gamma_k$, we get
% \begin{align}
% 	  \esp{\|\mathfrak{z}_{m+1} - \mathfrak{z}^\star \|^2 } & \le \Pi_{m+1} \esp{ \| \mathfrak{z}_{0} - \mathfrak{z}^\star\|^2 } + C_1 \sum_{l=1}^{m+1} \dfrac{\Pi_{m+1}}{\Pi_{l}} \gamma^2_{l} \nonumber \\
%	  & \leq  K \exp(-2 \tilde{\alpha}_{\pi, \psi} \Gamma_{m+1}) \esp{ \| \mathfrak{u}_{0} - \tilde{\mathfrak{u}}^\star\|^2 } \nonumber \\
%	  & \quad + C_1 K  \sum_{l=1}^{m+1} \exp(-2 \tilde{\alpha}_{\pi, \psi} (\Gamma_{m+1}-\Gamma_{l})) \gamma^2_l \label{L2:control:distance:to:target}
% \end{align}
% \noindent with $K:= \exp(C_2 \sum_{l\geq1} \gamma^2_l)$. The proof is now complete.
% \end{proof}
% Concerning the choice of the step sequence $(\gamma_{m})_{m\geq1}$ and its impact on the $L^{2}(\mathbb{P})$ convergence rate, we obtain the following results:
%\begin{itemize} 
%\item If we choose $\gamma_{m}=\frac{\gamma_1}{m}$, with $\gamma_1>0$, then using $\Gamma_{m}=\gamma_1 \log(m) +\gamma_1 \gamma + r_{m}$, where $\gamma$ is the Euler constant and $r_{m}\rightarrow 0$, we get 
%$$
%\exp(-2 \tilde{\alpha}_{\pi, \psi} \Gamma_{m}) = c \, m^{-2\gamma_1 \tilde{\alpha}_{\pi, \psi}}
%$$
%\noindent and for the second term appearing in \eqref{L2:control:distance:to:target} one considers the two disjoint cases:
%\begin{itemize}
%\item If $\gamma_1 < \frac{1}{2 \tilde{\alpha}_{\pi, \psi}}$, the series $\sum_{l=1}^{m}\exp(2 \tilde{\alpha}_{\pi, \psi} \Gamma_l)\gamma^{2}_{l}$ converges so that we obtain 
%$$
%\sum_{l=1}^{m} \exp(-2 \tilde{\alpha}_{\pi, \psi} (\Gamma_m-\Gamma_l)) \gamma^{2}_{l} = c \, m^{-2\gamma_1 \tilde{\alpha}_{\pi, \psi}}.
%$$
%\item If $\gamma_1 > \frac{1}{2 \tilde{\alpha}_{\pi, \psi}}$, a comparison between the series and the integral yields
%$$
%\sum_{l=1}^{m} \exp(-2\tilde{\alpha}_{\pi, \psi} (\Gamma_m-\Gamma_l)) \gamma^{2}_{l} = \frac{\gamma^2_1}{(2 \gamma_1 \tilde{\alpha}_{\pi, \psi}-1)} \frac{1}{m}.
%$$
%\end{itemize}
%\noindent where $c$ is some positive constant. The last case $\gamma_1 > \frac{1}{2 \tilde{\alpha}_{\pi, \psi}}$ provides the best convergence rate. Note that the optimal value for $\gamma_1$ under the constraint is $\gamma_1 = 1/ \tilde{\alpha}_{\pi, \psi}$ giving the convergence rate $1/(\tilde{\alpha}^2_{\pi, \psi} m)$.\\
%\medskip
%\noindent The above discussion on the value of $\gamma_1$ is clearly reminiscent of the one that appears in the Central Limit Theorem for stochastic algorithms. Indeed, if $\gamma_1> \frac{1}{2\mathcal{R}e(\lambda_{min})}$ where $\lambda_{min}$ denotes the eigenvalue of $Dh(\mathfrak{z}^{*})$ with the smallest real part then a Central Limit Theorem holds (see e.g. the book of Duflo \cite{duflo1996algorithmes}).
%\item If we choose $\gamma_{m}=\frac{\gamma_1}{m^{\rho}}$ with $\gamma_1>0$, $\frac{1}{2} < \rho < 1$, then $\Gamma_{m} \sim \frac{\gamma_1}{1-\rho} m^{1-\rho}$ as $m \uparrow + \infty$ and then elementary computations based on comparison between series and integral show that there exists $c>0$ (that may change from line to line) such that for all $m\ge 1$
%\begin{eqnarray*}
%\sum_{l=1}^{m} \exp(-2 \tilde{\alpha}_{\pi, \psi} (\Gamma_{m}-\Gamma_{l})) \gamma^2_l &= &  \sum_{l=1}^{\lfloor m/2 \rfloor} \gamma^2_l e^{-2 \tilde{\alpha}_{\pi, \psi} (\Gamma_{m}-\Gamma_{l})} +   \sum_{l=\lfloor m/2 \rfloor+1}^{m} \gamma^2_l e^{-2 \tilde{\alpha}_{\pi, \psi} (\Gamma_{m}-\Gamma_{l})}  \\
%& \leq &  \gamma_1^2 \sum_{l=1}^{\lfloor m/2 \rfloor} \frac{1}{l^{2\rho}} e^{-\frac{2 \tilde{\alpha}_{\pi, \psi}\gamma_1}{1-\rho} [m^{1-\rho}-l^{1-\rho}]} \\
%& + &  \frac{\gamma_1}{m^{\rho}} e^{-2 \tilde{\alpha}_{\pi, \psi} \Gamma_{m}}  \sum_{l=\lfloor m/2 \rfloor+1}^{m} e^{2 \tilde{\alpha}_{\pi, \psi} \Gamma_{l}} \gamma_l \\
%& \leq & c \gamma^2_1 \sum_{l=1}^{\lfloor m/2 \rfloor} \frac{1}{l^{2\rho}} e^{-2 \tilde{\alpha}_{\pi,\psi}\gamma_1 \frac{2^{1-\rho}-1}{2^{1-\rho}(1-\rho)} m^{1-\rho}} \\
%& + &   \frac{c\gamma_1}{m^{\rho}} e^{-2 \tilde{\alpha}_{\pi, \psi} \Gamma_{m}} \frac{e^{2 \tilde{\alpha}_{\pi, \psi} \Gamma_m} - e^{2 \tilde{\alpha}_{\pi, \psi} \Gamma_{\lfloor m/2 \rfloor}}}{2\tilde{\alpha}_{\pi, \psi}} \\
%& \leq&  c \big[ \gamma^2_1 e^{-2 \tilde{\alpha}_{\pi,\psi}\gamma_1 \frac{2^{1-\rho}-1}{2^{1-\rho}(1-\rho)} m^{1-\rho}}  + \frac{\gamma_1}{\tilde{\alpha}_{\pi, \psi}m^{\rho}} \big]
%\end{eqnarray*}
%\noindent where $c$ is a positive constant independent of $m$, $\gamma_1$.
%\end{itemize} 
%
%Precise rate of convergence and complexity analysis are done in the next Section when the $\psi$-functions are given by Section \ref{subse approx space}. 
%
% \begin{Remark}
% 	In practice, we choose the value of $(\gamma_m)_{0\le m \le M}$ depends on discrete step time $n$. We simplified this in \Cref{dynamics:sg:y}-(\ref{dynamics:sg:theta}) since it doesn't improve the converge rate or reduce complexity of computation.
% \end{Remark}
%
% We now present some results related to the convergence rate of the recursive scheme \eqref{RM:algorithm}. 
% We present in a general setting a study of the error $\cE_{\mathrm{RM}}$. Precise rate of convergence and complexity analysis are done in the next Section when the basis functions are given by Section \ref{subse approx space}. \\
%
%\begin{Proposition}\label{pr error of Picard sharper}
%% \textcolor{red}{Just to have a rough idea of what is going on. Some estimates should be certainly improved...}
%Let the assumptions of lemma \ref{lem:stochastic:gradient} and proposition \ref{error of Picard}. Assume that there exists a positive constant $C$ such that for any positive integer $p$
%\begin{align}\label{eq ass cs control global}
% \kappa_{\pi,\psi} L^1_{\pi,\psi,M_p}  \le C \text{ and } \; \frac{\kappa_{\pi,\psi}}{\alpha_{\pi,\psi}} L^2_{\pi,\psi,M_p} \le C 
%\end{align}
%\noindent with
%\begin{align*}
% L^1_{\pi,\psi,M_p} & := C_0  K \sum_{l=1}^{M_p} e^{-2 \tilde{\alpha}_{\pi, \psi}(\Gamma_{M_p}-\Gamma_l)} \gamma^2_l + K e^{-2 \tilde{\alpha}_{\pi, \psi}\Gamma_{M_p}} \mathbb{E}[\|\mathfrak{z}_0\|^2], \\
% L^{2}_{\pi, \psi, M_p} & := 2 C_0 K \sum_{l=1}^{M_p} e^{-2 \tilde{\alpha}_{\pi, \psi}(\Gamma_{M_p}-\Gamma_l)} \gamma^2_l +  K e^{-2 \tilde{\alpha}_{\pi, \psi}\Gamma_{M_p}}.
%\end{align*}
%\noindent If $T(1+ 2L^2(1+ h)) < 1$ and
%$\delta:=\frac{8L^2 T (1+2C)}{1-T(1+ 2L^2(1+ h))} < 1$, then for any $\varepsilon>0$ such that $\delta_\varepsilon := \delta (1+\varepsilon)<1$  it holds
%\begin{align}
%\cE_P \le \delta_\varepsilon^P \cE_0 + C_\varepsilon \sum_{p=1}^{P}\delta_{\varepsilon}^{P-p} [\frac{1}{M_p} + L^1_{\pi,\psi,M_p}\kappa_{\pi,\psi}  + L^{2}_{\pi, \psi, M_p} \frac{\kappa_{\pi, \psi}}{\alpha_{\pi,\psi}}] + C_\varepsilon  (\cE_{\psi} +  \cE_{\pi}).
%\end{align}
%\end{Proposition}
%%\begin{bluetext}
%\proof
%\emph{Step 1: }
%From Lemma \ref{le control f(y,z)}, we have
%\begin{align}\label{eq interm lemma 4.3}
%\vvvert \Phi(\mathfrak{u}^p_{M})  -  \bar{\mathfrak{u}} \vvvert^2
%\le \delta_{\varepsilon} \vvvert \mathfrak{u}^p_{M} -  \bar{\mathfrak{u}} \vvvert^2  + C_\varepsilon(\cE_\pi + \cE_{\psi})
%\end{align}
%Note that $C_\varepsilon$ is a constant that may change from line to line. Hence, for any $\varepsilon>0$, we obtain
%\begin{align*}
% \esp{\vvvert \Phi(\mathfrak{u}^p_{M_p}) \vvvert^2}
% &\le
% (1+\varepsilon) \esp{\vvvert \Phi(\mathfrak{u}^p_{M_p}) - \bar{\mathfrak{u}}\vvvert^2} + (1+\frac{1}{\varepsilon}) \vvvert \bar{\mathfrak{u}}\vvvert^2
% \\
% &\le  \delta_\varepsilon \esp{\vvvert \mathfrak{u}^p_{M_p} -  \bar{\mathfrak{u}} \vvvert^2} + C_\varepsilon(\cE_\pi + \cE_{\psi}+\vvvert \bar{\mathfrak{u}}\vvvert^2)
% \\
%  &\le  \delta_{\varepsilon} \esp{\vvvert \mathfrak{u}^p_{M_p}\vvvert^2} 
%  + C_\varepsilon(\cE_\pi + \cE_{\psi}+\vvvert \bar{\mathfrak{u}}\vvvert^2)
%\end{align*}
%\noindent up to a modification of $\varepsilon$.
%Noting again that 
%$$
%\esp{\vvvert \mathfrak{u}^p_{M_p}\vvvert^2}
%\le 2\esp{\vvvert\Phi_M(\mathfrak{u}^{p-1}_{M_{p-1}}) - \Phi(\mathfrak{u}^{p-1}_{M_{p-1}})\vvvert^2}
%+ 2 \esp{\vvvert \Phi(\mathfrak{u}^{p-1}_{M_{p-1}})\vvvert^2}
% $$
% we obtain
% \begin{align}\label{eq interm bound unif}
% \esp{\vvvert \Phi(\mathfrak{u}^p_{M_p}) \vvvert^2}
% &\le
%  2\delta_{\varepsilon} \esp{\vvvert  \Phi(\mathfrak{u}^{p-1}_{M_{p-1}}) \vvvert^2}+ 2  \delta_{\varepsilon}  \esp{\vvvert\Phi_{M_p}(\mathfrak{u}^{p-1}_{M_{p-1}}) - \Phi(\mathfrak{u}^{p-1}_{M_{p-1}})\vvvert^2} +C_\varepsilon \bigg( \cE_\pi + \cE_{\psi}+\vvvert \bar{\mathfrak{u}}\vvvert^2\bigg)
% \end{align}
%Recalling Assumption \ref{as psi function}, using Lemma \ref{lem:stochastic:gradient} one gets
%% \textcolor{yellow}{
%%\begin{align}
%%\esp{\vvvert\Phi_M(\mathfrak{u}^{p-1}_{M}) - \Phi(\mathfrak{u}^{p-1}_{M}) \frac{1}{\alpha_{\pi,\psi}}^2 } 
%%\le
%% L_{\pi,\psi,M} (1 +  \frac{\kappa_{\pi,\psi}}{\alpha_{\pi,\psi}}\esp{\vvvert\Phi(\mathfrak{u}^{p-1}_{M}) \vvvert^2 })
%%\end{align} 
%%}
%\begin{align}\label{RM:L2:error}
%\esp{\vvvert\Phi_{M_p}(\mathfrak{u}^{p-1}_{M_{p-1}}) - \Phi(\mathfrak{u}^{p-1}_{M_{p-1}})\vvvert^2 } 
%\le
% \frac{(|g|_\infty + T |f|_\infty)^2}{M_p} +  L^1_{\pi,\psi,M_p}\kappa_{\pi,\psi}  + L^{2}_{\pi, \psi, M_p} \frac{\kappa_{\pi, \psi}}{\alpha_{\pi,\psi}}\esp{\vvvert\Phi(\mathfrak{u}^{p-1}_{M_{p-1}}) \vvvert^2 }.
%\end{align} 
%Inserting the previous estimate back into \eqref{eq interm bound unif}, we get
% \begin{align*}%\label{eq interm bound unif last}
% \esp{\vvvert \Phi(\mathfrak{u}^p_{M_p}) \vvvert^2}
% &\le
%  \delta_\varepsilon(1+ 2L^{2}_{\pi, \psi, M_p} \frac{\kappa_{\pi, \psi}}{\alpha_{\pi,\psi}}) \esp{\vvvert  \Phi(\mathfrak{u}^{p-1}_{M_{p-1}}) \vvvert^2} + C_\varepsilon(\cE_\pi + \cE_{\psi}+\vvvert \bar{\mathfrak{u}}\vvvert^2) \\
% & \quad +  2 \delta_\varepsilon ( \frac{(|g|_\infty + T |f|_\infty)^2}{M_p} + L^1_{\pi,\psi,M_p} \kappa_{\pi,\psi}).
% \end{align*}
% Combining \eqref{eq ass cs control global} with the previous inequality, we obtain
%% \textcolor{red}{Assuming $\frac{\kappa_{\pi,\psi}L_{\pi,\psi,M}}{\alpha_{\pi,\psi}} \le C$ and
%% $\kappa_{\pi,\psi} L_{\pi,\psi,M}  \le C$, We can delete the second condition }, we obtain
% \begin{align*}
% \esp{\vvvert \Phi(\mathfrak{u}^p_{M_p}) \vvvert^2} \le \delta_\varepsilon^{p} \esp{\vvvert \Phi(\mathfrak{u}^0_{M_0}) \vvvert^2}+ C_\varepsilon(\cE_\pi + \cE_{\psi}+\vvvert \bar{\mathfrak{u}}\vvvert^2 + \delta_\varepsilon)\;.
% \end{align*}
% Coming back to \eqref{RM:L2:error}, for any positive integer $p$, we thus get
%  \begin{align*}
% \esp{\vvvert\Phi_{M_p}({\mathfrak{u}}^{p-1}_{M_{p-1}}) - \Phi({\mathfrak{u}}^{p-1}_{M_{p-1}}) \vvvert^2 } &\le  \frac{(|g|_\infty + T |f|_\infty)^2}{M_p} + L^1_{\pi,\psi,M_p}\kappa_{\pi,\psi}  + L^{2}_{\pi, \psi, M_p} \frac{\kappa_{\pi, \psi}}{\alpha_{\pi,\psi}}C_{\varepsilon}
% \end{align*}
%\noindent up to a modification of the constant $C_\varepsilon$. We then come back to Proposition \ref{error of Picard} and deduce
%\begin{align}
%\cE_P \le \delta_\varepsilon^P \cE_0 + C_\varepsilon \sum_{p=1}^{P}\delta_{\varepsilon}^{P-p} [\frac{1}{M_p} + L^1_{\pi,\psi,M_p}\kappa_{\pi,\psi}  + L^{2}_{\pi, \psi, M_p} \frac{\kappa_{\pi, \psi}}{\alpha_{\pi,\psi}}] + C_\varepsilon  (\cE_{\psi} +  \cE_{\pi})
%\end{align}
%\noindent which concludes the proof.
%\eproof
%
%\end{yellowtext}

\subsubsection{Study of the approximation error of the stochastic gradient descent algorithm} \label{subse error of RM}

%\begin{bluetext} 
%$L^2(\P)$-convergence rate.\\

%\begin{Lemma} 
%\end{Lemma}
In this subsection, our aim is to study the approximation error of $\Phi$ by $\Phi_M$ where $\Phi_M$ has been introduced in Definition \ref{de sgd for phi}.

\begin{Lemma} \label{le tool robbins-monro} Suppose that Assumption \ref{ass X0}, Assumption \ref{assumption:coefficient} (i) and Assumption \ref{as psi function} hold. Let $\tilde{\mathfrak{u}}$ be a fixed $\R^{K^y} \times \R^{d \bar{K}^z}$-valued random vector and set $\check{\mathfrak{u}} =(\check{\mathfrak{y}},\check{\mathfrak{z}}) := \Phi(\tilde{\mathfrak{u}})$ and $\mathfrak{u}_M =({\mathfrak{y}}_M,\mathfrak{z}_M):= \Phi_M(\mathfrak{u}_0,\mathfrak{X}_0,\mathfrak{W},\tilde{\mathfrak{u}})$, $M$ being a positive integer and where $(\mathfrak{u}_0,\mathfrak{X}_0,\mathfrak{W})$ (recall Definition \ref{de sgd for phi}) is independent of $\tilde{\mathfrak{u}}$. We denote by $\mathbb{E}_{\tilde{\mathfrak{u}}}[\cdot]$, the conditional expectation with respect to the sigma-field $\sigma(\tilde{\mathfrak{u}})$ generated by $\tilde{\mathfrak{u}}$. Then, for any positive integer $M$, the random vector $(\mathfrak{y}_M, \mathfrak{z}_M)$ satisfies:
%\begin{bluetext}
 \begin{align} 
  \mathbb{E}_{\tilde{\mathfrak{u}}} \Big[|\mathfrak{y}_{M} - \check{\mathfrak{y}} |^2 \Big]
 %&
 \le 
L_{K,M} (1+|\check{\mathfrak{y}}|^2) %\label{bound:two:first:component:SGD:algorithm}
\quad\textnormal{ and }\quad
 \mathbb{E}_{\tilde{\mathfrak{u}}} \Big[|\mathfrak{z}^{n,\cdot}_{M, l} - \check{\mathfrak{z}}^{n,\cdot}_{l} |^2 \Big]
 %&
 \le 
L_{K,M}\left(\frac{1}{h}+|\check{\mathfrak{z}}^{n,\cdot}_{l}|^2\right) \label{eq final step 2 robbins monro}
\end{align}
\noindent for any $l \in \left\{1, \cdots, d\right\}$, with
\begin{align}
 L_{K,M} &:=  \varrho_0 \varrho_1 \Big(1+ \mathbb{E}\Big[  |\mathfrak{u}_{0}|^2\Big]  \Big) \sum_{m=1}^{M} \exp\left(- {4} \frac{{\alpha}_{K}}{\beta_{K}} (\Gamma_{M}-\Gamma_{m}) \right) \gamma_m^2 \label{de LpsiM}
 \\
\Gamma_{m} &:= \sum_{k=1}^m\gamma_k \;,\; m \ge 1\,,
\end{align}
\noindent where the constants $\varrho_0$, $\varrho_1$ are defined respectively in equation \eqref{de varrho 0} and \eqref{de varrho 1} below.
%\end{bluetext}
%{\color{green}
% \begin{align} 
%  \mathbb{E}_{\tilde{\mathfrak{u}}} \Big[|\mathfrak{y}_{M} - \check{\mathfrak{y}} |^2 \Big]
% &\le 
%L^y_{\pi,\psi,M} (1+|\check{\mathfrak{y}}|^2) %\label{bound:two:first:component:SGD:algorithm}
%\end{align}
%with
%\begin{align}\label{de LpipsiM y}
% L^y_{\pi,\psi,M} := 2 \varrho_0 \varrho_1  \Big(1+ \mathbb{E}\Big[  |\mathfrak{u}_{0}|^2\Big]  \Big) \sum_{m=1}^{M} \exp\left(- {4} \frac{{\alpha}_{K}}{\beta^y_{\pi,\psi}} (\Gamma_{M}-\Gamma_{m}) \right) \gamma_m^2
%\end{align}
%and for $0 \le n \le N-1$, any $\ell \in \set{1,\dots, d}$,
%\begin{align}
% \mathbb{E}_{\tilde{\mathfrak{u}}} \Big[|\mathfrak{z}^{n,\cdot}_{M, \ell} - \check{\mathfrak{z}}^{n,\cdot}_{\ell} |^2 \Big]
% &\le 
%L^z_{\pi,\psi,M} (1+|\check{\mathfrak{z}}^{n,\cdot}_{\ell}|^2) 
%\end{align}
%where
%\begin{align}\label{de LpipsiM}
% L^z_{\pi,\psi,M} := 2 \varrho_0 \varrho_1  \Big(1+ \mathbb{E}\Big[  |\mathfrak{u}_{0}|^2\Big]  \Big) \sum_{m=1}^{M} \exp\left(- {4} \frac{h \alpha_{ \psi}}{\beta^z_{\pi,\psi}} (\Gamma_{M}-\Gamma_{m}) \right) \gamma_m^2
%\end{align}
%}
%\textcolor{magenta}{
%with $\Gamma_{m} = \sum_{k=1}^m\gamma_k$, the constants $\varrho_0$, $\varrho_1$ being defined respectively in equation \eqref{de varrho 0} and \eqref{de varrho 1}  below.
%}
%\textcolor{red}{JF: Note that $L^y$ (say) depends on $\mathbb{E}_{\tilde{\mathfrak{u}}}\Big[ |\mathfrak{y}_0|^2\Big]$: but $\tilde{\mathfrak{u}}$ and $\mathfrak{u}_0$ have been chosen to be independent so I write directly the expectation. Also in a previous version of the paper $\mathfrak{u}_0$ was set to zero. It seems to me - from the proof - that $\mathfrak{u}_0$ does not need to be independent of $\tilde{\mathfrak{u}}$. when looking at the picard iteration scheme, it could be equal to $ \lambda \mathfrak{u}_M^{p-1} + (1-\lambda) \mathfrak{o}$ where $\mathfrak{o}$ is indeed independent of everything else. It would still be feasible to prove the convergence result, would that be better  from a numerical point of view?}

%\begin{enumerate}
%\item
%\textcolor{yellow}{
%At $n=0$:
%\begin{align}\label{bound:two:first:component:SGD:algorithm old}
%\bcancel{\mathbb{E}_{\tilde{\mathfrak{u}}}\Big[{|y_M -  \check{y}|^2 + h |z_M - \check{z}|^2}\Big] \le \frac{C}{M}}\;.
%\end{align}
%}
%\item 
%\textcolor{yellow}{
%For any $1 \le n \le N-1$ and any $\ell \in \set{1,\dots, d}$:
% \begin{align} \label{eq final step 2 robbins monro old }
% \mathbb{E}_{\tilde{\mathfrak{u}}} \Big[|\mathfrak{z}^{n,\cdot}_{M, \ell} - \check{\mathfrak{z}}^{n,\cdot}_{\ell} |^2 \Big]
% \le 
%L_{\pi,\psi,M} (1+|\check{\mathfrak{z}}^{n,\cdot}_{\ell}|^2)
%\end{align}
%where we set
%\begin{align}\label{de LpipsiM old}
% L_{\pi,\psi,M} := 2 \varrho_0 \varrho_1  \Big(1+\mathbb{E}_{\tilde{\mathfrak{u}}}\Big[  |\mathfrak{z}^{n,\cdot}_{\ell,0}|^2\Big]\Big) \sum_{m=1}^{M} \exp\left(- \textcolor{magenta}{4} \frac{{\alpha}_{\pi, \psi}}{\beta_{\pi,\psi}} (\Gamma_{M}-\Gamma_{m}) \right) \gamma_m^2
%\end{align}
%}

%\item 
\noindent Moreover, it holds
%\textcolor{blue}{ 
\begin{align}\label{eq useful robbins-monro}
  \mathbb{E}_{\tilde{\mathfrak{u}}}\Big[\vvvert \Phi_M(\tilde{\mathfrak{u}}) - \Phi(\tilde{\mathfrak{u}})\vvvert^2\Big]
  \le
 \kappa_{K} L_{K,M}\left(1+ d N\right) + \frac{\kappa_{K}}{\alpha_{K}} L_{K,M} \vvvert\Phi(\tilde{\mathfrak{u}})\vvvert^2\,.
\end{align}
%}
%\end{enumerate}
%\textcolor{red}{il faudra simplifier $\kappa$ et $\alpha$ en faisant apparaitre explicitement $h$... (a reprendre une fois que tous les calculs sont bouclés)}
\end{Lemma}
\proof

\noindent \emph{Step 1: } We prove the estimate for the difference $\mathfrak{z}^{n,\cdot}_{M, l} - \check{\mathfrak{z}}^{n,\cdot}_{l}$. The proof for $\mathfrak{y}_{M} - \check{\mathfrak{y}}$ follows from similar arguments and we omit some technical details. From \eqref{def:funct:H:2nd:part}, one gets
\begin{align*}
|H^{n,l}(\cX_0,W,\tilde{\mathfrak{u}},\mathfrak{z}^{n,\cdot}_l)|^2 & = \frac{4}{(\beta_K \sqrt{h})^2}|\mathfrak{G}^{\tilde{\mathfrak{u}}} - \omega^{n,\cdot}_l \cdot \mathfrak{z}^{n,\cdot}_l|^2|\omega^{n,\cdot}_l|^2\le 
\frac{8}{\beta^2_K}(|\mathfrak{G}^{\tilde{\mathfrak{u}}}|^2 + h|\tilde{\omega}^{n,\cdot}_l|^2 | \mathfrak{z}^{n,\cdot}_l|^2)|\tilde{\omega}^{n,\cdot}_l|^2\;.
\end{align*}
Under the boundedness Assumption \ref{assumption:coefficient} (i), recalling \eqref{eq de Gamma}, we obtain
\begin{align}
|\mathfrak{G}^{\tilde{\mathfrak{u}}}|^2 \le2\left( |g|^2_\infty+T^2 |f|^2_{\infty} \right)
\end{align}
\noindent so that setting 
\begin{align}
\label{de varrho 0}
\varrho_0 := 8\max \set{ (|g|_\infty+T |f|_{\infty})^2,2}
\end{align}
\noindent and from the lower bound \eqref{eq de beta psi}, we obtain
\begin{align}\label{eq 2nd moment H n l}
\mathbb{E}_{\tilde{\mathfrak{u}}}\Big[|H^{n,l}(\cX_0,W,\tilde{\mathfrak{u}},\mathfrak{z}^{n,\cdot}_l)|^2\Big]
\le
\varrho_0(1 + h|\mathfrak{z}^{n,\cdot}_l - \check{\mathfrak{z}}^{n,\cdot}_l|^2 +h|\check{\mathfrak{z}}^{n,\cdot}_l|^2)\;.
\end{align}

\noindent \emph{Step 2:} We now introduce the natural filtration of the algorithm namely $\cF= (\cF_m)_{0 \le m \le M}$, defined by $\cF_m = \sigma(\mathfrak{u}_0,\cX_0^{(k)}, W^{(k)}, 1 \le k \le m)$, $m\geq1$, and $\cF_0=\sigma(\mathfrak{u}_0)$. From the dynamics \eqref{RM iteration 2}, we directly get  
 \begin{align*}
 |\mathfrak{z}^{n,\cdot}_{l , m+1} - \check{\mathfrak{z}}^{n,\cdot}_{l} |^2  =    |\mathfrak{z}^{n,\cdot}_{l, m} - \check{\mathfrak{z}}^{n,\cdot}_{l} |^2 &- 2 \gamma^z_{m+1} H^{n,l}(\cX_0^{(m+1)},W^{(m+1)}, \tilde{\mathfrak{u}}, \mathfrak{z}^{n,\cdot}_{l, m} )\cdot( \mathfrak{z}^{n,\cdot}_{l, m} - \check{\mathfrak{z}}^{n,\cdot}_{l}) \\
 &+ (\gamma^z_{m+1})^2| H^{n,l}(\cX_0^{(m+1)},W^{(m+1)},\tilde{\mathfrak{u}},\mathfrak{z}^{n,\cdot}_{l , m})|^2 
 \end{align*}
 
 \noindent so that introducing the sequence of $\cF$-martingale increments,
 \begin{align*}
 \Delta M_{m+1} := \Big(\frac1{\beta_K \sqrt{h}}\nabla_{\!\mathfrak{z}^{n,\cdot}_{l}} \mathfrak{H}^{n,l}(\tilde{\mathfrak{u}},\mathfrak{u}_m) - H^{n,l}(\cX_0^{(m+1)},W^{(m+1)},\tilde{\mathfrak{u}},\mathfrak{z}^{n,\cdot}_{l , m})\Big) \cdot(\mathfrak{z}^{n,\cdot}_{l, m} - \check{\mathfrak{z}}^{n,\cdot}_{l}),\,  m\geq 0,
 \end{align*}
 we have
 \begin{align*}
 |\mathfrak{z}^{n,\cdot}_{l, m+1} - \check{\mathfrak{z}}^{n,\cdot}_{l} |^2  
 =   |\mathfrak{z}^{n,\cdot}_{l , m} - \check{\mathfrak{z}}^{n,\cdot}_{l} |^2 
 &- \frac2{\beta_K \sqrt{h}} \gamma^z_{m+1} \nabla_{\!\mathfrak{z}^{n,\cdot}_{l}} \mathfrak{H}^{n,l}(\tilde{\mathfrak{u}},\mathfrak{u}_m)  \cdot( \mathfrak{z}^{n,\cdot}_{l, m} - \check{\mathfrak{z}}^{n,\cdot}_{l} ) 
 \\
 &+ 2 \gamma^z_{m+1} \Delta M_{m+1}  +(\gamma^z_{m+1})^2 | H^{n, l }(\cX_0^{(m+1)},W^{(m+1)},\tilde{\mathfrak{u}},\mathfrak{z}^{n,\cdot}_{l, m})|^2\,.
 \end{align*}
% \noindent where we introduced the sequence of $\cF$-martingale increments 
% $$
% \Delta M_{m+1} := (\partial_\mathfrak{u} \mathfrak{H}_2(\tilde{\mathfrak{u}},\mathfrak{z}_{m}) - H_2(W^{(m+1)}, \tilde{v}, \mathfrak{z}_m)) \cdot( \mathfrak{z}_{m} - \mathfrak{z}^{\star}),\,  m\geq 0.
% $$
  Now, from the previous equality, \eqref{eq convex prop:2} and the fact that $\mathbb{E}_{\tilde{\mathfrak{u}}}[\Delta M_{m+1} | \cF_m] = 0$, recall \eqref{eq link h and H}, we obtain
\begin{align}
\mathbb{E}_{\tilde{\mathfrak{u}}}\Big[ |  \mathfrak{z}^{n,\cdot}_{l , m+1} - \check{\mathfrak{z}}^{n,\cdot}_{l} |^2 \Big] & \leq  
\mathbb{E}_{\tilde{\mathfrak{u}}}\Big[|   \mathfrak{z}^{n,\cdot}_{l , m} - \check{\mathfrak{z}}^{n,\cdot}_{l}|^2\Big] \Big(1- {4} \frac{h\alpha_{K}}{\beta_K \sqrt{h}}\gamma^z_{m+1}\Big) + (\gamma^z_{m+1})^2 \mathbb{E}_{\tilde{\mathfrak{u}}}\Big[| H^{n,l}(\cX_0^{(m+1)},W^{(m+1)},\tilde{\mathfrak{u}},\mathfrak{z}^{n,\cdot}_{l , m})|^2\Big] \nonumber \\
 & \leq  \mathbb{E}_{\tilde{\mathfrak{u}}}\Big[ |   \mathfrak{z}^{n,\cdot}_{l , m} - \check{\mathfrak{z}}^{n,\cdot}_{l} |^2\Big]
 \Big(1-{4}  \frac{h\alpha_{K}}{\beta_K \sqrt{h}}\gamma^z_{m+1} + \varrho_0 h(\gamma^z_{m+1})^2 \Big) 
 + \varrho_0 (\gamma^z_{m+1})^2(1+h|\check{\mathfrak{z}}^{n,\cdot}_{l}|^2) \label{temp:ineq:sa}
 \end{align}
 
 \noindent where, for the last inequality, we used \eqref{eq 2nd moment H n l} together with the fact that, since $(\cX_0^{(m+1)},W^{(m+1)})$ is independent of $\mathcal{F}_m$ and $\mathfrak{z}_m$ is $\mathcal{F}_m$-measurable, one has
 $$
 \mathbb{E}_{\tilde{\mathfrak{u}}}\Big[ | H^{n, l}(\cX_0^{(m+1)},W^{(m+1)},\tilde{\mathfrak{u}},\mathfrak{z}^{n,\cdot}_{l , m})|^2 | \mathcal{F}_{m}\Big] = \mathbb{E}_{\tilde{\mathfrak{u}}}\Big[| H^{n,l}(\cX_0,W,\tilde{\mathfrak{u}},\mathfrak{z}^{n,\cdot}_{l})|^2 \Big]_{| \mathfrak{z}^{n, \cdot}_{l}= \mathfrak{z}^{n,\cdot}_{l,m}}.
 $$
 Observe now that by the very definition \eqref{eq de gamama} of the sequence $(\gamma^z_m)_{m\geq1}$ and using the fact that $\alpha_K/\beta_K\leq 1$ and $\varrho_0\geq 16$, one gets $1-{4}  \frac{h\alpha_{K}}{\beta_K \sqrt{h}}\gamma^z_{m+1} + \varrho_0 h(\gamma^z_{m+1})^2  = 1-(4 \frac{\alpha_{K}}{\beta_K}\gamma_{m+1} - \varrho_0 \gamma^2_{m+1})\geq 1- (\sqrt{\varrho_0} \gamma_{m+1} - \varrho_0 \gamma^2_{m+1})\geq 1- 1/4 = 3/4$. As a consequence, $\Pi_m := \prod_{k=1}^{m} (1-{4}  \frac{h\alpha_{K}}{\beta_K \sqrt{h}}\gamma^z_{k} + \varrho_0 h(\gamma^z_{k})^2 ) = \prod_{k=1}^{m} (1- {4} \frac{\alpha_{K}}{\beta_{K}}\gamma_{k} + \varrho_0 \gamma_{k}^2)$ is a product of positive terms. From \eqref{temp:ineq:sa}, we thus deduce
 %and $\Gamma^{n,l}_m = \sum_{k=1}^{m} \gamma^{n,l}_k$ (with the convention $\Gamma^{n,l}_0=0$), 
 \begin{align}
 	  \mathbb{E}_{\tilde{\mathfrak{u}}}\Big[ |\mathfrak{z}^{n,\cdot}_{l,m+1}&  - \check{\mathfrak{z}}^{n,\cdot}_{l} |^2 \Big]\nonumber
	  \\
	  & \le \Pi_{m+1} \mathbb{E}_{\tilde{\mathfrak{u}}}\Big[ | \mathfrak{z}^{n,\cdot}_{l,0} - \check{\mathfrak{z}}^{n,\cdot}_{l} |^2 \Big]
	  +  \varrho_0 (\frac1{h}+|\check{\mathfrak{z}}^{n,\cdot}_{l}|^2) \sum_{q=1}^{m+1} \dfrac{\Pi_{m+1}}{\Pi_{q}} \gamma_{q}^2 \nonumber \\
	  & \leq  2\varrho_1 \exp\Big(- {4} \frac{\alpha_{K}}{\beta_{K}} \Gamma_{m+1}\Big) \Big(\mathbb{E}_{\tilde{\mathfrak{u}}}\Big[  |\mathfrak{z}^{n,\cdot}_{l,0}|^2\Big] + |\check{\mathfrak{z}}^{n,\cdot}_{l} |^2  \Big) \nonumber \\
	  & \quad + \varrho_1\varrho_0 (\frac1{h}+|\check{\mathfrak{z}}^{n,\cdot}_{l}|^2) \sum_{q=1}^{m+1} \exp\left(- {4} \frac{\alpha_{K}}{\beta_{K}} (\Gamma_{m+1}-\Gamma_{q}) \right) \gamma_q^2\nonumber \\
	  & \leq    \varrho_0 \varrho_1  \Big(1+\mathbb{E}_{\tilde{\mathfrak{u}}}\Big[  |\mathfrak{z}^{n,\cdot}_{l,0}|^2\Big]\Big)  \left(\frac1h+|\check{\mathfrak{z}}^{n,\cdot}_{l}|^2\right)
 \sum_{q=1}^{m+1} \exp\left(- {4} \frac{\alpha_{K}}{\beta_{K}} (\Gamma_{m+1}-\Gamma_{q}) \right) \gamma_q^2 \label{L2:control:distance:to:target}
 \end{align}
 \noindent where we used the standard inequality $1+ x \leq e^x$, the fact that $\rho_0\geq 2$ and introduced the quantity 
 \begin{align}\label{de varrho 1}
\varrho_1:= \exp(\varrho_0 \sum_{m\geq1} \gamma^2_m).
 \end{align}
 This concludes the proof for \eqref{eq final step 2 robbins monro}.
% Observing that $\mathfrak{z}_0 = 0$, we get
% \begin{align} \label{eq final step 2 robbins monro}
% \esp{|\mathfrak{z}^{n,\cdot}_{l,m+1} - \check{\mathfrak{z}}^{n,\cdot}_{l} |^2 } 
% \le 
% 2 \varrho_0 \varrho_1 (1+|\check{\mathfrak{z}}^{n,\cdot}_{l}|^2)
% \sum_{q=0}^{m+1} \exp\left(-2 \frac{{\alpha}_{\pi, \psi}}{\beta_{\pi,\psi}} (\Gamma_{m+1}-\Gamma_{q}) \right) \gamma_q^2 \;.
% \end{align}
 %with  \textcolor{red}{the convention $\gamma_0 \neq 0$ (=1)...}
 
\noindent \emph{ Step 3:} Recalling Definition \ref{de double - triple norm} and using \eqref{eq link triple double} as well as Assumption \ref{as psi function}, we directly deduce 
 \begin{align*}
 \mathbb{E}_{\tilde{\mathfrak{u}}}\Big[\vvvert \Phi_M({\tilde{\mathfrak{u}}}) - \Phi({\tilde{\mathfrak{u}}})\vvvert^2 \Big]
 \le \mathbb{E}_{\tilde{\mathfrak{u}}}\Big[\kappa_{K}|\mathfrak{y}_M-\check{\mathfrak{y}}|^2 + h\kappa_{K} \sum_{n=1}^{N-1}\sum_{l=1}^d |\mathfrak{z}^{n,\cdot}_{l,M} -\check{\mathfrak{z}}^{n,\cdot}_{l} |^2 \Big]
 \end{align*}
 
 \noindent so that, using  \eqref{eq final step 2 robbins monro}
 \begin{align*}
 \mathbb{E}_{\tilde{\mathfrak{u}}}\Big[ \vvvert \Phi_M(\tilde{\mathfrak{u}}) - \Phi(\tilde{\mathfrak{u}})\vvvert^2\Big]
 &\le  
 \kappa_{K} L_{K,M}(1+ |\check{\mathfrak{y}} |^2)
+ h\kappa_{K} L_{K,M}\sum_{n=1}^{N-1}\sum_{l=1}^d (\frac1h+ |\check{\mathfrak{z}}^{n,\cdot}_{l} |^2) \,,
\\
& \le 
 \kappa_{K} L_{K,M} +
 \frac{\kappa_{K}}{\alpha_{K}} L_{K,M}\|\check{\mathfrak{y}}\|_y^2
+ h\kappa_{K} L_{K,M} Nd \frac1h+ \frac{\kappa_{K}}{\alpha_{K}} L_{K,M} \|\check{\mathfrak{z}}\|_z^2 \,,
\\
&\le \kappa_{K} L_{K,M}\left(1+ d N\right) + \frac{\kappa_{K}}{\alpha_{K}} L_{K,M} \vvvert\check{\mathfrak{u}}\vvvert^2\,,
 \end{align*}
 which concludes the proof.
\eproof

\vspace{2mm}
The following result provides an upper-bound for the quantity $L_{K,M}$  for a given specification of the
learning step that is useful to study the complexity of the global algorithm.

\begin{Lemma} \label{le gamma spec LpipsiM}
Let Assumption \ref{as psi function} hold. For $\gamma>0$, $\rho \in (\frac12,1)$, 
set $\gamma_m := \gamma m^{-\rho}$, $m \ge 1$. If the number of steps $M$ in the stochastic gradient descent algorithm satisfies 
\textcolor{black}{ 
\begin{align}\label{eq constraint alpha-beta-M 1}
\gamma\frac{{\alpha}_{ K}}{\beta_{K}}M^{1-\rho} \ge \frac{\sqrt{2}}2\;,  
\end{align}
}
\noindent then, there exists some positive constant $C:=C(\rho, \gamma)$ such that
%\begin{align}\label{upper:bound:rate:convergence:SG:algorithm}
%L_{K,M} \le C_{\rho}\gamma e^{\frac{ \textcolor{magenta}{4} \gamma }{1-\rho}\frac{{\alpha}_{\pi, \psi}}{\beta_{\pi,\psi}}}\left(
%\gamma \exp\left( -\textcolor{magenta}{ 2 } \gamma \frac{{\alpha}_{\pi, \psi}}{\beta_{\pi,\psi}} M^{1-\rho}   \right)
%+
%\textcolor{magenta}{\frac{2}{M^{2\rho - 1}}}
%% \frac{ \beta_{\pi,\psi}}{{\alpha}_{\pi,\psi}M^\rho}
%\right)
%\end{align} 
%\noindent with $C_\rho := 2\varrho_0\varrho_1 \Big(1+\mathbb{E}_{\tilde{\mathfrak{u}}}\Big[  |\mathfrak{z}^{n,\cdot}_{l,0}|^2\Big]\Big)$.

\begin{align}\label{eq bound LpsiM}
L_{K,M} \le C \left(e^{- 2\sqrt{2}\ln(2)\gamma\frac{\alpha_K }{\beta_{K}}M^{1-\rho}} 
+  \frac{ \beta_{K}}{\alpha_K M^\rho }
\right).
\end{align}

\end{Lemma}


\vspace{2mm}
\begin{Remark}\label{re condition beta}
\begin{enumerate}
\item In practice, $L_{K,M}$ should go to zero with respect to the optimal parameters. Thus, we must have that $\frac{ \beta_{K}}{\alpha_K M^\rho}$ goes to zero  and
$\frac{\alpha_K}{\beta_{K}} M^{1-\rho} $ goes to infinity at the same time as $M$ goes to infinity. This will be carefully discussed in \Cref{subse Com analysis}. With these constraints, we will naturally have that \eqref{eq constraint alpha-beta-M 1} is satisfied.
\item A careful analysis of the proof below shows that $\lim_{\rho \rightarrow  0.5^+} C(\rho, \gamma) = +\infty$, which comes from the dependence of $C(\rho, \gamma)$ with respect to $\sum_{1}^{+\infty} \frac1{m^{2 \rho}}$. However, one must bear in mind that $\rho$ is a fixed (but optimised) parameter.
\end{enumerate}
\end{Remark}

\vspace{2mm}
\noindent \textbf{Proof of Lemma \ref{le gamma spec LpipsiM}.}
We have, since $\Gamma_m = \gamma\sum_{q=1}^m \frac1{q^\rho} $, for $m\ge 1$,
\begin{align}
\frac{\gamma}{1-\rho}\left( m^{1-\rho} - 1\right)  \le \Gamma_m
\le   \frac{\gamma}{1-\rho}\left( m^{1-\rho} - 1\right) +  \gamma 
\end{align}

\noindent by standard computations based on comparison between series and integral, leading to
\begin{align}
\Gamma_m - \Gamma_M \le \frac{\gamma}{1-\rho}\left( m^{1-\rho} - M^{1-\rho}\right) 
+  \gamma .
\end{align}
Recalling \eqref{de LpsiM}, we employ the following decomposition
\begin{align}
 L_{K,M} &=  \varrho_0 \varrho_1  \Big(1+ \mathbb{E}\Big[  |\mathfrak{u}_{0}|^2\Big]  \Big) \sum_{m=1}^{M} \exp\left(- {4} \frac{{\alpha}_{K}}{\beta_{K}} (\Gamma_{M}-\Gamma_{m}) \right) \gamma_m^2 
 \\
 &\le 
  \varrho_0 \varrho_1   \Big(1+ \mathbb{E}\Big[  |\mathfrak{u}_{0}|^2\Big]  \Big)  \exp\left({4}\gamma \frac{{\alpha}_{K}}{\beta_{K}} \right) 
  \big(A_M + B_M +\gamma_M^2 \big)
\label{eq first to conclude}
\end{align}

%\begin{align}\label{eq lpipsisplit}
% L_{\pi,\psi,M} = &
%2\varrho_0\varrho_1 \Big(1+\mathbb{E}_{\tilde{\mathfrak{u}}}\Big[  |\mathfrak{z}^{n,\cdot}_{l,0}|^2\Big]\Big)  e^{\frac{ \textcolor{magenta}{4} \gamma}{1-\rho}\frac{{\alpha}_{\pi, \psi}}{\beta_{\pi,\psi}}} \big(A_M + B_M \big)
%% \\
%% &+
%% =: A_M \noindent
%% \\
%% &+ 
%%  \sum_{m=\floor{M/2}+1}^{M} \exp\left( 2\frac{{\alpha}_{\pi, \psi}}{\beta_{\pi,\psi}} \frac{\gamma}{1-\rho}\set{ (m+1)^{1-\rho} - (M+1)^{1-\rho} } \right)\frac{\gamma^2}{m^{2 \rho}} \Bigg) \,=: B_M \noindent
%\end{align}
with
\begin{align*}
A_M &:=  \sum_{m=1}^{\floor{M/2}} \exp\left( {4} \frac{{\alpha}_{K}}{\beta_{K}} \frac{\gamma}{1-\rho}\set{ m^{1-\rho} - M^{1-\rho} } \right)\frac{\gamma^2}{m^{2 \rho}},
\\
B_M &:=  \sum_{m=\floor{M/2}+1}^{M-1} \exp\left( {4} \frac{{\alpha}_{K}}{\beta_{K}} \frac{\gamma}{1-\rho}\set{ m^{1-\rho} - M^{1-\rho} } \right)\frac{\gamma^2}{m^{2 \rho}}.
\end{align*}
For the first term $A_M$, we observe that, for $m \le \floor{M/2} \le M/2$ and $\frac12<\rho<1$,
\begin{align}
 m^{1-\rho} - M^{1-\rho} \le - \frac{\sqrt{2}}{2} \ln(2) (1-\rho)M^{1-\rho}\;.
\end{align}
We then compute
\begin{align}
A_M &\le  \exp\left(- 2\sqrt{2}\ln(2) \gamma \frac{{\alpha}_{K}}{\beta_{K}} M^{1-\rho}  \right) \sum_{m=1}^{\floor{M/2}} \frac{\gamma^2}{m^{2 \rho}} \nonumber
\\
&\le  C_{\rho, \gamma}  \exp\left(- 2\sqrt{2}\ln(2) \gamma \frac{{\alpha}_{K}}{\beta_{K}} M^{1-\rho}  \right). \label{eq upper bound A}
\end{align}
%recalling that $\frac12 < \rho < 1$.
%Since $(\frac{\frac{M}2+1}{1+M})^{1-\rho} \le 2^{\rho-1}(1+\frac1{1+M})$, we get
%\begin{align}
%A_M &\le C_\rho\gamma^2 \exp\left( 2\frac{{\alpha}_{\pi, \psi}}{\beta_{\pi,\psi}} \frac{\gamma}{1-\rho}
%\set{ \frac{2^{1-\rho} -1}{2^{1-\rho}}}
%(M+1)^{1-\rho} 
%+ 2\frac{\gamma}{1-\rho}\frac{{\alpha}_{\pi, \psi}}{\beta_{\pi,\psi}(1+M)^\rho}
%\right) \noindent
%\\
%&\le C_{\rho,\iota} \gamma^2\exp\left( -\sqrt{2}\gamma\frac{{\alpha}_{\pi, \psi}}{\beta_{\pi,\psi}} (M+1)^{1-\rho}  \right)
%\label{eq upper bound A}
%\end{align}
%where we used \eqref{eq constraint alpha-beta-M 1} and the fact that $\rho \in (\frac12,1)$.
We now study the term $B_M$ which reads
%\textcolor{red}{
%\[ why \; not \; B_M \le  \sum_{m=\floor{M/2}+1}^{M-1}  \frac{\gamma^2}{m^{2 \rho}} \le  \gamma^2 \int_{M/2}^{M}  \frac{1}{m^{2 \rho}}  \ud x \le \frac{\gamma^2}{M^{2 \rho - 1}}  \]
%}
\begin{align*}
B_M = \gamma^2 \exp\left( - {4} \frac{{\alpha}_{K}}{\beta_{K}} \frac{\gamma}{1-\rho} M^{1-\rho}  \right)  \sum_{m=\floor{M/2}+1}^{M-1}\lambda(m)
\end{align*}
where, the map $\lambda$ is defined for $x \ge 1$ by
\begin{align}
\lambda(x) := \exp\left(  {4} \frac{{\alpha}_{K}}{\beta_{K}} \frac{\gamma}{1-\rho} x^{1-\rho}  \right)\frac{1}{x^{2 \rho}}.
\end{align}
We observe that $\lambda$ is increasing on $[\floor{M/2}+1,+\infty)$ when  \eqref{eq constraint alpha-beta-M 1} holds. This leads to
\begin{align*}
\sum_{m=\floor{M/2}+1}^{M-1}\lambda(m) &\le \int_{M/2}^{M} \lambda(x) \ud x\\
& \leq \frac{2^\rho}{M^{\rho}} \int_{M/2}^{M} \exp\left(  {4} \frac{{\alpha}_{K}}{\beta_{K}} \frac{\gamma}{1-\rho} x^{1-\rho}  \right)\frac{1}{x^{\rho}} \ud x
\\
&\le  \frac{ 2^{\rho-  {2} } \beta_{K}}{\gamma{M^\rho \alpha}_{K}}
\exp\left(  {4} \frac{{\alpha}_{K}}{\beta_{K}} \frac{\gamma}{1-\rho} M^{1-\rho}  \right)  
\end{align*}
which in turn yields
$ B_M \le  \frac{ \gamma\beta_{K}}{M^\rho \alpha_{K}}.$

Inserting the previous inequality and estimate \eqref{eq upper bound A} into \eqref{eq first to conclude} concludes the proof,  since $\mathbb{E}\Big[  |\mathfrak{u}_{0}|^2\Big] < \infty$, recall Definition \ref{de picard scheme full}, step 1. and  $\frac{\alpha_K}{\beta_K} \le 1$ recall Assumption \ref{as psi function} and \eqref{eq de beta psi}.
%
%\textcolor{magenta}{
%If we choose $\gamma_{m}=\frac{\gamma_1}{m^{\rho}}$ with $\gamma_1>0$, $\frac{1}{2} < \rho < 1$, then $\Gamma_{m} \sim \frac{\gamma_1}{1-\rho} m^{1-\rho}$ as $m \uparrow + \infty$ and then elementary computations based on comparison between series and integral show that there exists $c>0$ (that may change from line to line) such that for all $m\ge 1$
%\begin{eqnarray*}
%\sum_{l=1}^{m} \exp(-2 \tilde{\alpha}_{\pi, \psi} (\Gamma_{m}-\Gamma_{l})) \gamma^2_l &= &  \sum_{l=1}^{\lfloor m/2 \rfloor} \gamma^2_l e^{-2 \tilde{\alpha}_{\pi, \psi} (\Gamma_{m}-\Gamma_{l})} +   \sum_{l=\lfloor m/2 \rfloor+1}^{m} \gamma^2_l e^{-2 \tilde{\alpha}_{\pi, \psi} (\Gamma_{m}-\Gamma_{l})}  \\
%& \leq &  \gamma_1^2 \sum_{l=1}^{\lfloor m/2 \rfloor} \frac{1}{l^{2\rho}} e^{-\frac{2 \tilde{\alpha}_{\pi, \psi}\gamma_1}{1-\rho} [m^{1-\rho}-l^{1-\rho}]} \\
%& + &  \frac{\gamma_1}{m^{\rho}} e^{-2 \tilde{\alpha}_{\pi, \psi} \Gamma_{m}}  \sum_{l=\lfloor m/2 \rfloor+1}^{m} e^{2 \tilde{\alpha}_{\pi, \psi} \Gamma_{l}} \gamma_l \\
%& \leq & c \gamma^2_1 \sum_{l=1}^{\lfloor m/2 \rfloor} \frac{1}{l^{2\rho}} e^{-2 \tilde{\alpha}_{\pi,\psi}\gamma_1 \frac{2^{1-\rho}-1}{2^{1-\rho}(1-\rho)} m^{1-\rho}} \\
%& + &   \frac{c\gamma_1}{m^{\rho}} e^{-2 \tilde{\alpha}_{\pi, \psi} \Gamma_{m}} \frac{e^{2 \tilde{\alpha}_{\pi, \psi} \Gamma_m} - e^{2 \tilde{\alpha}_{\pi, \psi} \Gamma_{\lfloor m/2 \rfloor}}}{2\tilde{\alpha}_{\pi, \psi}} \\
%& \leq&  c \big[ \gamma^2_1 e^{-2 \tilde{\alpha}_{\pi,\psi}\gamma_1 \frac{2^{1-\rho}-1}{2^{1-\rho}(1-\rho)} m^{1-\rho}}  + \frac{\gamma_1}{\tilde{\alpha}_{\pi, \psi}m^{\rho}} \big]
%\end{eqnarray*}
%\noindent where $c$ is a positive constant independent of $m$, $\gamma_1$.
%}
\eproof



\begin{Remark}
Let us importantly point out that if one choses $\gamma_{m}= \gamma /m$, with $\gamma>0$, then from standard comparison between series and integral $\Gamma_{m} - \Gamma_M \leq \gamma (\ln(m/M)+1)$ so that repeating the computations of the proof of Lemma \ref{le gamma spec LpipsiM}, one has to consider the two disjoint cases $\gamma < \frac{\beta_K}{4\alpha_K}$ and $\gamma > \frac{\beta_K}{4\alpha_K}$ in order to provide an upper bound for the quantity of interest $L_{K, M}$. Only the latter allows to obtain the best convergence rate of order $1/M$. However, in practice, the user does not know the exact value of $\frac{\beta_{K}}{4\alpha_{K}}$ so that one will often consider higher values of $\gamma$ than requested which will have the undesirable effect to deteriorate the upper-bound as suggested by the value of $\varrho_1$ in \eqref{de varrho 1}. Moreover, as shown in Section \ref{se con and com analysis}, the value $\frac{\beta_{K}}{4\alpha_{K}}$ actually goes to infinity when the prescribed approximation error $\varepsilon$ goes to zero so that the latter condition becomes more and more stringent. 

%\noindent and for the second term appearing in \eqref{L2:control:distance:to:target} one considers the two disjoint cases:
%\begin{itemize}
%\item If $\gamma_1 < \frac{1}{2 \tilde{\alpha}_{\pi, \psi}}$, the series $\sum_{l=1}^{m}\exp(2 \tilde{\alpha}_{\pi, \psi} \Gamma_l)\gamma^{2}_{l}$ converges so that we obtain 
%$$
%\sum_{l=1}^{m} \exp(-2 \tilde{\alpha}_{\pi, \psi} (\Gamma_m-\Gamma_l)) \gamma^{2}_{l} = c \, m^{-2\gamma_1 \tilde{\alpha}_{\pi, \psi}}.
%$$
%\item If $\gamma_1 > \frac{1}{2 \tilde{\alpha}_{\pi, \psi}}$, a comparison between the series and the integral yields
%$$
%\sum_{l=1}^{m} \exp(-2\tilde{\alpha}_{\pi, \psi} (\Gamma_m-\Gamma_l)) \gamma^{2}_{l} = \frac{\gamma^2_1}{(2 \gamma_1 \tilde{\alpha}_{\pi, \psi}-1)} \frac{1}{m}.
%$$
%\end{itemize}
%\noindent where $c$ is some positive constant. The last case $\gamma_1 > \frac{1}{2 \tilde{\alpha}_{\pi, \psi}}$ provides the best convergence rate. Note that the optimal value for $\gamma_1$ under the constraint is $\gamma_1 = 1/ \tilde{\alpha}_{\pi, \psi}$ giving the convergence rate $1/(\tilde{\alpha}^2_{\pi, \psi} m)$.\\
%\medskip
%\noindent The above discussion on the value of $\gamma_1$ is clearly reminiscent of the one that appears in the Central Limit Theorem for stochastic algorithms. Indeed, if $\gamma_1> \frac{1}{2\mathcal{R}e(\lambda_{min})}$ where $\lambda_{min}$ denotes the eigenvalue of $Dh(\mathfrak{z}^{*})$ with the smallest real part then a Central Limit Theorem holds (see e.g. the book of Duflo \cite{duflo1996algorithmes}).
\end{Remark}


\noindent We now give an upper bound for the error $\cE_P$ defined by \eqref{eq de error picard}, with respect to all the algorithm's parameters. These parameters will be chosen in the next section taking into account the precise specification of the functional approximation space. 
\begin{Proposition} \label{pr main abstract error}
Suppose that Assumption \ref{ass X0}, Assumption \ref{assumption:coefficient} (i), (ii) and Assumption \ref{as psi function} hold. Assume that there exists a positive constant $\eta$ {(independent of $N$, $M$ and the basis functions $(\psi)$)} such that
\begin{align}\label{eq ass cs control global}
\frac{\kappa_{K}}{h \wedge \alpha_K } L_{K,M}  \le \eta \;.
 \end{align}
\noindent If $T(1+ 2L^2(1+ h)) < 1$ and
$\delta_{h,\eta}:=\frac{ 16L^2 T (1+\eta)}{1-T(1+ 2L^2(1+ h))} < 1$, then for any $\varepsilon>0$ there exists a positive constant $C_\varepsilon$ such that
$$
\cE_{\mathrm{RM}} \leq C_\varepsilon \frac{\kappa_{K}}{h \wedge \alpha_K } L_{K,M} $$
%such 
%that $\delta_{h,\eta,\varepsilon} := \delta_{h,\eta} (1+\varepsilon)<1$  it holds
so that, with the notations of Proposition \ref{error of Picard}, it holds
\begin{align}\label{global:control:error}
\cE_P \le \delta_{h, \varepsilon}^P \cE_0 + C_\varepsilon \left(
\frac{\kappa_{K}}{h \wedge \alpha_K } L_{K,M}  + \cE_{\psi} +  \cE_{\pi} \right).
\end{align}
%\textcolor{blue}{simplifier ces expressions en virant $\kappa$, $\alpha$}
\end{Proposition}

\vspace{2mm}
\begin{Remark} In practice, $\eta$ will be fixed to be a small constant as the term in the left hand side of \eqref{eq ass cs control global} should be asymptotically zero.
\end{Remark}

\vspace{2mm}

\noindent \textbf{Proof of Proposition \ref{pr main abstract error}.}

\noindent \emph{Step 1:} From Proposition \ref{error of Picard}, we see that to obtain \eqref{global:control:error}, it remains to control
\begin{align*}
\cE_{\mathrm{RM}} =\max_{1 \le p \le P} \esp{\vvvert \Phi_M(\mathfrak{u}^{p-1}_M) - \Phi(\mathfrak{u}^{p-1}_M)\vvvert^2}.
\end{align*}
Using Lemma \ref{le tool robbins-monro}, we have
\begin{align}\label{eq  robbins-monro here}
  \esp{\vvvert \Phi_M(\mathfrak{u}^{p-1}_M) - \Phi(\mathfrak{u}^{p-1}_M)\vvvert^2} 
  \le
\kappa_{K} L_{K,M}(1
+  d N )
+ \frac{\kappa_{K}}{\alpha_{K}} L_{K,M} \esp{\vvvert \Phi(\mathfrak{u}^{p-1}_M) \vvvert^2}.
\end{align}
To conclude the proof, we will in the next step, provide an  upper bound for the term $\esp{\vvvert \Phi(\mathfrak{u}^{p-1}_M) \vvvert^2}$, uniformly with respect to $p$.
\\

\noindent \emph{Step 2:} We denote by $C_\varepsilon$ a constant that may change from line to line along with $\varepsilon$.
%From Lemma \ref{le control f(y,z)}, we have
%\begin{align}\label{eq interm lemma 4.3}
%\vvvert \Phi(\mathfrak{u}^p_{M})  -  \bar{\mathfrak{u}} \vvvert^2
%\le \delta_{h}(1+\varepsilon) \vvvert \mathfrak{u}^p_{M} -  \bar{\mathfrak{u}} \vvvert^2  + C_\varepsilon(\cE_\pi + \cE_{\psi})
%\end{align}
From Young's inequality and Lemma \ref{le control f(y,z)}, we obtain
\begin{align*}
 \esp{\vvvert \Phi(\mathfrak{u}^p_{M}) \vvvert^2}
 &\le
 (1+\varepsilon) \esp{\vvvert \Phi(\mathfrak{u}^p_{M}) - \bar{\mathfrak{u}}\vvvert^2} + (1+\frac{1}{\varepsilon}) \vvvert \bar{\mathfrak{u}}\vvvert^2
 \\
 &\le \delta_{h}(1+\varepsilon)  \esp{\vvvert \mathfrak{u}^p_{M} -  \bar{\mathfrak{u}} \vvvert^2} + C_\varepsilon(\cE_\pi + \cE_{\psi}+\vvvert \bar{\mathfrak{u}}\vvvert^2)
 \\
  &\le \delta_{h}(1+\varepsilon) \esp{\vvvert \mathfrak{u}^p_{M}\vvvert^2} 
  + C_\varepsilon(\cE_\pi + \cE_{\psi}+\vvvert \bar{\mathfrak{u}}\vvvert^2)
\end{align*}
up to a modification of $\varepsilon$. From the previous inequality, we readily obtain $ \esp{\vvvert \Phi(\mathfrak{u}^0_{M}) \vvvert^2} \leq C_\varepsilon$. Now, if $p$ is a positive integer, noting again that 
$$
\esp{\vvvert \mathfrak{u}^p_{M}\vvvert^2}
\le 2\esp{\vvvert\Phi_M(\mathfrak{u}^{p-1}_{M}) - \Phi(\mathfrak{u}^{p-1}_{M})\vvvert^2}
+ 2 \esp{\vvvert \Phi(\mathfrak{u}^{p-1}_{M})\vvvert^2}
 $$
 we obtain
 \begin{align*}
 %\label{eq interm bound unif}
 \esp{\vvvert \Phi(\mathfrak{u}^p_{M}) \vvvert^2}
 \le
  2\delta_{h}(1+\varepsilon)\esp{\vvvert  \Phi(\mathfrak{u}^{p-1}_{M}) \vvvert^2} &+ 2  \delta_{h}(1+\varepsilon) \esp{\vvvert\Phi_{M}(\mathfrak{u}^{p-1}_{M}) - \Phi(\mathfrak{u}^{p-1}_{M})\vvvert^2} 
  \\
  &+C_\varepsilon \bigg( \cE_\pi + \cE_{\psi}+\vvvert \bar{\mathfrak{u}}\vvvert^2\bigg)
 \end{align*}
\noindent so that using \eqref{eq  robbins-monro here}, we get
%\textcolor{red}{\frac{C}M}
%+ \kappa_{\pi,\psi} L_{\pi,\psi,M} Nd 
%+ \frac{\kappa_{\pi,\psi}}{\alpha_{\pi,\psi}} L_{\pi,\psi,M} \esp{\vvvert \Phi(\mathfrak{u}^{p-1}_M) \vvvert^2}
 \begin{align*}
 %\label{eq bound unif almost final}
 \esp{\vvvert \Phi(\mathfrak{u}^p_{M}) \vvvert^2}
 \le&
  2\delta_{h}(1+\varepsilon)\left(1+\frac{\kappa_{K}}{\alpha_{K}} L_{K,M}\right) \esp{\vvvert  \Phi(\mathfrak{u}^{p-1}_{M}) \vvvert^2}
  \\
&+ 2  \delta_{h}(1+\varepsilon)  \kappa_{K} L_{K,M}\left(1+ d N  \right)
  +C_\varepsilon \bigg( \cE_\pi + \cE_{\psi}+\vvvert \bar{\mathfrak{u}}\vvvert^2\bigg)\;.
 \end{align*}
 From \eqref{eq ass cs control global} and the fact that $\delta_{h, \eta}$, we can set $\varepsilon$ such that $2\delta_{h}(1+\varepsilon)(1+\frac{\kappa_{K}}{\alpha_{K}} L_{K,M}) \le \delta_{h,\eta} (1+\varepsilon)<1$ so that from the above inequality, by induction, for any positive integer $p$, we get
 %\textcolor{red}{For $\delta_\epsilon$ small enough} such that $2\delta_{\varepsilon}(1+\frac{\kappa_{\pi,\psi}}{\alpha_{\pi,%\psi}} L_{\pi,\psi,M}) \le 1$ \textcolor{red}{A rediger plus proprement mettre c au lieu de C dans prop 3.4 de noufel... et %une remarque pour dire que c sera petit en pratique...}, 
 \begin{align*}
 \esp{\vvvert \Phi(\mathfrak{u}^p_{M}) \vvvert^2} \le   (\delta_{h,\eta}(1+\varepsilon))^{p}\esp{\vvvert \Phi(\mathfrak{u}^0_{M}) \vvvert^2}+ C_\varepsilon(\cE_\pi + \cE_{\psi}+\vvvert \bar{\mathfrak{u}}\vvvert^2 + \delta_h) \le C_\varepsilon\;,
 \end{align*}
 which concludes the proof.
\eproof

%\begin{bluetext}

\vspace{2mm}
\noindent We now have all the ingredients to give the proof of the main result announced in Section \ref{subse picard algo} on the upper bound for the global convergence error at the initial time.% \emph{Picard algorithm}.

\paragraph{Proof of Theorem \ref{th main conv result}} From the very definition \eqref{eq de error algorithm} of the global error, we deduce
\begin{align}\label{eq start decompose}
\cE_{\mathrm{MSE}} \le 2\esp{|u(0,\cX_0) - \bar{u}(\cX_0)|^2 + |Y^{\bar{\mathfrak{u}}}_0 - Y^{\mathfrak{u}^P_M}_0|^2}
\end{align}
\noindent where we used the notations introduced in \eqref{eq de Y starting point}, \eqref{y:reference:solution} and \eqref{the:reference:solution}. A fortiori, we have
\begin{align} \label{eq interm step decompose}
\esp{|u(0,\cX_0) - \bar{u}_0(\cX_0)|^2} \le \cE_\psi \quad \text{ and } \quad
\esp{|Y^{\bar{\mathfrak{u}}}_0 - Y^{\mathfrak{u}^P_M}_0|^2} \le \cE_P
\end{align}
recalling \eqref{eq error approx space}, \eqref{eq rewritte norms} and \eqref{eq de error picard}. Combining \eqref{eq interm step decompose} and \eqref{eq start decompose} yields
\begin{align}
\cE_{\mathrm{MSE}}  \le 2 \left( \cE_\psi  + \cE_P \right)\,.
\end{align}
We eventually conclude the proof by invoking Proposition \ref{pr main abstract error} together with Lemma \ref{le gamma spec LpipsiM}. \eproof
%\end{bluetext}
%\end{bluetext}





%\begin{Proposition}\label{pr error of Picard sharper}
%% \textcolor{red}{Just to have a rough idea of what is going on. Some estimates should be certainly improved...}
%Let the assumptions of Lemma \ref{le control robbins monro error} hold.
%Under Assumption \ref{as psi function}, if moreover, 
%\begin{align}\label{eq ass cs control global}
%\frac{\kappa_{\pi,\psi}L_{\pi,\psi,M}}{\alpha_{\pi,\psi}} \le C \; \text{ and }\;
% \kappa_{\pi,\psi} L_{\pi,\psi,M}  \le C 
%\end{align}
% %(see the proof for the definition of $L_{\pi,\psi,M}  $ )}, where 
% %\textcolor{red}{$ \| \cdot \|^2\le \frac{1}{\alpha_{\pi,\psi}} \vvvert \cdot \vvvert^2 $
% %\text{ and } $\vvvert \cdot \vvvert^2 \le {\kappa_{\pi,\psi}}  \| \cdot \|^2$}, 
% the following holds
%%\textcolor{red}{has to be improved ? see next section Prop \ref{error of Picard sharper}}
%For $T<1$ and $L^2T$ small enough, the following holds for some $ \tilde{\delta} \in [0,1)$
%\begin{align}
%\cE_P &\le C_{\tilde{\delta}} \Big( \tilde{\delta} ^P \cE_0+  \cE_{\mathrm{\psi}} +  \cE_{\mathrm{\pi}}  
%+ \frac{\kappa_{\pi,\psi}L_{\pi,\psi,M}}{\alpha_{\pi,\psi}} \Big)\;.
%%\\
%%&+C_{\tilde{\delta}} \frac{\kappa_{\pi,\psi}}{\alpha_{\pi,\psi}}
%%\Big(
%% \exp\left({-2\gamma\alpha_{\pi,\psi} M^{1-\eta}+ 2 \gamma\alpha_{\pi,\psi}+ C\gamma^2 \beta_{\pi,\psi}M^{1-2\eta}}\right) 
%% \nonumber
%%%\\ 
%%%&
%%+\exp\left(  C\gamma^2 \beta_{\pi,\psi} M^{1-2\eta}\right)\beta_{\pi,\psi} M^{1-2\eta}
%%\Big)
%\end{align}
%\end{Proposition}
%%\begin{bluetext}
%\proof
%1. 
%%\textcolor{yellow}{
%%First, we observe that Lemma \ref{le control robbins monro error} reads
%%\begin{align}\label{eq rewrites lemma robmon}
%% \esp{\|\Phi_M(\tilde{\mathfrak{u}}) - \Phi(\tilde{\mathfrak{u}}) \|^2 } &\le
%% L_{\pi,\psi,M} (1 +  \esp{\| \Phi(\tilde{\mathfrak{u}}) \|^2 })
%%\end{align}
%%}
%Using Lemma \ref{le control f(y,z)}, we have
%\begin{align}\label{eq interm lemma 4.3}
%\vvvert \Phi(\mathfrak{u}^p_{M})  -  \bar{\mathfrak{u}} \vvvert^2
%\le \delta^2 \vvvert \mathfrak{u}^p_{M} -  \bar{\mathfrak{u}} \vvvert^2 + \bar{C}_\delta(\cE_\pi + \cE_{\psi})
%\end{align}
%Note that $ \bar{C}_\delta$ is a constant that may change from line to line. \\
%We then compute
%\begin{align*}
% \esp{\vvvert \Phi(\mathfrak{u}^p_{M}) \vvvert^2}
% &\le
% 2 \esp{\vvvert \Phi(\mathfrak{u}^p_{M}) - \bar{\mathfrak{u}}\vvvert^2} + 2 \vvvert \bar{\mathfrak{u}}\vvvert^2
% \\
% &\le  2\delta^2 \esp{\vvvert \mathfrak{u}^p_{M} -  \bar{\mathfrak{u}} \vvvert^2} + \bar{C}_\delta(\cE_\pi + \cE_{\psi}+\vvvert \bar{\mathfrak{u}}\vvvert^2)
% \\
%  &\le  4\delta^2 \esp{\vvvert \mathfrak{u}^p_{M}\vvvert^2} 
%  +\bar{C}_\delta(\cE_\pi + \cE_{\psi}+\vvvert \bar{\mathfrak{u}}\vvvert^2)
%\end{align*}
%where we have used \eqref{eq interm lemma 4.3}.
%Noting that 
%$$
%\esp{\vvvert \mathfrak{u}^p_{M}\vvvert^2}
%\le 2\esp{\vvvert\Phi_M(\mathfrak{u}^{p-1}_{M}) - \Phi(\mathfrak{u}^{p-1}_{M})\vvvert^2
%+\vvvert \Phi(\mathfrak{u}^{p-1}_{M})\vvvert^2}
% $$
% we obtain
% \begin{align}\label{eq interm bound unif}
% \esp{\vvvert \Phi(\mathfrak{u}^p_{M}) \vvvert^2}
% &\le
%  8\delta^2 \esp{\vvvert  \Phi(\mathfrak{u}^{p-1}_{M}) \vvvert^2+\vvvert\Phi_M(\mathfrak{u}^{p-1}_{M}) - \Phi(\mathfrak{u}^{p-1}_{M})\vvvert^2} + \bar{C}_\delta(\cE_\pi + \cE_{\psi}+\vvvert \bar{\mathfrak{u}}\vvvert^2)
% \end{align}
%Recalling Assumption \ref{as psi function},
%%Since \textcolor{red}{$ \| \cdot \|^2\le \frac{1}{\alpha_{\pi,\psi}} \vvvert \cdot \vvvert^2 $
% %\text{ and } $\vvvert \cdot \vvvert^2 \le {\kappa_{\pi,\psi}}  \| \cdot \|^2$}, 
% we compute using \eqref{eq rewrites lemma robmon},
%% \textcolor{yellow}{
%%\begin{align}
%%\esp{\vvvert\Phi_M(\mathfrak{u}^{p-1}_{M}) - \Phi(\mathfrak{u}^{p-1}_{M}) \frac{1}{\alpha_{\pi,\psi}}^2 } 
%%\le
%% L_{\pi,\psi,M} (1 +  \frac{\kappa_{\pi,\psi}}{\alpha_{\pi,\psi}}\esp{\vvvert\Phi(\mathfrak{u}^{p-1}_{M}) \vvvert^2 })
%%\end{align} 
%%}
%\begin{align}
%\esp{\vvvert\Phi_M(\mathfrak{u}^{p-1}_{M}) - \Phi(\mathfrak{u}^{p-1}_{M})\vvvert^2 } 
%\le
% L_{\pi,\psi,M}\kappa_{\pi,\psi} \left(  1+  \frac1{\alpha_{\pi,\psi}}\esp{\vvvert\Phi(\mathfrak{u}^{p-1}_{M}) \vvvert^2 }\right)
%\end{align} 
%Inserting the previous estimate back into \eqref{eq interm bound unif}, we get
% \begin{align*}%\label{eq interm bound unif last}
% \esp{\vvvert \Phi(\mathfrak{u}^p_{M}) \vvvert^2}
% &\le
%  8\delta^2(1+\frac{\kappa_{\pi,\psi}L_{\pi,\psi,M}}{\alpha_{\pi,\psi}}) \esp{\vvvert  \Phi(\mathfrak{u}^{p-1}_{M}) \vvvert^2} + \bar{C}_\delta(\cE_\pi + \cE_{\psi}+\vvvert \bar{\mathfrak{u}}\vvvert^2) +  8\delta^2 L_{\pi,\psi,M} \kappa_{\pi,\psi}
% \end{align*}
% Combining \eqref{eq ass cs control global} with the previous inequality, we obtain
%% \textcolor{red}{Assuming $\frac{\kappa_{\pi,\psi}L_{\pi,\psi,M}}{\alpha_{\pi,\psi}} \le C$ and
%% $\kappa_{\pi,\psi} L_{\pi,\psi,M}  \le C$, We can delete the second condition }, we obtain
% \begin{align*}
% \max_{0 \le p \le P } \esp{\vvvert \Phi(\mathfrak{u}^p_{M}) \vvvert^2} \le C(1+\cE_\pi + \cE_{\psi}+\vvvert \bar{\mathfrak{u}}\vvvert^2)\;.
% \end{align*}
% 2. For all $p$ we thus get
%  \begin{align*}
% \esp{\vvvert\Phi_M({\mathfrak{u}}^p_M) - \Phi({\mathfrak{u}}^p_M) \vvvert^2 } &\le
%C \frac{\kappa_{\pi,\psi}}{\alpha_{\pi,\psi}} L_{\pi,\psi,M}\;.
%%\Big(
%% \exp\left({-2\gamma\alpha_{\pi,\psi} M^{1-\eta}+ 2 \gamma\alpha_{\pi,\psi}+ C\gamma^2 \beta_{\pi,\psi}M^{1-2\eta}}\right) 
%% \nonumber
%%\\ 
%%&+\exp\left(  C\gamma^2 \beta_{\pi,\psi} M^{1-2\eta}\right)\beta_{\pi,\psi} M^{1-2\eta}
%%\Big)
% \end{align*}
% The proof is concluded using Proposition \ref{error of Picard}.
%\eproof
%%\end{bluetext}

